Towards Prototyping Driverless Vehicle Behaviors, City Design, and Policies Simultaneously

Autonomous Vehicles (AVs) can potentially improve urban living by reducing accidents, increasing transportation accessibility and equity, and decreasing emissions. Realizing these promises requires the innovations of AV driving behaviors, city plans and infrastructure, and traffic and transportation policies to join forces. However, the complex interdependencies among AV, city, and policy design issues can hinder their innovation. We argue the path towards better AV cities is not a process of matching city designs and policies with AVs' technological innovations, but a process of iterative prototyping of all three simultaneously: Innovations can happen step-wise as the knot of AV, city, and policy design loosens and tightens, unwinds and reties. In this paper, we ask: How can innovators innovate AVs, city environments, and policies simultaneously and productively toward better AV cities? The paper has two parts. First, we map out the interconnections among the many AV, city, and policy design decisions, based on a literature review spanning HCI/HRI, transportation science, urban studies, law and policy, operations research, economy, and philosophy. This map can help innovators identify design constraints and opportunities across the traditional AV/city/policy design disciplinary bounds. Second, we review the respective methods for AV, city, and policy design, and identify key barriers in combining them: (1) Organizational barriers to AV-city-policy design collaboration, (2) computational barriers to multi-granularity AV-city-policy simulation, and (3) different assumptions and goals in joint AV-city-policy optimization. We discuss two broad approaches that can potentially address these challenges, namely, "low-fidelity integrative City-AV-Policy Simulation (iCAPS)" and "participatory design optimization".

==> abstract.tex <==
% Qian
Autonomous Vehicles (AVs) can potentially improve urban living by reducing accidents, increasing transportation accessibility and equity, and decreasing emissions. Realizing these promises requires the innovations of AV driving behaviors, city plans and infrastructure, and traffic and transportation policies to join forces. However, the complex interdependencies among AV, city, and policy design issues can hinder their innovation.
We argue the path towards better AV cities is not a process of matching city designs and policies with AVs’ technological innovations, but a process of iterative prototyping of all three simultaneously: Innovations can happen step-wise as the knot of AV, city, and policy design loosens and tightens, unwinds and reties.
In this paper, we ask: How can innovators innovate AVs, city environments, and policies simultaneously and productively toward better AV cities?
The paper has two parts. First, we map out the interconnections among the many AV, city, and policy design decisions, based on a literature review spanning HCI/HRI, transportation science, urban studies, law and policy, operations research, economy, and philosophy. This map can help innovators identify design constraints and opportunities across the traditional AV/city/policy design disciplinary bounds.
Second, we review the respective methods for AV, city, and policy design, and identify key barriers in combining them: (1) Organizational barriers to AV-city-policy design collaboration, (2) computational barriers to multi-granularity AV-city-policy simulation, and (3) different assumptions and goals in joint AV-city-policy optimization. We discuss two broad approaches that can potentially address these challenges, namely, “low-fidelity integrative City-AV-Policy Simulation (iCAPS)” and “participatory design optimization”.

% camera ready - abstact as arXiv metadata
Autonomous Vehicles (AVs) hold the potential to significantly improve urban living by reducing accidents, increasing accessibility, and decreasing emissions. However, to realize these benefits, it is crucial to address the complex interplay between AVs, city design, and policies. This paper examines the intertwined relationships among these three aspects, forming a "knot" that challenges innovation. We first present a comprehensive map of these interconnections based on a cross-disciplinary literature review. This map aids innovators in identifying design constraints and opportunities across traditional disciplinary boundaries. Next, we explore how innovators might simultaneously prototype AV, city, and policy innovations by reviewing existing methods and discussing the barriers to combining them. We propose two potential approaches, "low-fidelity integrative City-AV-Policy Simulation" and "participatory design-optimization," to overcome these barriers and foster collaboration between AV designers, urban planners, and policymakers. Our work aims to catalyze a more principled discussion on how these stakeholders can work together to innovate AVs and better cities.

% v3
Autonomous Vehicles (AVs) have the potential to make cities safer, more livable, sustainable, efficient, and equitable. Unfortunately, these benefits will not unfold automatically. In fact, evidence suggests that AV implementation without policy interventions and changes to urban infrastructure could result in adverse effects. To achieve optimal outcomes with the introduction of AVs, cities must therefore coordinate design of urban infrastructure, AV behaviors, and policy. \placeholder{We argue that current methods such as stakeholder engagement which work for localized decision making, and single goal optimization, which work for network-wide decision making will not work with AVs.} In conclusion, we observe a clear need for novel AV Policy making methods and outline two possible directions. 






 % + economics?
%  Current AV design, through real-world trials, takes city infrastructure, and AV policy as determinate. 
% Cities are governed by complex rules that were established over long periods of time. 
% To address these circular dependencies and complexities, we need to devise new  methods and tools.
% Holistic policy, urban infrastructure, and autonomous vehicle simulation can provide insights into the interdependencies among these components and to anticipate how ideals of efficient, livable, sustainable cities fold out.  Multi-goal optimization is one possible method to understand the trade-offs between these goals. To illustrate the potential of these methods, we explore the tensions between AVs as commercial products and as public infrastructure.

% % v2
% Autonomous Vehicles (AVs) promise to help make cities more livable, sustainable, efficient, and equitable. % Qian: how? evidence?
% % Autonomous Vehicles (AVs) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. 
% % Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% However, cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes city infrastructure, and AV policy as determinate. To achieve optimal outcomes of livable, sustainable, efficient, and equitable cities with the introduction of AVs, cities must consider the malleability and interconnectedness of urban infrastructure, AV behavior, and policy. % + economics?
% % To address these circular dependencies and complexities, we need to devise new  methods and tools.
% % Holistic policy, urban infrastructure, and autonomous vehicle simulation can provide insights into the interdependencies among these components and to anticipate how ideals of efficient, livable, sustainable cities fold out.  Multi-goal optimization is one possible method to understand the trade-offs between these goals. To illustrate the potential of these methods, we explore the tensions between AVs as commercial products and as public infrastructure.



% v1
% Autonomous Vehicles (AVs) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. However, cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes city infrastructure, and AV policy as determinate. To achieve optimal outcomes of livable, sustainable, efficient, and equitable cities with the introduction of AVs, cities must consider the malleability and interconnectedness of urban infrastructure, AV behavior, and policy. % + economics?
% To address these circular dependencies and complexities, we need to devise new  methods and tools.
% Holistic policy, urban infrastructure, and autonomous vehicle simulation can provide insights into the interdependencies among these components and to anticipate how ideals of efficient, livable, sustainable cities fold out.  Multi-goal optimization is one possible method to understand the trade-offs between these goals. To illustrate the potential of these methods, we explore the tensions between AVs as commercial products and as public infrastructure.


==> archive/snippets.tex <==
\section{Introduction}
\hauke{Move most of this -> into RW}\qian{Some can go to the first para of intro too.}
% The pursuit of creating livable cities for all through technology innovations such as autonomous vehicles has become increasingly prevalent, but the development of socially desirable autonomous vehicles that enable sustainable mobility for all and not simply amplify existing issues cannot be left solely in the hands of individual car companies, and proactive policymaking by local governments is required to ensure that the potential pitfalls of AV technology are addressed.

% How AV testing is done currently  
Across the world, many cities have allowed AV trials, which enable AV developers to develop, test and refine their technology. These trials consider the nascent state of the technology with policy exemptions and focus on ensuring safe test of the technology. These trials are run in location and time-limited sandboxes, which allow experimentation of technology even in situations where the legislation is not yet on par with the technology developments \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}. 
% What policies are currently implemented / Why Gov needs to do someting and private engagement is not sufficient
As of now, all known implemented AV policies are targeting AV technology trials \cite{APA_Board_of_Directors2018-dq}. Some policymakers acknowledge that the implementation of the technology has pitfalls and want to consider policies that mitigate adverse AV effects in the future. Governments need to support that socially desirable autonomous vehicles are created. Autonomous vehicles should enable sustainable mobility for all, and not amplify existing issues of individual car ownership. This means that the development of autonomous vehicles cannot just be left in the hands of individual car companies, as their business models are not fully compatible with social good. Notable work by \citet{Fagan2021-np} advocates for proactive policymaking by local governments.




\section{Related work}

\hauke{
RW
= Why is simulation useful for prototyping/evaluating new transportation policies
= Current simulations focused single optimization goals
== even that cannot run at very large scale
= These simulations do not consider infrastructure as changeable 

Important previously-unknown research question: How do we draw the line between AVs as products vs AVs as public infrastructure? 
RW
=“Transportation for all” is important, everyone (from industry to academia) agrees
Towards, “transportation for all” PD workshops “hit a wall” (needs a better word for this) whenever AVs’ commercial nature/interests kick in
==Current simulations/PD workshops don’t consider different AV types/companies
==visions [cite:Wendy \& Helen]
==commercially not viable 
=This tension hasn’t been studied 
=There are emergent signs of this tension
==Uber as public transit
==John Zimmerman?? Someone at CMU? car data ownership
==Berlin car public infrastructure parking??
}

\hauke{
Key observations: the introduction of autonomous vehicles (AVs) into cities will have a significant impact on city design, but there is uncertainty about how and what the impacts will be. Ridesharing has mixed findings, some papers suggest the potential to minimize congestion, while others found an increase in vehicle miles traveled. City and transport planning complex slow. Many different approaches used in practice and novel methods proposed. Complexity due to many stakeholder, various demands, much interfacing between people, difficult responsibility and economics, policy making long term, principles and reality clash. Mistakes in planning are costly and sometimes impossible to reverse once infrastructur is built. Interfacing between governmental agencies and private companies/planners with conflicts of interests. AVs are predominanetly build through real world testing and simulation. Closed tracks offer only limited use. City and transport design rely incresingly on computational methods. It is important to be able to assess qality of life in a city through more holistic metrics, which is is an ongoing discussion.  SImulations are used for improving traffic flow, micromonility service provider and ride sharing use simulation and optmization approaches successfully for increased efficiendy of their networks. Better integration of ride sharing and public transport. Simulation and optimization of cities and transport networks, are very useful but have limitations. Only sub components of itnerest are usuallt modeled, some variables are hold fixed, i.e,, city planners treat traffic with simpler models, traffic planners take cities as fixed, polict makers take assumptions about how vehicles behave. 
}

\begin{figure}
    \centering
    \includegraphics[width=0.333\textwidth]{figures/Temporary_1.png}\includegraphics[width=0.333\textwidth]{figures/Temporary_2.png}
    \caption{Tools for planning cities, autonomous vehicles, and policies.}
    \label{fig:simulator}
\end{figure}

ONE LINE SENTENCE

\qian{This paragraph is making quite a few arguments; Try streamline the arguments and spread them over multiple paragraphs.}
The introduction of autonomous vehicles into cities will have significant impacts on city design, but there is uncertainty about the nature and magnitude of these impacts, and complex stakeholder interactions and conflicts of interest make planning difficult, with costly and sometimes irreversible consequences, and simulation and optimization tools are useful but limited. While cities and transportation are carefully planned, AV training currently is passive, learning from the given environment and copying human behaviors. 
%% BODY; --To done-- reorganize section
The extent of AVs effects on transportation and cities as a whole is uncertain. 
Analysis of impacts of on-demand ride-sharing, micromobility and taxi services show mixed findings, with some studies suggesting potential congestion reduction and others indicating an increase in vehicle miles travelled \cite{Tettamanti2016ImpactsOA, Felipe-Falgas2022-dz}. The impact of these novel technologies, appear to fold out differently in locations due to differences in policy and culture. Micromobility, for example, was found to be a sustainable improvement to city transport by some studies and a mere tourist travel tool in other regions. 
City and transport planning is complex and slow due to the involvement of multiple stakeholders with different demands, conflicting interests, and limited interfaces between them. Mistakes in planning are costly and often irreversible once infrastructure is built. 
Therefor for planning, a variety of methods and tools, such as digital twins, tangible city modelling, simulation, optimization, participatory workshops etc. are used. AVs are mainly built using data gathered from real-world testing, but increasingly relying on simulation methods as well. Algorithmic fleet management systems and route optimization software are successfully used by robotaxi fleets, ride-sharing services, and modern long-distance bus companies to efficiently plan the allocation of vehicles and routes within a city or between cities.
The use of simulation and optimization is effective in achieving individual goals, such as fleet utilization and traffic flow optimization, but they are not integrated with each other, limited in the use for optimizing multiple factors, multiple interdependent systems anticipating cause and effect with other system agents, take many variables as fixed assumptions, and are computationally limited to model only subcomponents of interest.
These tools can also serve as boundary tools for interfacing between governmental agencies, private companies/planners and the public. Due to conflicts of interest and  hard to quantify goals such as walkability and accessibility, design thinking and participatory design workshops are frequently used to facilitate multi-stakeholder alignment and planning. 
Resolving incompatibilities between visions for the future can be challenging, particularly when differences arise between the practicality of business models and ideal outcomes. One open question is whether autonomous vehicles, the infrastructure supporting them, and the services, as well as data, gathered can be considered public assets and public or are exclusively private property?

 % -- TODO-- Add all the new and old citations. 
\hauke{How about reactionist? I am looking for a word that describes well that the AVs take the environment and behaviors as given, without ambition to shape them.}

\hauke{1. Introduction of AVs and their potential impact on city design, along with the uncertainty and complexity of their impacts.
2. Mixed findings on the impact of on-demand ride-sharing, micro-mobility, and taxi services, with differences in policy and culture affecting outcomes.
3. Complexity and challenges of city and transport planning due to multiple stakeholders, conflicting interests, and limited interfaces.
4. Use of various tools and methods, including simulation and optimization, participatory workshops, and digital twins, to aid in planning and decision-making.
5. Success of simulation and optimization in achieving individual goals, but limitations in their integration and ability to model multiple interdependent systems.
6. Role of boundary tools like design thinking and participatory design workshops in facilitating multi-stakeholder alignment and planning.
7. Challenges in resolving incompatibilities between visions for the future, particularly in balancing practical business models and ideal outcomes.}


% OLD NOTES Keeep for now for easy copy pasting (!)
(Interaction Research)
Vehicle interaction research provides a rich history of humans interacting with cars. This line of research is crucial to understand how, human driven cars interact with each other, and how humans interact with Avs. 
(Tangible city prototyping)
Playful tools for prototyping with tangible material have been devised in the HCI community. These tools often show as one of their use cases the design of cities and urban space. To our knowledge, none of these tools have been picked up for policy making, city design and outside museums. 
(Design Thinking city)
Design thinking approaches have been extremely successful in product development. Naturally, these approaches have been tried to be applied in city and transportation design as well \cite{Schliwa2019-dr}. The success of these techniques seem to have been less fruitful. (WHY?) 
(Simulation environments)
Traffic simulation are heavily used in transportation science, city planning and vehicle interaction research. There is a multitude of highly specialized tools for various purposes. Because these tools are developed by different entities and based on different software backends, the simulation models are incompatible. As these incompatibilities between simulation environments hinder process a few open simulators are emerging. Notable is CARLA which is receiving industry and academic support for development of the platform  \cite{Dosovitskiy2017-jb}, extension of it \cite{Hofbauer2020-vc} and datasets \cite{Kloukiniotis2022-nc, Maag2022-ly, Yuan2021-sj}. 

Transportation optimization 
Various models of transportation have been created. Usually they model sub-aspects of a transportation network. As solving complex networks, with multiple variables is still to difficult to compute, multiple approximations and optimization approaches are used. These models often define individual goals, such as transportation efficiency or sustainability to be optimized. Multi goal optimization through e.g. Bayesian optimization are advancing in promising directions to become of use for city and AV design.
Multi-optimization-goal simulation is a potentially good way to prototype/evaluate new transportation policies (e.g., Bayesian optimization)

(AV development in simulators and on the road)
AV development is increasingly done in simulators. These simulator allows flexible creation of urban scenes, various road networks, and unique scenarios. Synethtic data from these simulators can help overcome dat bias from the real world. 
(Requirement specification) 
Researchers recognized that the influence of AVs reaches beyond local impact. Policy thus cannot, as done now, only specify local requirements such as safety and efficiency but has to address social and sociotechnical impacts\cite{Gilbert2022-vh}. 
(Measuring livability)
Not all qualities of cities are systematically addressed and measured. Important properties of city design such as walkability and accessibility only have been recently quantified\cite{Ewing2009-hv}. Complexities of aligning competing variables have been successfully addressed by designers. 
(Competing visions)
AV developers and service providers seek competing visions for autonomous futures. \citet{Goldenfein2020-it} categorize them in the archetypes driver assist, driverless cars, and connected cars. Contrary to the SAE model \cite{Of_Automotive_Engineers_SAE2018-hd}, which seems to suggest development along a linear trajectory, there will be different models of AVs, with varying levels of connectivity and human control.

(Design streets for AVs)
Need to specifically design streets for AV was mentioned in \cite{Riggs2019-lx}. AVs have various different technical demands and opportunities. Street infrastructure can assist AVs. 

(Micromobility chaos)
Valuable lessons can be taken from the similar coordination difficulties which occurred with micromobility services. Because of chaos in some locations due to initially loose policies, many cities have  reacted with very strict policies. Often, only individual providers were fractured, which forced some micromobility providers to stop offering their services. Due to these inconsistent policy changes, the micromobility market is very fragmented, international, national, and sometimes even on a local level. This fragmentation, though necessary for local governments to take control, has downsides for user experience and competition. 

(Policy Labs)
Policy labs are set up in cities for multi stakeholder design of policy. These policy labs usually us design thinking methods with the hope for more modern, i.e., fast paced, iterative policy making. Policy making is usually still a slow process that requires a lot of interactions between multiple partys. Ambiguous policies are a feature and problem of policies. 

(Stakeholder and market misalignment)
“Transportation for all” is important, everyone (from industry to academia) agrees on this. 
Towards, “transportation for all” PD workshops “hit a wall” whenever AVs’ commercial nature/interests kick in. Even well intending companies need to face business realities. 
Current simulations/PD workshops don’t consider different AV types/companies as competitors. 
Different AV visions are competing with each other. I.e., robotaxi like public transport in the hand of a few commercial entities, individual vehicle ownership with highly advanced assistive systems, fully connected (cars and infrastructure) systems of cars. 
Are AVs private commercial products or are they part of the public infrastructure this is not really studied academically. 
However there are are emergent signs of this tension:
1. Uber as public transit, required to behave fairly to customers beyond what a private company usually needs to. I.e, requiement for accessible vehicles, and requirement to drive in dangerous, low tipping neighbourhoods. The reverse exists as well, not just private companies being pushed to act in public interest, but also private companies trying to get benefits of being public good. 2. Example of Berlin ridesharing services trying to skip paying parking fees to the city as they would contribute to public transportation rather than blocking parking space. 3. Discussions regarding data ownership. Increasing arguments that data collected from autonomous vehicles should be public use and not property of infividual companies. 

(complex interdependent system)
A complex interdependent system involving diverse traffic members, such as human-driven cars, AVs, pedestrians, cyclists, buses, metro, delivery robots and more, interacts with each other on roads and city-spanning networks. The changing of one variable in this complex sociotechnical system can have unintended consequences, as both city infrastructure and local norms determine AV behavior, while AVs can also determine other road members' behavior. Simulation studies show that a few AVs can control mixed traffic flow \cite{Wu2018-oy}, highlighting the importance of considering city infrastructure as a flexible and adaptive system that can be changed to accommodate AVs. The design and optimization of this interdependent system is challenging.
Policy and legislation towards new technology are often conservative, as unwary policy can cause harm, while overcautious policy limits technology adoption. Effective policy design requires a well-calibrated understanding of the risks and benefits of technology, as demonstrated by the repeal of the red flag law in late 19th century Britain after three decades\cite{Wikipedia_contributors2022-xo}.
Workshops with role-playing elements for policymaking of AVs have been proposed as a method for rapid, iterative design of complex systems for multiple stakeholders. 

\section{Proposition}
% \qian{What's the takeaway from this paragraph?}
% In a busy city, delivery robots are deployed to meet the growing demand for food delivery. However, due to lacking behind city infrastructure and policy, these robots frequently get stuck at sidewalks. As a result, pedestrians are unable to walk freely, and delivery takes long in some neighborhoods, leading to customer as well as non customer dissatisfaction.
% The challenge facing city planners is to determine which solutions are the best fit for the city's needs. How can they determine which solutions are the most cost-efficient, which ones are best for quality of living, and which ones can be implemented later? 
% The list of potential solutions is long; including street upgrades such as building accessibility ramps, wider sidewalk; new types of infrastructure, such as dedicated delivery lanes, mixed traffic lanes, or delivery drop off centers; new technical infrastructure improvements, such as smart traffic lights, that can be controlled by robots, and policy solutions such as, collecting local tolls, allowing robots to use bicycle paths or roads and limiting their dwell time. 
% The question arises, which of these alternatives is the right one? Which solution is most cost-efficient? Which solution is best for the quality of living? How can the city implement these solutions, given that the technologies are not yet deployed?
% Without proper AV policy design methods, including real-world experiments and simulations, it is difficult for city planners to make informed decisions about the deployment of autonomous vehicles.

% It is crucial for city planners to reason about alternatives in a systematic and evidence-based manner. Otherwise, they risk implementing solutions that are inefficient, ineffective, or even harmful to the city's residents. These complications show the need for new, effective AV policy design methods. 
% Potential design methods such as real-world experiments, simulations, and participatory design, that can help city planners make informed decisions have to be devised. Without these methods, it is difficult to determine which solution is the best, considering the implications of each solution on cost and quality of life. By adopting better design methods, cities can ensure that AV policies are well-informed and effective in promoting sustainable and equitable transportation.



\section{Discussion}

The use of autonomous vehicles in urban transportation has the potential to revolutionize the way people and goods are transported. However, the deployment of these vehicles is not without challenges, especially in terms of policy design. Cities need to adopt evidence-based and systematic approaches to policy design to ensure that AVs are deployed in a way that is sustainable, efficient, and equitable.
One of the key challenges in AV policy design is to ensure that the deployment of these vehicles aligns with the city's overall vision and goals. For instance, cities need to ensure that AVs promote sustainability, improve road safety, and enhance access to transportation for all. 
Another challenge in AV policy design is the integration of AVs into the existing urban infrastructure. Cities need to consider the implications of deploying AVs on the street network, including traffic flow, accessibility, and safety. For example, cities need to determine which types of infrastructure, such as dedicated delivery lanes, mixed traffic lanes, or delivery drop-off centers, are most suitable for AV deployment.
The use of real-world experiments, simulations, and participatory design can help cities make informed decisions about AV policy design. These methods can provide valuable insights into the implications of different policy solutions, such as the cost and quality of life, and help cities identify the best solutions for their needs.
In conclusion, the deployment of autonomous vehicles in urban transportation requires careful policy design to ensure that they are deployed in a way that is sustainable, efficient, and equitable. Cities need to adopt evidence-based and systematic approaches to policy design, such as real-world experiments, simulations, and participatory design, to ensure that AVs align with the city's overall vision and goals and integrate well with the existing urban infrastructure. By taking these steps, cities can ensure that the deployment of AVs promotes sustainable and equitable transportation for all.

==> archive/v1.tex <==
\hauke{
Abstract \checkmark, Introduction, RW \checkmark, method \checkmark, proposition (half), discussion \checkmark }

\section{Introduction}
% Title+ abstract + Introduction: 1 1/3 page

AVs have the potential to improve cities in various ways, such as by increasing safety, sustainability, and equity. \qian{Why? how? Add evidence.}

This paper acknowledges the interdependence between AVs, policies, and urban infrastructure and emphasizes the need to consider these factors together. In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues. The paper concludes that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities. We propose to develop AV integration simulators \hauke{Needs better name} to prototype AV, driving policy, and the necessary city infrastructure together. 

\hauke{Move most of this -> into RW}

% The pursuit of creating livable cities for all through technology innovations such as autonomous vehicles has become increasingly prevalent, but the development of socially desirable autonomous vehicles that enable sustainable mobility for all and not simply amplify existing issues cannot be left solely in the hands of individual car companies, and proactive policymaking by local governments is required to ensure that the potential pitfalls of AV technology are addressed.

Cities transportation infrastructure and in connection quality of life at the curb leave much to be desired. To create livable cities for all, technology innovations are promoted as the key enabler, rather than pouring more money into old infrastructure and processes \cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. Public transport infrastructure on the one hand is expensive and cannot transport individuals all the way through their journey. Individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Therefore, many local governments put hope into AVs; opportunities sought are improved road safety, sustainability, lowered congestion, and improved access to transportation \cite{World_Economic_Forum2020-ox}.
Across the world, many cities have allowed AV trials, which enable AV developers to develop, test and refine their technology. These trials consider the nascent state of the technology with policy exemptions and focus on ensuring safe test of the technology. These trials are run in location and time-limited sandboxes, which allow experimentation of technology even in situations where the legislation is not yet on par with the technology developments \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}. 
As of now, all known implemented AV policies are targeting AV technology trials \cite{APA_Board_of_Directors2018-dq}. Some policymakers acknowledge that the implementation of the technology has pitfalls and want to consider policies that mitigate adverse AV effects in the future. Governments need to support that socially desirable autonomous vehicles are created. Autonomous vehicles should enable sustainable mobility for all, and not amplify existing issues of individual car ownership. This means that the development of autonomous vehicles cannot just be left in the hands of individual car companies, as their business models are not fully compatible with social good. Notable work by \citet{Fagan2021-np} advocates for proactive policymaking by local governments.


\section{Related Work}
%Related Work (“What do other people think so far”?)
% RW: ½ leaf

% \hauke
% { 
% AVs’ great promises in making cities better: more livable, sustainable, efficient, and equitable cities (added safer, did not add healthier as this can be considered to be part of livable) 
% }

AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}.

% \hauke
% { 
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together.
% There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence 
% simulations focus on one goal only
% }

It is recognized that AVs and policies \cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn}, as well as AVs and urban infrastructure \cite{Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP} are interrelated and mutually influential, they \textit{should} be considered together \cite{Staricco2019TowardPT, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me}. Examples of unique AV infrastructure are newly designed roads, lanes, and crossings \cite{Riggs2019-lx, National_Association_of_City_Transportation_Officials2019-ll}, newly designed traffic lights \cite{Niroumand2023-an}, reduced or displaced parking space \cite{Staricco2019-gn} and alternative use of street space \cite{Freemark2020-ms}.  Examples of unique AV policy are incentivizing the use of shared AVs, requiring a minimum amount of accessible AVs, and  pricing curbside parking dynamically\cite{Sperling2018-vk, Freemark2020-ms, National_Association_of_City_Transportation_Officials2019-ll}. 
 
There are trade-offs to be made implementing these high-level ideals of safer, more livable, sustainable, efficient, and equitable cities. These are in the literature often described as either-or social dilemmas, such as 'should self-interest or the public good predominate \cite{Bonnefon2015TheSD}', 'should autonomous vehicles be owned or shared \cite{Lee2019AutonomousVC, Campbell2018-rr}', and 'should AVs be planned or self-organize \cite{Bosch2017-sv}'? These hard choices need to be made in the design process. This nuanced considering of trade-offs is usually not considered in simulations and optimization, where only individuals goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 

% \hauke
% { 
% People working on these 3 things are not working with each other
% We don’t quite know why people are not working together, but we do know…
% they do not
% }

While we do not know the reasons for more holistic design and development of AVs, city infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{National_Association_of_City_Transportation_Officials2019-ll}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  

% \hauke
% { 
% They unknowingly disagree about how these ideals (livable, sustainable, etc.) should look like in reality.
% E.g., tensions between AVs as commercial products versus AVs as public infrastructure
% }

There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019TowardPT, Meeder2017AutonomousVP, Acheampong2021-ql}. Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.

% \hauke
% { 
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes city infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …
% }

People who try to design policies, AVs, and urban infrastructure together lack methods to do so \cite{Rouse2021-ph}; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.

 
Cities are governed by complex rules that were established over long periods of time; AV design methods, however, do not include the design of policies and infrastructure, testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}. Simulations focus on AV only, with often very simple road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}. The simulator environments used for training of AVs, which have all flexibility in infrastructure and policy re-development, do not do so \citetodo{}.   
%  Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}.  

Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.  \citet{Yang2019-nr} recognize the lack of any analysis-design-evaluation decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

% \hauke
% {
% As a result, tensions (e.g., tensions between AVs as commercial products versus AVs as public infrastructure) are discussed, but never resolved.
% }

As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.

A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}, and there is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 


\section{Research Goal}


Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores the potential design-related problems that could arise from the deployment of autonomous vehicles without adequate methods and tools for integrated policy and city design. 

The initial research question guiding this work was "How should we design autonomous vehicles and cities together at scale?". Branching off from this we ventured into diverse fields and research areas including transportation science, urban studies, city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, philosophy, and participatory design. 
The analysis of the contributing literature, particularly in AV technology and infrastructure, the potential impact of AVs on transportation efficiency, equity, and sustainability, and the role of policy in regulating the deployment of AVs, revealed many open problems and desire for more open and interdisciplinary collaboration. 

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 



\section{Proposition}
% Finding/Your proposition (“What do you argue and what’s the evidence?”)
% Findings/Our proposition: 1.5 pages


The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 

Simulation tools, specifically created for policymaking city officials, are required to project how city infrastructure, AV behavior and AV policy interact. 
% economics of designing livable cities and distributing costs between individuals and AV providers.
We argue that simulators are necessary because only they allow for the evaluation and optimization of transportation policies in a safe, controlled, and cost-effective environment, without having to conduct expensive real-world experiments, and before building infrastructure. This provided insights would not be available through traditional analysis, making them the best way to prototype and evaluate new transportation policies.
Simulation is the solution when models are too complex and cannot be fully solved. Even simulations though run into computational limitations. Here recent work pushed simulators to run at large scale \cite{Chan2018-km}.
With holistic approaches to simulation of AVs, city infrastructure and implemented policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look like in reality.
Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a lower level. 
Multi-goal-optimization can become a helpful tool for such as some, i.e, cities livability, cannot be reduced to individual metrics such as road efficiency. Bayesian optimization, which can help policymakers to evaluate the effects of different policies on multiple objectives such as travel time, energy use, and environmental impact, seems to be a promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 
\hauke{We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.}
While the dilemmas of AV, e.g., public vs. private vehicle ownership, appear as dilemmas, historically they were resolved one way or another. Using holistic simulation, we can discuss them early on and hopefully avoid badly planned cities. Using these tools, we can better anticipate if the public should intervene, and how much they have to invest to achieve higher goals. 



\section{Discussion}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools, as it allows for the most flexibility and integration. We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. Ultimately, even the HCI community cannot realize these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. 

Even though we promote integrated approaches, specialized field expertise is necessary, we do not see such an AV policy infrastructure simulator as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v2.tex <==

\section{Introduction}
% Title+ abstract + Introduction: 1 1/3 page

% This paragraph: Describe the great promises of AVs + cities + policies working together. Subtext: Why, despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 

% This paragraph: What prior work has done in realizing the promises, what is still lacking, and why that's not good.
While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not  optimally prepare urban infrastructure and policies for the arrival of AVs. 
\newline
% This paragraph: This paper's contribution in realizing the great promises.
In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. With \textit{policies}, we refer to both transportation policies and traffic laws. With urban infrastructure, we refer to transport infrastructure such as roadway features  traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. %zoning? Would be part of urban planning if we go to that category of urban zoning we would say AVs do not incorporate possibilites of urban planning... 
The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 



% The pursuit of creating livable cities for all through technology innovations such as autonomous vehicles has become increasingly prevalent, but the development of socially desirable autonomous vehicles that enable sustainable mobility for all and not simply amplify existing issues cannot be left solely in the hands of individual car companies, and proactive policymaking by local governments is required to ensure that the potential pitfalls of AV technology are addressed.


\section{Related Work}
%Related Work (“What do other people think so far”?)
% RW: ½ leaf

\subsection{Promises (or the inherent entanglement??) of AVs+Cities+Policy}

% This paragraph: AVs’ great promises in making cities better: more livable, sustainable, efficient, and equitable cities (added safer, did not add healthier as this can be considered to be part of livable) 
AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}. Commonly, mentioned benefits are reduced traffic accidents, decrease in vehicle emissions and congestion, improved safety for pedestrians and cyclists, better mobility for the elderly and disabled, increase in active travel, as well as reduced need for parking space. 

% \qian{Add a few sentences elaborating the evidence presented in these papers. It's rare that readers actually go find these papers and read them, then decide whether they buy this argument or not.}

% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }

% This paragraph: Realizing these promises needs (1) AV-city-policy coordinating with each other.
Realizing such AV-infused better cities requires the \textit{coordination} between the designs of AV behaviors, traffic law, traffic policy, and urban infrastructure~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019TowardPT, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me}. Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}. For example, without policy intervention, it is likely that vehicle activity will increase overall due to the convenience of AVs over mass transport~\cite{Soteropoulos2019-tw}.
% \qian{clarify what kind of policy. traffic law? AV algorithm policy?}
%are interrelated and mutually influential, Qian: I feel the fact that AV/city/policy is somewhat self-evident from the examples we give below, so I removed this part. If we want to add it back, we should elborate on why and how they are interconnected and mutually influential.
\hauke{The interrelatedness and mutually influentialness seems indeed evident. I like the word coordination, but is it enough? Probably separate papers suggesting coordination from those that discuss the need to understand "interaction effects". This shall be a pointer to need to simulations to understand the dynamics between these as a system. 
What policy? I meant transportation policy. Data and algorithm policy, might matter too but it has less impact on the urban infrastructure. Traffic laws should be considered too. thus actually we are talking about impact on transpotation law and policy as well as traffic law and policy -> The term that groups all four concepts (traffic law, traffic policy, transportation law, and transportation policy) together is "transportation governance.}
%\placeholder{In order for AVs and cities to XXXX} \qian{Add this phrase to make clear how considering AV+city+policy together can help realize the promises of better cities (the promises described in the prev. paragraph}, 

To fully realize the promised benefits of AVs, it is crucial to implement AV-specific policies, such as ensuring a minimum number of accessible AVs; On the other hand, in order to mitigate the potential negative impacts of AVs, policies must be put in place that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, National_Association_of_City_Transportation_Officials2019-ll}. 
In order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, National_Association_of_City_Transportation_Officials2019-ll}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}. \hauke{Changed to present tense as this has not happened yet.}

\subsubsection{Challenges in designing policies, cities, and AVs together}
% This paragraph: Realizing these promises needs (2) AV-city-policy designs make trade-offs in order to achieve XXX
Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% These are in the literature often described as either-or social dilemmas, 
Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}


\subsection{Existing (Isolated) Methods in Designing AVs, Cities, Policies}

% This paragraph: However, people are not working together. Methods are isolated from each other.
% People working on these 3 things are not working with each other. We don’t quite know why people are not working together, but we do know…they do not...

These hard choices need to be made in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 

While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{National_Association_of_City_Transportation_Officials2019-ll}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  

% \hauke
% { 
% They unknowingly disagree about how these ideals (livable, sustainable, etc.) should look like in reality.
% E.g., tensions between AVs as commercial products versus AVs as public infrastructure
% }

There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019TowardPT, Meeder2017AutonomousVP, Acheampong2021-ql}. Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.

% \hauke
% { 
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …
% }

People who try to design policies, AVs, and urban infrastructure together lack methods to do so \cite{Rouse2021-ph}; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
 
Cities are governed by complex rules that were established over long periods of time; AV design methods, however, do not include the design of policies and infrastructure, testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}. Simulations focus on AV behavior only, with often very simple road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}. Simulator environments used for training of AVs, have flexibility in infrastructure and policy re-development, but do not do so \citetodo{}.   
%  Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}.  

Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.  \citet{Yang2019-nr} recognize the lack of any analysis-design-evaluation decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

% \hauke
% {
% As a result, tensions (e.g., tensions between AVs as commercial products versus AVs as public infrastructure) are discussed, but never resolved.
% }

As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.

A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}, and there is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

\subsubsection{Emergent Technologies}
Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 
\newpara
% This paragraph: Prior work did X, did not do Y.
% \placeholder{Overall, we know <overarching goal> is important (AV-enhanced cities, more sustainable...).}

Toward this goal, prior work proposed many isolated methods that combine one or two of these complexities. However, no method can anticipate how opportunities and breakdowns/tensions might emerge from the interactions across urban infrastructure, AVs, and policy. This work attempts to fill this gap.

\section{Research Method}

% This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
\placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}


Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores the potential design-related problems that could arise from the deployment of autonomous vehicles without adequate methods and tools for integrated policy and city design. 

The initial research question guiding this work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this we ventured into diverse fields and research areas including transportation science, urban studies, city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, philosophy, and participatory design. 
The analysis of the contributing literature, particularly in AV technology and infrastructure, the potential impact of AVs on transportation efficiency, equity, and sustainability, and the role of policy in regulating the deployment of AVs, revealed many open problems and the desire for more open and interdisciplinary collaboration. 

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 



\section{Proposition}
\hauke{Feed the examples one by one (rather than copmplexity all at once)
Write the example you want to communicate and rework back}

AVs are like micromobility and trains simultaneously

% Finding/Your proposition (“What do you argue and what’s the evidence?”)
% Findings/Our proposition: 1.5 pages

% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?

\subsubsection{What is novel about AVs in terms of planning complexity?}
- AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
- AVs rollout can act slowly over time, or spontaneously all at once. 
- AV rollout can occur in individual locations, or everywhere all at once. 

- AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  


\subsection{Proposals of Methods that do AV+city+policy together}
\placeholder{We identify two promising approaches that can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy.}

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulation tools, specifically created for policymaking city officials, are required to project how urban infrastructure, AV behavior and AV policy interact. 
% economics of designing livable cities and distributing costs between individuals and AV providers.
We argue that simulators are necessary because only they allow for the evaluation and optimization of transportation policies in a safe, controlled, and cost-effective environment, without having to conduct expensive real-world experiments, and before building infrastructure. This provided insights that would not be available through traditional analysis, making them the best way to prototype and evaluate new transportation policies.

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV simulation. 



% This paragraph: Why can it reveal opportunities? 

With holistic approaches to simulation of AVs, urban infrastructure and implement policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look like in reality.

% This paragraph: Why can it identify challenges?

Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 


\subsubsection{Multi-Goal Optimization}


% This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
% This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.

Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a lower level. 
Multi-goal-optimization can become a helpful tool for such as some, i.e, cities livability, cannot be reduced to individual metrics such as road efficiency. Bayesian optimization, which can help policymakers to evaluate the effects of different policies on multiple objectives such as travel time, energy use, and environmental impact, seems to be a promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 



% \subsubsection{An Example}


\subsection{Open Research Questions that Need to be Answered Before These Methods Become Useful}

\qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
\placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 







\section{Discussion}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. \hauke{Summary of final reasons from propsition here}
%, as it allows for the most flexibility and consolidation. 

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. 

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote integrated approaches, specialized field expertise is necessary, we do not see such an AV policy infrastructure simulator as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v3.tex <==
\section{Introduction}
% Title+ abstract + Introduction: 1 1/3 page


% This paragraph: Describe the great promises of AVs + cities + policies working together. Subtext: Why, despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 

% This paragraph: What prior work has done in realizing the promises, what is still lacking, and why that's not good.
While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not  optimally prepare urban infrastructure and policies for the arrival of AVs. 

% This paragraph: This paper's contribution in realizing the great promises.
In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. With \textit{policies}, we refer to both transportation policies and traffic laws. With urban infrastructure, we refer to transport infrastructure such as roadway features  traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. %zoning? Would be part of urban planning if we go to that category of urban zoning we would say AVs do not incorporate possibilites of urban planning... 
The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 







\section{Related Work}
%Related Work (“What do other people think so far”?)
% RW: ½ leaf


% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
\qian{This paragraph: Examples of why coordination is needed.}
For example, without policy intervention, it is likely that vehicle activity will increase overall due to the convenience of AVs over mass transport~\cite{Soteropoulos2019-tw}.
To fully realize the promised benefits of AVs, it is crucial to implement AV-specific policies, such as ensuring a minimum number of accessible AVs; On the other hand, in order to mitigate the potential negative impacts of AVs, policies must be put in place that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}. 
In order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, National_Association_of_City_Transportation_Officials2019-ll}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}

\qian{This paragraph: However, it's unclear how these things should be coordinated and what policies, city design choices are involved. In the remainder of this section, we will review....}

\input{fig_rw_interactions}

\vspace{3pt}\noindent
\textbf{The designs of vehicles, urban design, and policies inherently impact each other.~}
\qian{This paragraph: Introduce the components: traffic policy, transportation policy, AV motion design, AV service design.}
\
With \textit{policies}, we refer to both transportation policies and traffic laws. With urban infrastructure, we refer to transport infrastructure such as roadway features  traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. %zoning? Would be part of urban planning if we go to that category of urban zoning we would say AVs do not incorporate possibilites of urban planning... 

\qian{This paragraph: Explain how they are interconnected. }
\placeholder{Traffic policy and motion design are inherently... transportation policy and service design... These policies restrict what AV designs are possible; but also are subject to changes... All of these are based upon urban/infra design; can ask for change, but cannot change too fast. All of these operate in the backdrop of civil rights laws.}
Figure~\ref{fig:interactions}

\qian{This paragraph: These interconnections makes coordination necessary in improving cities more difficult. AV for accessibility as an example -- need to consider many variables.}
\placeholder{e.g., to realize the promise of a new AV service design - accessible AVs, one needs to update city infra (e.g., accessible lanes, parking space), might need to update AV motion design as well, considerations of potential traffic regulations (similar to school bus stop laws), }
Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}

\qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
\placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

\qian{This paragraph: As a result, people call for coordination among agencies.}
While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{National_Association_of_City_Transportation_Officials2019-ll}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  

\vspace{3pt}\noindent
\textbf{Common methods for designing AVs, cities, or policies rarely support the coordination among them.}
\qian{This paragraph: Existing methods often consider either AVs or cities or policies.}
People who try to design policies, AVs, and urban infrastructure together lack methods to do so \cite{Rouse2021-ph}; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
Cities are governed by complex rules that were established over long periods of time; AV design methods, however, do not include the design of policies and infrastructure, testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}. Simulations focus on AV behavior only, with often very simple road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}. Simulator environments used for training of AVs, have flexibility in infrastructure and policy re-development, but do not do so \citetodo{}.   
Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.  \citet{Yang2019-nr} recognize the lack of any analysis-design-evaluation decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.
%  Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}.  

% Tactical design \cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}
% Design patterns and guides for infrastructure \cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}
% multiple Wendys wizard of oz methods for AVs \cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}
% VR motion design \cite{Goedicke2022-ys}

\qian{This paragraph: Different agencies optimize for different goals.}
These hard choices need to be made in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019TowardPT, Meeder2017AutonomousVP, Acheampong2021-ql}. 


\qian{This paragraph: Different goals reflect different social values, suggesting that optimal solutions that achieve these individual goals are unknowingly in conflict. They cannot be easily combined.}
Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
social dilemmas, 
Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.
% \hauke
% { 
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …

\vspace{3pt}\noindent
\textbf{Emergent research started simultaneously designing some combinations of AVs, cities, and policies.~}
Toward this goal, prior work proposed many isolated methods that combine one or two of these complexities. 
\qian{This paragraph: People have started designing policy and cities together}
A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 

% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 

\qian{This paragraph: people have *proposed* designing road infra and AVs together. 
If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

\qian{This paragraph: However, no work did three all togehter.}
However, no method can anticipate how opportunities and breakdowns/tensions might emerge from the interactions across urban infrastructure, AVs, and policy. This work attempts to fill this gap.



\section{Research Method}

% This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
% \placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}

Our goal is to investigate what methods can bridge AVs, urban and rural design, as well as policy making.
In order to understand the potential design-related problems as well as opportunities that could emerge from the interactions across these, we conducted a comprehensive literature review.
% Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores 

The initial research question guiding this review work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this, we ventured into diverse fields and research areas including transportation science, urban studies, city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, philosophy, and participatory design. 
The analysis of the contributing literature revealed a strong grade of specialization into subfields with desire for interdisciplinary collaboration. 
In the next section we synthesize the conclusions drawn from open problems mentioned in the literature, particularly related to those with relationship to AV Design, such as technology and infrastructure, the impact of AVs on transportation, as well as the role of policy in regulating the deployment of AVs.

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 



\section{Proposition}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}

% AVs are like micromobility and trains simultaneously

% Finding/Your proposition (“What do you argue and what’s the evidence?”)
% Findings/Our proposition: 1.5 pages

% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?

\subsubsection{What is novel about AVs in terms of planning complexity?}

% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }

Autonomous vehicles represent a new frontier in urban and rural planning complexity. In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  

In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 




\subsection{Proposals of Methods that do AV+city+policy together}

Current scope limited AV tests, complimentary simulation studies and analysis of human natural driving are unlike the effects AVs will present at scale. They also do not consider opportunistic re-design of the urban/rural infrastructure.  

We identify three promising approaches that can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulation tools, specifically created for policymaking city officials, are the only known methods capable of projecting how urban infrastructure, AV behavior and AV policy interact in the future. 
% economics of designing livable cities and distributing costs between individuals and AV providers.
We argue that simulators are necessary because only they allow for the evaluation and optimization of transportation policies in a safe, controlled, and cost-effective environment, without having to conduct expensive real-world experiments, and before building infrastructure. This provided insights that would not be available through traditional analysis, making them one of the best ways to prototype and evaluate new AV transportation as well as traffic policies. 

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV 
% This paragraph: Why can it reveal opportunities? 
With holistic approaches to simulation of AVs, urban infrastructure and policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look like in reality. Shared mobility services allowed to collect some pre-AV-deployment insights to AV service design and policy. The interdependencies of AV motion design, infrastructure design are of higher urgency as they are less researched. 

% This paragraph: Why can it identify challenges?

% Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 

\subsubsection{Multi-Goal Optimization}
In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These goals relate to the current problems. 

AV motion design predominately tries to solve the safety of AVs. Achieving  better than human levels of safety is the most pressing goal to turn AVs into a reality. Simulation work in traffic regulations, addresses predominately questions of optimizing road networks efficiency, i.e., its throughput without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Policy research in transportation regulations nowadays primarily addresses sustainability. AV service design the highest goal is optimization of the efficient use of all AVs, i.e., minimizing idle time. Between these 5 areas, urban rural infrastructure design is the only are that needs to satisfy all goals at once. The prioritization has changed throughout the years, nowadays, research focus shifted, particularly in the U.S., to improving livability. Safety, efficiency have always been of importance, but so are equity and sustainability. 

AVs need to satisfy all these goals, to deliver upon their promise. 
% This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
% This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.
 
Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a fine-grained level. 
Some multi-goal-optimization limitations are resolved meanwhile, and therefore it can become a tool for policy optimization. A few examples of bayesian multi goal traffic optimization, are promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 

\subsubsection{Primitive AV/policy/infrastructure prototyping}
Many citizen needs cannot be understood through simulations and optimization. We suggest adopting rising participatory design methods in urban planning for AV planning. Testing urban prototypes with members of the public and guerilla style action of individuals have successfully reshaped urban room in many cities. \citetodo{}  These methods are grouped under the category tactical urbanism. Tactical urbanism offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. We suggest that policymakers, and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. 

% \subsubsection{An Example}

\subsection{Requirement: Open Data and Simulators}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. 


% \qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
% \placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% % The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
% Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
% Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
% Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 







\section{Discussion}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. \hauke{Summary of final reasons from propsition here}
%, as it allows for the most flexibility and consolidation. 

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. 

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote integrated approaches, specialized field expertise is necessary, we do not see such an AV policy infrastructure simulator as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v4.tex <==
\section{Introduction}
% Title+ abstract + Introduction: 1 1/3 page


% This paragraph: The great promises of AVs + AV services = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Autonomous Vehicles (AVs) promise many societal benefits that are impossible to realize otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce car crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
AV ride-sharing services can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighbourhoods~\cite{Gilbert-Sociotechnical}. 
By coordinating with each other and with smart city infrastructure, AVs can reduce congestion and cruising-for-parking, thereby decreasing vehicle emissions~\cite{Rojas-Rueda2017-xl}.
Taken together, AVs appear to have the potential to catalyze safer, more accessible, more sustainable, and more livable cities.

% Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 
% AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}. Commonly, mentioned benefits are reduced traffic accidents, decrease in vehicle emissions and congestion, improved safety for pedestrians and cyclists, better mobility for the elderly and disabled, increase in active travel, as well as reduced need for parking space. 


% This paragraph: Realizing these promises requires AV motion+service designs to coordinate with city design and policies. They currently are not. 
Realizing these promises, however, requires careful coordination among AV driving behaviors, city infrastructure, and related regulations at various levels~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019TowardPT, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Even making AVs available to the public involves complex policy questions (e.g., liability, privacy, and insurance)~\cite{fagnant2015preparing} and requires nontrivial infrastructural changes (e.g., allocating lanes for autonomous food-delivery robots~\cite{food-delivery-robot-bikelane-wired}).
% not to mention creating safer, more equal, more livable, or more sustainable cities through AV design.

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.

Coordinating AV, policy, and city infrastructure is not just complex; It requires designers to confront the three-way chick-and-egg relationship among driving behaviors, policies, and city design~\cite{Gilbert-Sociotechnical,Wu2018-oy}:
When designing AV driving behaviors, should AV designers consider city infrastructure and traffic policies as given constraints, or additional levels they can pull to improve safety?
When designing traffic rules and streets, should urban planners and policymakers consider various AVs' motion-planning algorithms static and homogeneous or embrace their complexities as well?
Many researchers have expounded on the necessity of considering AV, city, and policy designs simultaneously~\citetodo{}. Few, however, have the know-how to handle all these complexities at once. 
% To date, it remains unclear what methodologies or workflows can help coordinate AV, city, and policy designs, in order to realize AVs' promises for better cities.
% Qian: might move this example to RW. Too long. %(for example, rather than paintakingly improving Computer Vision algorithms that can recognize various road signs in different weathers and view blocks, they might designing new road signs that are easily recognizable by both Computer Vision algorithms and naked eyes~\cite{Gilbert-Sociotechnical})
% (e.g., sensors, signs of pedestrian crossings) 
% take into account, for example, the different driving behaviors of AVs from different companies, as they design cities and set traffic rules?

% As a result, AV designers often treated existing city infrastructure and policies as fixed constraints, even though they can change somewhat frequently and easily~\citetodo{}.
% Urban designers and policymakers have started envisioning AV-ready city infrastructure and regulations. Yet these designs rarely considered, for example, how the different driving behaviors of AVs from different companies might create unexpected broader impacts and new regulatory needs~\citetodo{}. % Cite https://www.restreet.com/ and other related work.


% This paragraph: This paper's contribution in realizing these great promises.
We wanted to understand better how the designs of AV driving behaviors, smart city infrastructure, and policies might coordinate and together shape safer, more accessible, and more sustainable cities.
\textbf{Towards this goal, this paper first delineates the entangled relationships among AV, urban, and policy\footnote{This paper focuses mostly on US law and policies. This is a limitation of this work.} design decisions}, based on a comprehensive literature synthesis across the fields of human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, philosophy, and social sciences. % This is good! a great list.
In doing so, we highlight the benefits and, sometimes, the \textit{necessity} of simultaneously designing AV behaviors, AV services, city infrastructure, and policies~(chapter~\ref{sec:rw}).

\textbf{Next, we explore methods that might make such simultaneous design and prototyping possible}~(chapter~\ref{sec:proposition}).
\placeholder{map out the existing methods used in AV, city, and policy design. We demonstrate that these methods in these design tasks are isolated. We identify opportunities for integrating them.... e.g., \newmethodlong (\newmethod)}\qian{Will come back to this.}
Through this work, we hope to invite a more principled discussion around, not just whether, but \textit{how} AV designers, urban planners, and policymakers can work together to form better future smart cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Arguing for Designing AV Behaviors, Cities, and Policies Simultaneously}\label{sec:rw}
%Related Work (“What do other people think so far”?)
% RW: ½ leaf


% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
\qian{This paragraph: Examples of why coordination is needed.}
\placeholder{Empirical reserach} has shown that, without policy intervention, it is likely that vehicle activity will increase overall due to the convenience of AVs over mass transport~\cite{Soteropoulos2019-tw}.
To fully realize the promised benefits of AVs, it is crucial to implement AV-specific policies, such as ensuring a minimum number of accessible AVs; On the other hand, in order to mitigate the potential negative impacts of AVs, policies must be put in place that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}. 
In order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}

\qian{This paragraph: However, it's less clear how these things should be coordinated and what policies, city design choices are involved. Here we review....}

\input{fig_rw_interactions}

\vspace{3pt}\noindent
\textbf{The designs of vehicles, urban design, and policies inherently impact each other.~}
\qian{This paragraph: Introduce the components: traffic policy, transportation policy, AV motion design, AV service design.}
\
With \textit{policies}, we refer to both transportation policies and traffic laws. With urban infrastructure, we refer to transport infrastructure such as roadway features  traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. %zoning? Would be part of urban planning if we go to that category of urban zoning we would say AVs do not incorporate possibilites of urban planning... 

\subsubsection{What is novel about AVs in terms of planning complexity?}
Autonomous vehicles represent a new frontier in urban and rural planning complexity. In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  

In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

\qian{This paragraph: Explain how they are interconnected. }
\placeholder{Traffic policy and motion design are inherently... transportation policy and service design... These policies restrict what AV designs are possible; but also are subject to changes... All of these are based upon urban/infra design; can ask for change, but cannot change too fast. All of these operate in the backdrop of civil rights laws.}
Figure~\ref{fig:interactions}

\qian{This paragraph: These interconnections make coordination necessary in improving cities more difficult. AV for accessibility as an example -- need to consider many variables.}
\placeholder{e.g., to realize the promise of a new AV service design - accessible AVs, one needs to update city infra (e.g., accessible lanes, parking space), might need to update AV motion design as well, considerations of potential traffic regulations (similar to school bus stop laws), }
Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}

\qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
\placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

\qian{This paragraph: As a result, people call for coordination among agencies.}
While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  



% \section{Research Method}

% % This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
% % \placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}

% Our goal is to investigate what methods can bridge AVs, urban and rural design, as well as policy making.
% In order to understand the potential design-related problems as well as opportunities that could emerge from the interactions across these, we conducted a comprehensive literature review.
% % Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores 

% The initial research question guiding this review work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this, we ventured into diverse fields human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, philosophy, and social sciences; and research areas city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, AV ethics, and participatory design. \hauke{seperated fields and research areas}
% The analysis of the contributing literature revealed a strong grade of specialization into subfields with desire for interdisciplinary collaboration. 
% In the next section we synthesize the conclusions drawn from open problems mentioned in the literature, particularly related to those with relationship to AV Design, such as technology and infrastructure, the impact of AVs on transportation, as well as the role of policy in regulating the deployment of AVs.

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 

\section{Exploring Methods for Designing AV Behaviors, Cities, and Policies Simultaneously}\label{sec:proposition}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}

% AVs are like micromobility and trains simultaneously

% Finding/Your proposition (“What do you argue and what’s the evidence?”)
% Findings/Our proposition: 1.5 pages

% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?



% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }


% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 


\vspace{3pt}\noindent
\textbf{Common methods for designing AVs, cities, or policies rarely support the coordination among them.}
\qian{This paragraph: Existing methods often consider either AVs or cities or policies.}
People who try to design policies, AVs, and urban infrastructure together lack methods to do so \cite{Rouse2021-ph}; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
Cities are governed by complex rules that were established over long periods of time; AV design methods, however, do not include the design of policies and infrastructure, testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}. Simulations focus on AV behavior only, with often very simple road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}. 3D Simulator environments used for training of AVs~\cite{Dosovitskiy2017, NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp}, could be extended for flexibility in infrastructure and policy re-development~\cite{Haegler2021-xv}, but to our knowledge have never been. Instead, city planning is done with low-detail maps or street cross-profiles~\cite{Riggs2017-hm, Lee2022-vd, Remix_by_Via2021-vm}. 
Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.  \citet{Yang2019-nr} recognize the lack of any analysis-design-evaluation decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.
%  Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}.  
\placeholder{Tactical design \cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}
Design patterns and guides for infrastructure \cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}
multiple Wendys wizard of oz methods for AVs \cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}
VR motion design \cite{Goedicke2022-ys}}

\input{fig_rw_methods}

\qian{This paragraph: Different agencies optimize for different goals.}
Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019TowardPT, Meeder2017AutonomousVP, Acheampong2021-ql}. 


\qian{This paragraph: Different goals reflect different social values, suggesting that optimal solutions that achieve these individual goals are unknowingly in conflict. They cannot be easily combined.}
Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
social dilemmas, 
Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.
% \hauke
% { 
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …

\vspace{3pt}\noindent
\textbf{Emergent research started simultaneously designing some combinations of AVs, cities, and policies.~}
Toward this goal, prior work proposed many isolated methods that combine one or two of these complexities. 
\qian{This paragraph: People have started designing policy and cities together}
A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 

% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 

\qian{This paragraph: people have *proposed* designing road infra and AVs together. }
If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

\qian{This paragraph: However, no work did three all together.}
However, no method can anticipate how opportunities and breakdowns/tensions might emerge from the interactions across urban infrastructure, AVs, and policy. This work attempts to fill this gap.



\subsection{Proposals of Methods that do AV+city+policy together}

Current scope limited AV tests, complementary simulation studies, and analysis of natural human driving are unlike the effects AVs will present at scale. They also do not consider opportunistic re-design of the urban/rural infrastructure.  

We identify three promising approaches that can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulation tools, specifically created for policymaking city officials, are the only known methods capable of projecting how urban infrastructure, AV behavior and AV policy interact in the future. 
% economics of designing livable cities and distributing costs between individuals and AV providers.
We argue that simulators are necessary because only they allow for the evaluation and optimization of transportation policies in a safe, controlled, and cost-effective environment, without having to conduct expensive real-world experiments, and before building infrastructure. This provided insights that would not be available through traditional analysis, making them one of the best ways to prototype and evaluate new AV transportation as well as traffic policies. 

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV 
% This paragraph: Why can it reveal opportunities? 
With holistic approaches to the simulation of AVs, urban infrastructure, and policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look in reality. Shared mobility services allowed to collect some pre-AV-deployment insights to AV service design and policy. The interdependencies of AV motion design, and infrastructure design are of higher urgency as they are less researched. 

% This paragraph: Why can it identify challenges?

% Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 

\subsubsection{Multi-Goal Optimization}
In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These goals relate to the current problems. 

AV motion design predominately tries to solve the safety of AVs. Achieving  better than human levels of safety is the most pressing goal to turn AVs into a reality. Simulation work in traffic regulations, addresses predominately questions of optimizing road networks efficiency, i.e., its throughput without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Policy research in transportation regulations nowadays primarily addresses sustainability. AV service design the highest goal is optimization of the efficient use of all AVs, i.e., minimizing idle time. Between these 5 areas, urban rural infrastructure design is the only are that needs to satisfy all goals at once. The prioritization has changed throughout the years, nowadays, research focus shifted, particularly in the U.S., to improving livability. Safety, efficiency have always been of importance, but so are equity and sustainability. 

AVs need to satisfy all these goals, to deliver upon their promise. 
% This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
% This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.
 
Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a fine-grained level. 
Some multi-goal-optimization limitations are resolved meanwhile, and therefore it can become a tool for policy optimization. A few examples of bayesian multi goal traffic optimization, are promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 

\subsubsection{Primitive AV/policy/infrastructure prototyping}
\hauke{Could go to related work}\placeholder{Many citizen needs cannot be understood through simulations and optimization. We suggest adopting rising participatory design methods in urban planning for AV planning. Testing urban prototypes with members of the public and guerilla style action of individuals have successfully reshaped urban room in many cities \citetodo{}. These methods are grouped under the category of tactical urbanism.} Tactical urbanism offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. 

% \subsubsection{An Example}

\subsection{Requirement: Open Data and Simulators}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. 


% \qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
% \placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% % The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
% Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
% Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
% Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 







\section{Discussion}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. \hauke{Summary of final reasons from propsition here}
%, as it allows for the most flexibility and consolidation. 

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. 

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote integrated approaches, specialized field expertise is necessary, we do not see such an AV policy infrastructure simulator as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v5.tex <==
\section{Introduction}
% Title+  Introduction: 1 page


% This paragraph: The great promises of AVs + AV services = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Autonomous Vehicles (AVs) promise many societal benefits that are impossible to realize otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce car crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
AV ride-sharing services can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighbourhoods~\cite{Gilbert-Sociotechnical}. 
By coordinating with each other and with smart city infrastructure, AVs can also reduce congestion and cruising-for-parking, thereby decreasing vehicle emissions~\cite{Rojas-Rueda2017-xl}.

% Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 
% AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}. Commonly, mentioned benefits are reduced traffic accidents, decrease in vehicle emissions and congestion, improved safety for pedestrians and cyclists, better mobility for the elderly and disabled, increase in active travel, as well as reduced need for parking space. 


% This paragraph: Realizing these promises requires AV motion+service designs to coordinate with city design and policies. They currently are not. 
Yet AVs' societal benefits are far from guaranteed; Realizing them requires careful coordination among AV driving behavior design, city infrastructure, and various related regulations~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019-gn, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Just making AVs available to the public involves complex policy questions (e.g., liability, privacy, and insurance)~\cite{fagnant2015preparing} and requires potential city-scale infrastructural changes (e.g., allocating lanes for autonomous food-delivery robots~\cite{food-delivery-robot-bikelane-wired});
% \hauke{This example is somehow throwing me off. }
% Why? If you don't like it, feel free to change to a different one.
much more so in making AVs catalysts of safer, more equal, more sustainable, or more livable cities.

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.

% This paragraph: articulate precisely what problems/questions this paper solves 
Coordinating AV, policy, and city designs is not just complex; It requires designers to confront the three-way ``\textit{chick-and-egg}'' relationship among them~\cite{Gilbert-Sociotechnical,Wu2018-oy}.
Changes to any one of them---vehicles' driving patterns, city layout, and policies---must be compatible with the other two to work, yet changes to any one of them also change the other two over time.
In this context, many researchers have argued for considering the three simultaneously~\cite{Matowicki2020-vy, Aoyama2021-jj, Duarte2018-wg, OToole2020-so, Freemark2020-ms, Staricco2019-gn}.
But how?
How can AV designers identify the city infrastructure and policy design choices relevant to their AV driving behavior algorithms? How can urban planners and policymakers identify relevant aspects of AVs' varying and fast-evolving driving behavior algorithms, so that the streets and AV regulations they design can account for them?  % <- Figures 1 and 2 answer these two questions.
What methods and tools can help AV designers, urban planners, and policymakers work together and coordinate their designs? % <- Our new method answers this question.
This paper explores these questions.

% Yet few have the know-how to handle all these complexities at once. 
% To date, it remains unclear what methodologies or workflows can help coordinate AV, city, and policy designs, in order to realize AVs' promises for better cities.
% Qian: might move this example to RW. Too long. %(for example, rather than paintakingly improving Computer Vision algorithms that can recognize various road signs in different weathers and view blocks, they might designing new road signs that are easily recognizable by both Computer Vision algorithms and naked eyes~\cite{Gilbert-Sociotechnical})
% (e.g., sensors, signs of pedestrian crossings) 
% take into account, for example, the different driving behaviors of AVs from different companies, as they design cities and set traffic rules?

% As a result, AV designers often treated existing city infrastructure and policies as fixed constraints, even though they can change somewhat frequently and easily~\citetodo{}.
% Urban designers and policymakers have started envisioning AV-ready city infrastructure and regulations. Yet these designs rarely considered, for example, how the different driving behaviors of AVs from different companies might create unexpected broader impacts and new regulatory needs~\citetodo{}. % Cite https://www.restreet.com/ and other related work.


% This paragraph: This paper's contribution in realizing these great promises.
We wanted to understand how the designs of AVs, cities, and various policies might coordinate and together shape safer, more accessible, and more sustainable cities. Towards this goal, \textbf{this paper first maps the entangled relationships among AV, city, and policy design decisions} based on a comprehensive literature synthesis across the fields of human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, and philosophy. %<- chapter 2.1
%, and the social sciences. % The social sciences is not one field. It's many.
This mapping helps those who aspire to shape AV-infused future cities to identify relevant design issues across the traditional ``\textit{AV design}'', ``\textit{urban planning}'', and ``\textit{legal and policy design}'' boundaries.%<- chapter 2.2
% In doing so, we highlight the benefits and, sometimes, the \textit{necessity} of simultaneously designing AV behaviors, AV services, city infrastructure, and policies~(chapter~\ref{sec:rw}).

\textbf{Next, we explore methods that could bridge these design choices}, allowing AV, city, and policy designers prototype their designs simultaneously and observe their broader impacts. % Chapter 3.
We envision a new approach, namely ``\textit{\newmethodlong}'' (\newmethod), as an initial step in addressing the methodological barriers of designing AVs, cities, and policies simultaneously
We invite a more principled discussion around, not just whether, but \textit{how} AV designers, urban planners, and policymakers should work together to shape future smart cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Mapping AV, City, and Policy Design Choices}\label{sec:rw}
% This chapter is entirely Related Work (“What do other people think so far”?).
% Our contribution is merely organizing related work.
% Length budget: 2 pages of texts + 1 figure.


% This paragraph: AV, city, policy designs needs coordination, because any driving behavior, city, and policy designs need coordination. The components are the same.
 \input{fig_rw_interactions}
\vspace{3pt}\noindent
\textbf{The design choices around AV movement, AV services, city infrastructure, and policies are inherently interrelated.~}
Their connections echo the inherent connections among any vehicle's driving behaviors, services, city infrastructure, and policies. Figure~\ref{fig:interactions} maps out these relationships.
From top to bottom: \textit{Civil rights laws and policies}\footnote{This paper focuses mainly on US law and policies. This is a limitation of this work.} set rules that apply to all players in transportation. For example, they require car companies and their designs to allow free sharing of car-repair-related data~\citetodo{https://www.theverge.com/2020/11/4/21549129/massachusetts-right-to-repair-question-1-wireless-car-data-passes}; they mandate that cities have certain amount of accessible parking and ride-sharing services have certain amount of accessible vehicles~\citetodo{https://adata.org/factsheet/ADA-accessible-transportation}. 
\textit{Traffic regulations} instruct how vehicles and people should move (e.g., that all vehicles should yield to blind pedestrians and stop for school buses), % e.g., pedestrians law, school bus stopping law, clean ice and snow, yield to blind pedestrians, etc.
while \textit{transportation regulations} set rules and incentives related to road use and vehicle use (e.g., authorizing protected planes for bikes and scooters~\citetodo{https://t4america.org/2022/02/23/the-new-infrastructure-law-micromobility/}.) % e.g., safety and accidents, auto insurance law, highway law, accessible parking mandates, electric vehicle subsidies, micromobility vehicle laws (e.g., protected lanes for scooters and bikers).
Within these legal and regulatory bounds (red arrows in Fig~\ref{fig:interactions}), AV designers design algorithms to instruct how their AVs move in relation to city infrastructure and other actor on the road (\textit{AV motion design}); AV service designers create additional rules and incentives related to such movements (e.g., via dynamic pricing~\citetodo{}).
Good designs and services, after proven effective, could change transport infrastructure and even become policy mandates (green arrows in Fig~\ref{fig:interactions}, e.g., the wide adoption of ride-hailing services led to dedicated guest boarding zones at airports).
% With urban infrastructure, we refer to transport infrastructure such as roadway features and traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. 

This map makes it evident that realizing AVs' societal benefits \textit{requires} the coordination among AV, city, and policy designs. 
Empirical evidence from small-scale AV trials and large-scale traffic simulations agree~\cite{Soteropoulos2019-tw,Sperling2018-vk, Freemark2020-ms, Nacto2019-pe,Riggs2019-lx, Niroumand2023-an,Staricco2019-gn,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
For example, reducing congestion requires not only efficient AV navigation algorithms, but AV services, policies, and city infrastructure that incentivize shared rather than personally-owned AVs~\citetodo{}.
Making future cities more accessible to people with mobility disabilities needs more than accessible AVs.
Incorporating accessible AVs into public transport services can radically scale up AV's accessibility benefits, while corresponding laws and policies could help minimize risks (e.g., by mandating blind driver boarding zones.)~\citetodo{}
% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
% According to a review study on AV modelling work, in the absence of policy intervention, the use of autonomous vehicles is likely to increase overall as they offer greater convenience over mass transportation~\cite{Soteropoulos2019-tw}.
% To fully realize the promised benefits of AVs, it is, therefore, crucial to implement AV-specific policies. Literature has suggested policies to mitigate the potential negative impacts of AVs, that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}, and promoting benefits such as ensuring a minimum number of accessible AVs. 
% Further, in order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}

 % (e.g., when AVs stop or accelerate)
  % (e.g., AV ride-sharing)
   % (e.g., road signs, public cameras and sensors)
   % s (e.g., how pedestrians are supposed to move) 
    % (e.g., when drivers stop or accelerate)
    % (ride-sharing)


\vspace{3pt}\noindent
\textbf{Different regulations and components of city infrastructure impact different types of AVs.~}
So far, we have treated AVs as one type of vehicle. Yet AVs are far from homogeneous (Think autonomous long-haul trucks, autonomous commercial drivers' vehicles, autonomous scooters for last-mile transportation, and food delivery robots.) Therefore, they will likely achieve wide adoption at different times, use different parts of the city infrastructure, and operate under different traffic and transportation regulations (e.g., AV scooters will likely be subject to micro-mobility laws, while low-haul trucks will be to Hours of Service regulations in the U.S.)
In this sense, the wide variety of future AVs will add further complexities to the already complex AV-city-policy design landscape.
% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }
% AVs are like micromobility and trains simultaneously
% \subsubsection{What is novel about AVs in terms of planning complexity?}
% Autonomous vehicles represent a new frontier in urban and rural planning complexity.
% In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
% Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
% Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  
% In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% \section{Research Method}

% % This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
% % \placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}

% Our goal is to investigate what methods can bridge AVs, urban and rural design, as well as policy making.
% In order to understand the potential design-related problems as well as opportunities that could emerge from the interactions across these, we conducted a comprehensive literature review.
% % Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores 

% The initial research question guiding this review work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this, we ventured into diverse fields human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, philosophy, and social sciences; and research areas city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, AV ethics, and participatory design. \hauke{seperated fields and research areas}
% The analysis of the contributing literature revealed a strong grade of specialization into subfields with desire for interdisciplinary collaboration. 
% In the next section we synthesize the conclusions drawn from open problems mentioned in the literature, particularly related to those with relationship to AV Design, such as technology and infrastructure, the impact of AVs on transportation, as well as the role of policy in regulating the deployment of AVs.

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 

\section{Exploring Methods for Designing AVs, Cities, and Policies Simultaneously}\label{sec:proposition}
% This chapter is half Related Work (existing methods) and half our new ideas/contributions (iCAP-- “What do you argue and what’s the evidence?”)
% Length budget: 2 pages of texts + 1 figure.

\subsection{Common Methods Used In Current Practice}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}


% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?






% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 


%%%%% =====  stuff moved from chatper 2 to here START ====== %%%%
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }
% \qian{trade-offs across multiple goals}
% Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}
% \qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
% \placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
% most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
% Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
% Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

% \qian{This paragraph: As a result, people call for coordination among agencies.}
% While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  
%%%%% =====  Stuff moved from chatper 2 to here END ====== %%%%


% This paragraph: Current methods are isolated. Give examples.
The common methods used in today's AV, city, or policy design rarely support the coordination among them.
People who try to design policies, AVs, and urban infrastructure together lack methods to do so \cite{Rouse2021-ph}; therefore they mostly work separately. Their methods exclude other moving parts’ complexity.
While cities are governed by complex rules established over long periods, AV design methods do not include policy and infrastructure design.  Testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}. Due to the limitations of technical AV testing, researchers devised Wizard of Oz methods for human-AV experiments on real roads~\cite {Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}.  Many simulations focus on AV behavior only, with often basic road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}, due to limitations researchers devised VR simulators~\cite{Goedicke2022-ys}. These research methods incorporate human considerations, but not policy or infrastructure. 
3D Simulator environments used for training of AVs~\cite{Dosovitskiy2017-jb, NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp}, could be extended for flexibility in infrastructure and policy re-development~\cite{Haegler2021-xv}, but to our knowledge have never been. Instead, city planning is done with low-detail maps or street cross-profiles~\cite{Riggs2017-hm, Lee2022-vd, Remix_by_Via2021-vm}. For infrastructure design, guidelines, and design patterns were established over time~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. These demand an update with specific AV patterns~\cite{Nacto2019-pe}.  
Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}. Participatory design methods are used in multiple areas to understand people's needs, in urban planning, tactical urbanism, citizen-led prototyping is becoming popular and shows unsatisfied needs by conventional planning~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}. Tactical urbanism has informed policymaking, but not AV design.
As \citet{Yang2019-nr} note, there is a lack of decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

%\citet{Yang2019-nr} recognize the lack of any analysis-design-evaluation decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior. \hauke{methods for integrated design of transport infrastructure and public spaces with consideration of human behavior.enough?}
%  Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}.  

\input{fig_rw_methods}

% This paragraph: These methods can lead to results that are difficult to synthesize, because (1) they work under different assumptions and at different levels of granularity.

Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
social dilemmas, 
Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.
% hauke:
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …

% This paragraph: These methods can lead to results that are difficult to synthesize, because (2) they optimize toward different goals.
\qian{This paragraph: Different agencies optimize for different goals.}
Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019-gn, Meeder2017AutonomousVP, Acheampong2021-ql}. 


\subsection{Emergent Research: Simultaneously Designing Some Combinations of AVs, Cities, and Policies}
Toward this goal, prior work proposed many isolated methods that combine one or two of these complexities.

% This paragraph: People have started designing policy and cities together
\vspace{3pt}\noindent
\textbf{Designing Smart City and Policies Simultaneously.~}
A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 

% This paragraph: people have *proposed* designing road infra and AVs together.
\vspace{3pt}\noindent
\textbf{Designing AV and Smart City Simultaneously.~}If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

 



% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 


\qian{This paragraph: However, no work did three all together.}
However, no method can anticipate how opportunities and breakdowns/tensions might emerge from the interactions across urban infrastructure, AVs, and policy. This work attempts to fill this gap.



\subsection{Our Proposal: Integrative City-AV-Policy Simulation (iCAPS)}

% Prototyping AV Motion, City, and Policy Designs Simultaneously in Low-Fidelity using Simulations
Current scope limited AV tests, complementary simulation studies, and analysis of natural human driving are unlike the effects AVs will present at scale. They also do not consider opportunistic re-design of the urban/rural infrastructure.  

We identify three promising approaches that can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulation tools, specifically created for policymaking city officials, are the only known methods capable of projecting how urban infrastructure, AV behavior and AV policy interact in the future. 
% economics of designing livable cities and distributing costs between individuals and AV providers.
We argue that simulators are necessary because only they allow for the evaluation and optimization of transportation policies in a safe, controlled, and cost-effective environment, without having to conduct expensive real-world experiments, and before building infrastructure. This provided insights that would not be available through traditional analysis, making them one of the best ways to prototype and evaluate new AV transportation as well as traffic policies. 

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV 
% This paragraph: Why can it reveal opportunities? 
With holistic approaches to the simulation of AVs, urban infrastructure, and policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look in reality. Shared mobility services allowed to collect some pre-AV-deployment insights to AV service design and policy. The interdependencies of AV motion design, and infrastructure design are of higher urgency as they are less researched. 

% This paragraph: Why can it identify challenges?

% Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 

\subsubsection{Multi-Goal Optimization}
In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These goals relate to the current problems. 

AV motion design predominately tries to solve the safety of AVs. Achieving  better than human levels of safety is the most pressing goal to turn AVs into a reality. Simulation work in traffic regulations, addresses predominately questions of optimizing road networks efficiency, i.e., its throughput without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Policy research in transportation regulations nowadays primarily addresses sustainability. AV service design the highest goal is optimization of the efficient use of all AVs, i.e., minimizing idle time. Between these 5 areas, urban rural infrastructure design is the only are that needs to satisfy all goals at once. The prioritization has changed throughout the years, nowadays, research focus shifted, particularly in the U.S., to improving livability. Safety, efficiency have always been of importance, but so are equity and sustainability. 

AVs need to satisfy all these goals, to deliver upon their promise. 
% This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
% This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.
 
Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a fine-grained level. 
Some multi-goal-optimization limitations are resolved meanwhile, and therefore it can become a tool for policy optimization. A few examples of Bayesian multi goal traffic optimization, are promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 

\subsubsection{Primitive AV/policy/infrastructure prototyping}
Many citizen needs cannot be understood through simulations and optimization. We suggest adopting rising participatory design methods in urban planning for AV planning. Testing urban prototypes with members of the public and guerilla style action of individuals have successfully reshaped urban room in many cities \cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew} These methods are grouped under the category of tactical urbanism. Tactical urbanism offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. Further, we see potential to create hybrid methods, using Wizard of Oz to design AV motion and participatory design to design policy all simultaneously. 

% \subsubsection{An Example}

\subsection{Requirement: Open Data and Simulators}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. 


% \qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
% \placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% % The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
% Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
% Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
% Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 







\section{Discussion}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. \hauke{Summary of final reasons from propsition here}
%, as it allows for the most flexibility and consolidation. 

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. 

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote integrated approaches, specialized field expertise is necessary, we do not see such an AV policy infrastructure simulator as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v6.tex <==
\section{Introduction}
% Title+  Introduction: 1 page


% This paragraph: The great promises of AVs + AV services = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Autonomous Vehicles (AVs) promise to improve cities in ways that would not have been possible otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce car crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
AV ride-sharing services can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighborhoods~\cite{Gilbert-Sociotechnical}. 
AVs can also reduce congestion and cruising-for-parking by coordinating with each other and with smart city infrastructure, hence decrease vehicle emissions~\cite{Rojas-Rueda2017-xl}.
These promises of safer, more equal, more sustainable, or more livable cities have long been central considerations in AV design.

% Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 
% AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}. Commonly, mentioned benefits are reduced traffic accidents, decrease in vehicle emissions and congestion, improved safety for pedestrians and cyclists, better mobility for the elderly and disabled, increase in active travel, as well as reduced need for parking space. 


% This paragraph: Realizing these promises requires AV motion+service designs to coordinate with city design and policies. They currently are not. 
Yet AVs' societal benefits are far from guaranteed; Realizing them requires careful coordination among the designs of AVs, city infrastructure, as well as related regulations~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019-gn, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Making AVs available to the public alone involves complex policy questions (e.g., liability, privacy, and insurance)~\cite{fagnant2015preparing} and can entail city-scale infrastructural changes (e.g., should autonomous food-delivery robots use bike lanes or new dedicated lanes?~\cite{food-delivery-robot-bikelane-wired}). Not to mention realizing AVs' more ambitious promises.
% \hauke{This example is somehow throwing me off. }
% Why? If you don't like it, feel free to change to a different one.
% much more so in making AVs catalysts of safer, more equal, more sustainable, or more livable cities.

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.

% This paragraph: articulate precisely what problems/questions this paper solves 
Coordinating AV, policy, and city designs is not just complex; It requires designers to confront the three-way ``\textit{chick-and-egg}'' relationship among them~\cite{Gilbert-Sociotechnical,Wu2018-oy, Brozynski2022-yv}.
Changes to any one of them---AVs' driving patterns, city layout, and traffic and transportation policies---must be compatible with the other two to be practical. However, changes to any of them also change the other two.
Many researchers therefore have argued for considering the three simultaneously~\cite{Matowicki2020-vy, Aoyama2021-jj, Duarte2018-wg, OToole2020-so, Freemark2020-ms, Staricco2019-gn}.
But how?
How can AV designers go beyond simple road scenarios and today's traffic laws when designing AVs for future cities? How can urban planners accommodate AVs' infrastructural needs while mitigating unintended consequences? How can policymakers account for and regulate various AVs' constantly-evolving driving behavior algorithms?  % <- Figures 1 and 2 answer these two questions.
Finally, what methods and tools can help AV designers, urban planners, and policymakers work together towards these goals? % <- Our new method answers this question.
% This paper explores these questions.

% Yet few have the know-how to handle all these complexities at once. 
% To date, it remains unclear what methodologies or workflows can help coordinate AV, city, and policy designs, in order to realize AVs' promises for better cities.
% Qian: might move this example to RW. Too long. %(for example, rather than paintakingly improving Computer Vision algorithms that can recognize various road signs in different weathers and view blocks, they might designing new road signs that are easily recognizable by both Computer Vision algorithms and naked eyes~\cite{Gilbert-Sociotechnical})
% (e.g., sensors, signs of pedestrian crossings) 
% take into account, for example, the different driving behaviors of AVs from different companies, as they design cities and set traffic rules?

% As a result, AV designers often treated existing city infrastructure and policies as fixed constraints, even though they can change somewhat frequently and easily~\citetodo{}.
% Urban designers and policymakers have started envisioning AV-ready city infrastructure and regulations. Yet these designs rarely considered, for example, how the different driving behaviors of AVs from different companies might create unexpected broader impacts and new regulatory 


% This paragraph: This paper's contribution in realizing these great promises.
This paper explores how the designs of AVs, cities, and policies can better coordinate and together shape better cities. \textbf{We first map the entangled relationships among AV, city, and policy design decisions} based on a comprehensive literature synthesis across human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, operations research, economy, and philosophy. %<- chapter 2.1
%, and the social sciences. % The social sciences is not one field. It's many.
This mapping helps those who aspire to shape AV-infused future cities to identify relevant design issues across the traditional \textit{AV design}, \textit{urban planning}, and \textit{legal and policy design} boundaries.%<- chapter 2.2
% In doing so, we highlight the benefits and, sometimes, the \textit{necessity} of simultaneously designing AV behaviors, AV services, city infrastructure, and policies~(chapter~\ref{sec:rw}).

\textbf{Next, we explore methods that could bridge these design issues, allowing AV, city, and policy designers prototype their designs simultaneously and observe their broader impacts}. % Chapter 3.
We envision a new approach, namely ``\textit{\newmethodlong}'' (\newmethod), \qian{will come back to this.}
We invite a more principled discussion around, not just whether, but \textit{how} AV designers, urban planners, and policymakers should work together to shape future smart cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Mapping AV, City, and Policy Design Choices}\label{sec:rw}
% This chapter is entirely Related Work (“What do other people think so far”?).
% Our contribution is merely organizing related work.
% Length budget: 2 pages of texts + 1 figure.


% This paragraph: AV, city, policy designs needs coordination, because any driving behavior, city, and policy designs need coordination. The components are the same.
 \input{fig_rw_interactions}
\vspace{3pt}\noindent
\textbf{The design choices around AV movement, AV services, city infrastructure, and policies are inherently interrelated.~}
Their connections echo the inherent connections among any vehicle's driving behaviors, services, city infrastructure, and policies. Figure~\ref{fig:interactions} maps out these relationships.
From top to bottom: \textit{Civil rights laws and policies}\footnote{This paper focuses mainly on US law and policies. This is a limitation of this work.} set rules that apply to all players in transportation. For example, they require car companies and their designs to allow free sharing of car-repair-related data~\cite{Robertson2020-uq}; they mandate that cities have certain amount of accessible parking and ride-sharing services have certain amount of accessible vehicles~\cite{Reck2018-sq, ADA_National_Network2018-bq}. 
\textit{Traffic regulations} instruct how vehicles and people should move (e.g., that all vehicles should yield to blind pedestrians and stop for school buses), % e.g., pedestrians law, school bus stopping law, clean ice and snow, yield to blind pedestrians, etc.
while \textit{transportation regulations} set rules and incentives related to road use and vehicle use (e.g., authorizing protected planes for bikes and scooters~\cite{Pierce2022-vq}.) % e.g., safety and accidents, auto insurance law, highway law, accessible parking mandates, electric vehicle subsidies, micromobility vehicle laws (e.g., protected lanes for scooters and bikers).
Within these legal and regulatory bounds (red arrows in Fig~\ref{fig:interactions}), AV designers design algorithms to instruct how their AVs move in relation to city infrastructure and other actor on the road (\textit{AV motion design}); AV service designers create additional rules and incentives related to such movements (e.g., via dynamic pricing~\cite{Kaddoura2020-vw}).
Good designs and services, after proven effective, could change transport infrastructure and even become policy mandates (green arrows in Fig~\ref{fig:interactions}, e.g., the wide adoption of ride-hailing services led to dedicated guest boarding zones at airports).
% With urban infrastructure, we refer to transport infrastructure such as roadway features and traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. 

This map makes it evident that realizing AVs' societal benefits \textit{requires} the coordination among AV, city, and policy designs. 
Empirical evidence from small-scale AV trials and large-scale traffic simulations agree~\cite{Soteropoulos2019-tw,Sperling2018-vk, Freemark2020-ms, Nacto2019-pe,Riggs2019-lx, Niroumand2023-an,Staricco2019-gn,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
For example, reducing congestion requires not only efficient AV navigation algorithms, but AV services, policies, and city infrastructure that incentivize shared rather than personally-owned AVs~\cite{Campbell2018-rr, Sanguinetti2019-de, Kaddoura2020-vw}.
Making future cities more accessible to people with mobility disabilities needs more than accessible AVs.
Incorporating accessible AVs into public transport services can radically scale up AV's accessibility benefits, while corresponding laws and policies could help minimize risks (e.g., by mandating blind driver boarding zones, or standardized way finding beacons)~\cite{Reck2018-sq, ADA_National_Network2018-bq,Ustwo2015-ck}.
% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
% According to a review study on AV modelling work, in the absence of policy intervention, the use of autonomous vehicles is likely to increase overall as they offer greater convenience over mass transportation~\cite{Soteropoulos2019-tw}.
% To fully realize the promised benefits of AVs, it is, therefore, crucial to implement AV-specific policies. Literature has suggested policies to mitigate the potential negative impacts of AVs, that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}, and promoting benefits such as ensuring a minimum number of accessible AVs. 
% Further, in order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}

 % (e.g., when AVs stop or accelerate)
  % (e.g., AV ride-sharing)
   % (e.g., road signs, public cameras and sensors)
   % s (e.g., how pedestrians are supposed to move) 
    % (e.g., when drivers stop or accelerate)
    % (ride-sharing)


\vspace{3pt}\noindent
\textbf{Different regulations and components of city infrastructure impact different types of AVs.~}
So far, we have treated AVs as one type of vehicle. Yet AVs are far from homogeneous. (Think autonomous long-haul trucks, autonomous commercial drivers' vehicles, autonomous scooters for last-mile transportation, and food delivery robots.) Therefore, they will likely achieve wide adoption at different times, use different parts of the city infrastructure, and operate under different traffic and transportation regulations (e.g., AV scooters will likely be subject to micro-mobility laws, while low-haul trucks will be to Hours of Service regulations in the U.S.)
In this sense, the wide variety of future AVs will add further complexities to the already complex AV-city-policy design landscape.
% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }
% AVs are like micromobility and trains simultaneously
% \subsubsection{What is novel about AVs in terms of planning complexity?}
% Autonomous vehicles represent a new frontier in urban and rural planning complexity.
% In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
% Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
% Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  
% In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% \section{Research Method}

% % This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
% % \placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}

% Our goal is to investigate what methods can bridge AVs, urban and rural design, as well as policy making.
% In order to understand the potential design-related problems as well as opportunities that could emerge from the interactions across these, we conducted a comprehensive literature review.
% % Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores 

% The initial research question guiding this review work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this, we ventured into diverse fields human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, philosophy, and social sciences; and research areas city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, AV ethics, and participatory design. \hauke{seperated fields and research areas}
% The analysis of the contributing literature revealed a strong grade of specialization into subfields with desire for interdisciplinary collaboration. 
% In the next section we synthesize the conclusions drawn from open problems mentioned in the literature, particularly related to those with relationship to AV Design, such as technology and infrastructure, the impact of AVs on transportation, as well as the role of policy in regulating the deployment of AVs.

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 

\section{Exploring Methods for Designing AVs, Cities, and Policies Simultaneously}\label{sec:proposition}
% This chapter is half Related Work (existing methods) and half our new ideas/contributions (iCAP-- “What do you argue and what’s the evidence?”)
% Length budget: 2 pages of texts + 1 figure.

\subsection{Common Methods Used In Current Practice}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}


% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?






% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 


%%%%% =====  stuff moved from chatper 2 to here START ====== %%%%
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }
% \qian{trade-offs across multiple goals}
% Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}
% \qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
% \placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
% most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
% Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
% Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

% \qian{This paragraph: As a result, people call for coordination among agencies.}
% While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  
%%%%% =====  Stuff moved from chatper 2 to here END ====== %%%%


% This paragraph: Current methods are isolated (AV design - 3D simulation on basic road conditions, road trials; city planning - low-detail maps and patterns, PD prototyping; urban infrastrcture - simulaion . Give examples.
Methods commonly used in designing AVs, cities, and policies rarely support the coordination among them~\cite{Rouse2021-ph,Yang2019-nr}.
% As \citet{Yang2019-nr} note, there is a lack of decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textit{Designing AV driving behavior algorithms:} Designers typically train algorithms using data that capture how human drivers drive on today's roads or test roads~\cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja,Dowling2022-wu, Suo2021-vm}. They then further evaluate and improve the algorithms using human feedback.  Virtual Reality (VR) and microscopic driving simulation, is used to gather insights to enable AVs better coordinate with other road users at crossroads~\cite{Dosovitskiy2017-jb, NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp}. These simulation environments typically are simple road situations rather than real-world driving conditions; Most have few if any pedestrians or other types of vehicles, and do not use AI models to simulate AV behavior.~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz, Pell2017-al};

% Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}. 

% These research methods incorporate human considerations, but not policy or infrastructure. 
% Due to the limitationThese simulation environments typically only include simple road situations, such as prototypical crossroads and parking space, with few if any pedestrians or other types of vehicles.s of technical AV testing, researchers devised Wizard of Oz methods for human-AV experiments on real roads~\cite {Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}.  Many simulations focus on AV behavior only, with often basic road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}, due to limitations researchers devised VR simulators~\cite{Goedicke2022-ys}. 
% Testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}.  
    \item \textit{City planning:~} City planning heavily relies upon established design patterns~\cite{alexander1977pattern}. Planners then apply or update the design patterns using low-detail maps or street cross-profiles~\cite{Riggs2017-hm, Lee2022-vd, Remix_by_Via2021-vm}. Geographic information systems manage access to increasing layers of information \cite{Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}. In recent years, participatory design (PD) methods have gained popularity, helping incorporate citizen needs and preferences into the process of urban design and prototyping~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew};
% low-detail maps and patterns, PD prototyping
    \item \textit{Urban infrastructure design and policy~}also heavily relies on established design patterns and guidelines~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. Additionally, designers~\cite{Zhang2022-uh, Dembski2020-gk} and policy makers~\cite{White2021-vo, Charitonidou2022-zg} use infrastructure simulations to identify, for example, the city bus lane arrangement that causes the least traffic disruption; % they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
    \item \textit{Traffic, transportation, and civil rights policy:~}\qian{We should describe current methods for policy as well. Prev. draft only mentioned PD.} Transportation research for policymaking uses modeling approaches, to examine questions of how for example, toll and fines impact traffic. Some researchers critique that the study of transportation policy is focusing too strongly on quantitative methods and tools, has become distant from the acutal messy policymaking cycle in the field, and assumes top-down execution of proposed ideas~\cite{Marsden2017-lu}. 
    To overcome these  limitations, methods that enable policymakers themselves to make good decisions through data from the environment and citizens are proposed~\cite{White2021-vo, Marcucci2020-qg}. Participatory methods have been part of policymaking since the beginning, through officials, agencies, and organized interest groups. Progress on how to scale up these approaches, better recognize efforts, and align various interests is still ongoing~\cite{Blomkamp2018-yg, Blomkamp2022-be, Oostveen2004-lk}. 
     \placeholder{Pilots in isolated regions to test AV safety. \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}}
\end{itemize}
% This parargaph: Some methods have the potential of supporting multiple designs. But no one acted on it.
A few researchers have argued that some of these methods have the potential to support in multiple design tasks. For example, \citet{Haegler2021-xv} argued that VR microscopic driving simulations might also help prototype infrastructure and policy re-development. \hauke{VR microscopic driving simulation is not something I came across. The link is for a city simulation for architecture only. I don't know about a specifc research that argues this.}
\citet{Marcucci2020-qg} and \citet{White2021-vo} have called for simulation and design tools for designing urban infrastructure and policy simultaneously. \citet{Riggs2020-yc} even extended this idea to AV, outlining the interrelated road space allocation and policy design issues related to AV and livable streets.
However, we did not find any research that further explored this possibility or created such tools. 
% This paragraph: People have started designing policy and cities together
% A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
% There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 
% If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

% hauke:
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …



\input{fig_rw_methods}

\subsection{Challenges in Bridging AV, City, Policy Design Methods}
% This paragraph: These methods can lead to results that are difficult to synthesize, because (1) they work under different assumptions and towards different goals
A closer look into current AV-, city-, and policy-design methods reveals more significant challenges in combining them.
First, these methods often operate on different fundamental assumptions and pursue different goals. In urban design contexts, AVs are part of the public infrastructure aiming to provide public goods. In AV motion design, AVs are commercial, often privately owned, products that provide passengers value. 
These differences can be seen as the roots of many debates around how AVs should move, who has a say in how AVs should move, and how they fit into the public sphere~\cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
% Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}. 
% Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
% As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.


% This paragraph: (2) they work at different levels of granularity.
Second, methods for AV design and methods for city- and policy-design operate at different levels of granularity.
Take simulations as an example. Driving simulations in AV motion design are microscopic, focusing on individual vehicles, pedestrians, and the interactions in-between within short periods of time~\cite{Saidallah2016-zx}. In contrast, simulations for city infrastructure and policy design are macroscopic, focusing on traffic flows, their longitudinal patterns, and their broader interactions with the city (e.g., would AV navigation algorithms over time isolate a neighborhood or lead to uneven road wear across the city?~\cite{Gilbert-Sociotechnical}.)
Combining methods of varying granularity levels means that designers must wrestle with the complex human-AV-environment interactions at multiple levels at the same time. It is likely to be cognitively demanding for the designers and computationally demanding for their design tools (e.g., VR simulation.)

% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 
\qian{Add a paragraph acknowledging the politics involved in all these? Av, city, policy design apparently are jobs of different sectors of the society. Getting them to cooperate is never as easy as it should be.} \hauke{I have a bit of that in line 187  \cite{Marsden2017-lu} argues that the field of policymaking study do not acknowledge the comlexities in the policy making cycle. Other than that I do not have a direct source in mind I read. https://www.taylorfrancis.com/books/mono/10.4324/9780203857557/politics-mobility-geoff-vigar (not read). We could also reference Winners bridges to briefly acknowldge that infrastructure (datasets, algorithms and policy too)  has built politics in.}
\placeholder{
AV, city, and policy design involve complex political processes that are often not fully acknowledged. The design of infrastructure, in particular, is embedded with politics and can shape the power dynamics of a society. As Winner argues, "the design of technology is itself a profoundly political activity" \cite{Winner1985-hp}. Similarly, Marsden \cite{Marsden2017-lu} argues that policymaking studies often overlook the complexities of the policymaking cycle. Bringing together these different sectors to cooperate in designing AVs, cities, and policies requires recognizing and addressing these political complexities and is not an easy task.
}

% Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} 
% For infrastructure design, guidelines, and design patterns were established over time~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. These demand an update with specific AV patterns~\cite{Nacto2019-pe}.  
% Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
% Participatory design methods are used in multiple areas to understand people's needs, in urban planning, tactical urbanism, citizen-led prototyping is becoming popular and shows unsatisfied needs by conventional planning~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}. Tactical urbanism has informed policymaking, but not AV design.

% Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
% There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019-gn, Meeder2017AutonomousVP, Acheampong2021-ql}. 


\subsection{Our Proposal: Integrative City-AV-Policy Simulation (iCAPS)}
\hauke{Complete, Citizen Centered City Simulation (4CS)}
\hauke{Complete, Citizen Centered City AV Replicator (4CAR)} (or renderer)

%his paragraph is summarizing the proposed methods.
Current scope-limited AV tests, complementary simulation studies, and analysis of natural human driving do not fully capture the effects that AVs will have at scale. They also do not consider the opportunities for re-designing urban and rural infrastructure or address nuanced human preferences.
We identify two promising approaches. \textit{Citizen led city-AV-policy design} can help to ease value tension through democratic (participatory) processes. \textit{Holistic simulations} can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

\subsubsection{Citizen Led City-AV-Policy Design}
We propose utilizing participatory design methods across all areas having impact on and being impacted by AVs. 
Besides a lack of methods that allow coordination, we identified a method blind spot. While participatory design is fairly common for infrastructure design and civil rights inquiries, it is rare for AV motion design/traffic regulations and AV service design/transportation regulations. It is crucial for AV motion design and AV service design to address citizens' needs and moral values. 
\begin{itemize}
\item \textit{AV Neighborhood Prototyping:~}
%Many citizen needs cannot be understood through quantitative simulation and optimization. We suggest adopting rising participatory design methods in urban planning for AV planning. 
%Testing urban prototypes with members of the public and guerilla style action of individuals have successfully reshaped urban room in many cities. These methods are grouped under the category of tactical urbanism. 
Urban prototyping, offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. 
We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. We see potential to create hybrid methods, using Wizard of Oz to design AV motion and traditional participatory design to design policy and AV Service, all simultaneously. % WoZ with simulated AVs is most useful to simulate individual interactions with vehicles in individual streets. %Just as with tactical urbanism, 
AV Neighborhood Prototyping will be most effective with people from their relevant neighborhoods and enable them to influence design choices such as where AV pick up spots and delivery stations shall be placed. 

\item \textit{Nuanced AV Motion Design:~}
%this paragraph describes one potential citizen led CAPS experiment
A change in traffic regulations just on AV provider's request without sufficient evidence is unlikely. To prove that, new av motion, which requires change in regulations, is satisfying user needs, a VR driving study could be conducted that asks people to fine-tune AV motion, traffic regulations, and urban infrastructure while assuming various perspectives such as a passenger, pedestrian encountering a vehicle, and resident in a neighborhood. The outcome of such a study will unravel different preferences for AV motion (e.g., AV acceleration values), urban infrastructure (e.g., width of AV lane) and traffic regulations (e.g., AV speed limit). With such a study, we can go beyond current AV motion design, which imitates human \textit{driver} behavior and takes regulations as well as infrastructure as fixed.
%this paragraph describes a second potential citizen led CAPS experiment
\item \textit{Moral Cities:~}:
% Another similar study, could probe for upcoming moral questions of AV traffic routing and zoning. In an online experiment, participants could contribute opinions on complicated AV transportation regulation questions with impact on infrastructure. Should AVs drive through the predominantly poor district, or through the sightseeing district;  assuming the same efficiency, who should bear the noise and emissions? Should AVs park outside the city in dedicated slots, providing space for other use, or inside the city at the curb, minimizing pick up waiting time? Experiments like this can gather information about socially acceptable norms for AV service, AV transport regulations, and AV infrastructure. 
A comparable study, targeting transportation regulation, could explore future ethical AV dilemmas, by conducting an online experiment; participants provide input on complex questions related to AV traffic routing and zoning that have implications for infrastructure. These questions might include determining whether AVs should travel through primarily low-income areas or sightseeing districts when efficiency is equal, who should bear the burden of noise and emissions. Additionally, the study could investigate whether AVs should park in designated slots outside the city to free up space for other uses or at curbside in the city to minimize wait times for pick-up.
\end{itemize}
The three examples presented above for citizen-led city AV-policy design can inform and assist policymakers and AV developers in coordinating actionable human preferences and resolving \textit{seemingly} trolley-problem-like conflicts.

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulators are necessary because only they allow for the evaluation and optimization of future transportation policies, city designs and AV behavior in a safe, controlled, and cost-effective environment. 
Holistic city simulators allow various stakeholders to engage across disciplines, but they allow policymakers to simulate how AV service and motion design might react to regulation and infrastructure changes. Do the implemented changes lead to the desired effects, will they cause unintended consequences, will the learning and automated AVs evade them?

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV 
% This paragraph: Why can it reveal opportunities? 
% With holistic approaches to the simulation of AVs, urban infrastructure, and policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look in reality. Shared mobility services allowed to collect some pre-AV-deployment insights to AV service design and policy. The interdependencies of AV motion design, and infrastructure design are of higher urgency as they are less researched. 



% This paragraph: Why can it identify challenges?

% Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 

% \hauke{Multi Goal optimation would not be an own method and so do the other not. All our envisioned/found methods fall under the category holistic simulation. Digital methods can be easily combined into \textit{holistic tools.} The promise of digital twins, and geospatial information systems, always was to bring diverse information as layers and help to compare and see it side by side. Requries that modeling and simulatio are done in compatible data formats/enviornments. Similar to work by taubman harvard analogue (participatory) methods can be called simulations too. }

\begin{itemize}
    \item \textit{Transgenic Twin:~}  To make Digital Twins, which are data-based replicas of cities components and processes, useful for prototyping AVs, city infrastructure, and policies simultaneously they need to be equipped with the appropriate design tools to manipulate AV behavior, regulations, and infrastructure. Nowadays, these tools are not found in digital twins but only in the specific tools such as city planners. Also, digital Twin assets are often static. We need to either include HD Maps, usually expensive proprietary assets, or develop tools which, for example, transfer point clouds of city scans into modifiable geometry of houses, streets, and traffic signs. Machine learning methods that can detect bounding boxes of houses, street and traffic signs, already used for AV motion design, can automate these processes. To simulate the complex processes of the city,  rather than hand modeling, we can learn behavior from the twins rich data~\cite{Suo2021-vm}. Once processes and components are turned flexible, react with each other in a complex model, we can start to play with the simulated DNA of the city,  engineering preferable twins.   % \hauke{For combining data that can be used for AV motion design as well as infrastrucute and policy desing, 3d spatial digital twins are the ideal tool. They are continuos updating data sources and therfore an ideal enviornment to train and finetune AVs in. With another layer of transportation, the AV service design can also be integrated. This can aid coordination. New infrastructure designs aan immediately tested with AV models. }
    \item \textit{Multi-Goal Optimization}:~   \hauke{I am tending to favour to leave multi goal simulation out. }
    % \hauke{Multi goal optimization is a method to optimize multiple goals. Even if not done in a lot of 'traditional; traffic modeling work it is becoming a default practice.} 
In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These address the problems of their specific subfields.  
    AV motion design predominately tries to solve the safety of AVs, achieving  better than human levels of safety. Traffic regulation research favors network efficiency, without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Transportation regulations nowadays turned to sustainability. AV service design prioritizes the optimization of the efficient use of all AVs.  Human needs are multi-goal, therefore urban rural infrastructure design addresses many goals. Livable cities, and transport, cannot be described in narrow single  goal terms. We propose the good practice to use (bayesian) multi goal optimzaton for simulations that acknowledge multiple goals. 
    % This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
    % This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.
    % Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a fine-grained level. 
    % Some multi-goal-optimization limitations are resolved meanwhile, and therefore it can become a tool for policy optimization. A few examples of Bayesian multi goal traffic optimization, are promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 
 
\end{itemize}



% \subsubsection{An Example}



% \qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
% \placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% % The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
% Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
% Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
% Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 

The existing and proposed methods complement and complete each in a rich method space. Insights represented inside Transgenic Twins, combined with insights from Citizen Led City-AV-Policy Design can, with novel multi goal optimization techniques, help to find the Pareto optimal configuration of the city, and then policymakers can use subjective criteria and deliberation to decide for the best compromise. 





\section{Discussion: What is needed from government, industry, and academia?}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated and participatory city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. 
%, as it allows for the most flexibility and consolidation. 

%\subsection{Requirement: Open Data, Simulators and Standards}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. Data sharing platforms could also facilitate communication and collaboration between different stakeholders, making it easier to identify potential conflicts or issues. Finally, we suggest developing integrated design guidelines and standards that cover all aspects of AV design, city infrastructure, and policy can help ensure that all designs are compatible with each other and contribute to the goals of better cities. These guidelines and standards could be developed collaboratively by designers, policymakers, and other stakeholders and could be used to evaluate and approve new AV designs, infrastructure plans, and policy proposals.

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. HCI should step ahead with the development of such methods and tools.

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote citizen-led and integrated approaches, specialized field expertise is necessary, we do not see participatory methods and holistic simulators as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v7.tex <==
\section{Introduction}
% Title+  Introduction: 1 page


% This paragraph: The great promises of AVs + AV services = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Autonomous Vehicles (AVs) promise to improve cities in ways that would not have been possible otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce car crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
AV ride-sharing services can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighborhoods~\cite{Gilbert-Sociotechnical}. 
AVs can also reduce congestion and cruising-for-parking by coordinating with each other and with smart city infrastructure, hence decrease vehicle emissions~\cite{Rojas-Rueda2017-xl}.
These promises of safer, more equal, more sustainable, or more livable cities have long been central considerations in AV design.

% Cities urban infrastructure and in connection quality of life at the curb leave much to be desired. Building and maintaining public transport is expensive, and it cannot transport individuals end-to-end; individual car ownership, on the other hand, is causing accidents, unsustainable and not scalable. Governments put therefore hope into AVs \cite{World_Economic_Forum2020-ox}. AVs have the potential, if properly implemented, to improve the livability of cities in various ways, such as by closing transportation gaps, reducing car infrastructure, increasing safety, sustainability, and equity~\cite{Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. %\qian{Why? how? Add evidence.} 
% AVs show great promises in improving cities. Their potential to create safer, more livable, sustainable, efficient, and equitable cities is widely acknowledged \cite{Golbabaei2020TheRO, PETTIGREW201964, Rojas-Rueda2017-xl}. Commonly, mentioned benefits are reduced traffic accidents, decrease in vehicle emissions and congestion, improved safety for pedestrians and cyclists, better mobility for the elderly and disabled, increase in active travel, as well as reduced need for parking space. 


% This paragraph: Realizing these promises requires AV motion+service designs to coordinate with city design and policies. They currently are not. 
Yet AVs' societal benefits are far from guaranteed; Realizing them requires careful coordination among the designs of AVs, city infrastructure, as well as related regulations~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019-gn, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Making AVs available to the public alone involves complex policy questions (e.g., liability, privacy, and insurance)~\cite{fagnant2015preparing} and can entail city-scale infrastructural changes (e.g., should autonomous food-delivery robots use bike lanes or new dedicated lanes?~\cite{food-delivery-robot-bikelane-wired}). Not to mention realizing AVs' more ambitious promises.
% \hauke{This example is somehow throwing me off. }
% Why? If you don't like it, feel free to change to a different one.
% much more so in making AVs catalysts of safer, more equal, more sustainable, or more livable cities.

% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.

% This paragraph: articulate precisely what problems/questions this paper solves 
Coordinating AV, policy, and city designs is not just complex; It requires designers to confront the three-way ``\textit{chick-and-egg}'' relationship among them~\cite{Gilbert-Sociotechnical,Wu2018-oy, Brozynski2022-yv}.
Changes to any one of them---AVs' driving patterns, city layout, and traffic and transportation policies---must be compatible with the other two to be practical. However, changes to any of them also change the other two.
Many researchers therefore have argued for considering the three simultaneously~\cite{Matowicki2020-vy, Aoyama2021-jj, Duarte2018-wg, OToole2020-so, Freemark2020-ms, Staricco2019-gn}.
But how? \qian{Need to articulate our research questions better still. Will come back to this.}
How can AV designers go beyond simple road scenarios and today's traffic laws when designing AVs for future cities? How can urban planners accommodate AVs' infrastructural needs while mitigating unintended consequences? How can policymakers account for and regulate various AVs' constantly-evolving driving behavior algorithms?  % <- Figures 1 and 2 answer these two questions.
Finally, what methods and tools can help AV designers, urban planners, and policymakers work together towards these goals? % <- Our new method answers this question.
% This paper explores these questions.

% Yet few have the know-how to handle all these complexities at once. 
% To date, it remains unclear what methodologies or workflows can help coordinate AV, city, and policy designs, in order to realize AVs' promises for better cities.
% Qian: might move this example to RW. Too long. %(for example, rather than paintakingly improving Computer Vision algorithms that can recognize various road signs in different weathers and view blocks, they might designing new road signs that are easily recognizable by both Computer Vision algorithms and naked eyes~\cite{Gilbert-Sociotechnical})
% (e.g., sensors, signs of pedestrian crossings) 
% take into account, for example, the different driving behaviors of AVs from different companies, as they design cities and set traffic rules?

% As a result, AV designers often treated existing city infrastructure and policies as fixed constraints, even though they can change somewhat frequently and easily~\citetodo{}.
% Urban designers and policymakers have started envisioning AV-ready city infrastructure and regulations. Yet these designs rarely considered, for example, how the different driving behaviors of AVs from different companies might create unexpected broader impacts and new regulatory 


% This paragraph: This paper's contribution in realizing these great promises.
This paper explores how the designs of AVs, cities, and policies can better coordinate and together shape better cities. \textbf{We first map the entangled relationships among AV, city, and policy design decisions} based on a comprehensive literature synthesis across human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, operations research, economy, and philosophy. %<- chapter 2.1
%, and the social sciences. % The social sciences is not one field. It's many.
This mapping helps those who aspire to shape AV-infused future cities to identify relevant design issues across the traditional \textit{AV design}, \textit{urban planning}, and \textit{legal and policy design} boundaries.%<- chapter 2.2
% In doing so, we highlight the benefits and, sometimes, the \textit{necessity} of simultaneously designing AV behaviors, AV services, city infrastructure, and policies~(chapter~\ref{sec:rw}).

\textbf{Next, we explore methods that could bridge these design issues, allowing AV, city, and policy designers prototype their designs simultaneously and observe their broader impacts}. % Chapter 3.
We envision a new approach, namely ``\textit{\newmethodlong}'' (\newmethod), \qian{will come back to this.}
We invite a more principled discussion around, not just whether, but \textit{how} AV designers, urban planners, and policymakers should work together to shape future smart cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Mapping AV, City, and Policy Design Choices}\label{sec:rw}
% This chapter is entirely Related Work (“What do other people think so far”?).
% Our contribution is merely organizing related work.
% Length budget: 2 pages of texts + 1 figure.


% This paragraph: AV, city, policy designs needs coordination, because any driving behavior, city, and policy designs need coordination. The components are the same.
 \input{fig_rw_interactions}
\vspace{3pt}\noindent
\textbf{The design choices around AV movement, AV services, city infrastructure, and policies are inherently interrelated.~}
Their connections echo the inherent connections among any vehicle's driving behaviors, services, city infrastructure, and policies. Figure~\ref{fig:interactions} maps out these relationships.
From top to bottom: \textit{Civil rights laws and policies}\footnote{This paper focuses mainly on US law and policies. This is a limitation of this work.} set rules that apply to all players in transportation. For example, they require car companies and their designs to allow free sharing of car-repair-related data~\cite{Robertson2020-uq}; they mandate that cities have certain amount of accessible parking and ride-sharing services have certain amount of accessible vehicles~\cite{Reck2018-sq, ADA_National_Network2018-bq}. 
\textit{Traffic regulations} instruct how vehicles and people should move (e.g., that all vehicles should yield to blind pedestrians and stop for school buses), % e.g., pedestrians law, school bus stopping law, clean ice and snow, yield to blind pedestrians, etc.
while \textit{transportation regulations} set rules and incentives related to road use and vehicle use (e.g., authorizing protected planes for bikes and scooters~\cite{Pierce2022-vq}.) % e.g., safety and accidents, auto insurance law, highway law, accessible parking mandates, electric vehicle subsidies, micromobility vehicle laws (e.g., protected lanes for scooters and bikers).
Within these legal and regulatory bounds (red arrows in Fig~\ref{fig:interactions}), AV designers design algorithms to instruct how their AVs move in relation to city infrastructure and other actor on the road (\textit{AV motion design}); AV service designers create additional rules and incentives related to such movements (e.g., via dynamic pricing~\cite{Kaddoura2020-vw}).
Good designs and services, after proven effective, could change transport infrastructure and even become policy mandates (green arrows in Fig~\ref{fig:interactions}, e.g., the wide adoption of ride-hailing services led to dedicated guest boarding zones at airports).
% With urban infrastructure, we refer to transport infrastructure such as roadway features and traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. 

This map makes it evident that realizing AVs' societal benefits \textit{requires} the coordination among AV, city, and policy designs. 
Empirical evidence from small-scale AV trials and large-scale traffic simulations agree~\cite{Soteropoulos2019-tw,Sperling2018-vk, Freemark2020-ms, Nacto2019-pe,Riggs2019-lx, Niroumand2023-an,Staricco2019-gn,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
For example, reducing congestion requires not only efficient AV navigation algorithms, but AV services, policies, and city infrastructure that incentivize shared rather than personally-owned AVs~\cite{Campbell2018-rr, Sanguinetti2019-de, Kaddoura2020-vw}.
Making future cities more accessible to people with mobility disabilities needs more than accessible AVs.
Incorporating accessible AVs into public transport services can radically scale up AV's accessibility benefits, while corresponding laws and policies could help minimize risks (e.g., by mandating blind driver boarding zones, or standardized way finding beacons)~\cite{Reck2018-sq, ADA_National_Network2018-bq,Ustwo2015-ck}.
% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
% According to a review study on AV modelling work, in the absence of policy intervention, the use of autonomous vehicles is likely to increase overall as they offer greater convenience over mass transportation~\cite{Soteropoulos2019-tw}.
% To fully realize the promised benefits of AVs, it is, therefore, crucial to implement AV-specific policies. Literature has suggested policies to mitigate the potential negative impacts of AVs, that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}, and promoting benefits such as ensuring a minimum number of accessible AVs. 
% Further, in order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}

 % (e.g., when AVs stop or accelerate)
  % (e.g., AV ride-sharing)
   % (e.g., road signs, public cameras and sensors)
   % s (e.g., how pedestrians are supposed to move) 
    % (e.g., when drivers stop or accelerate)
    % (ride-sharing)


\vspace{3pt}\noindent
\textbf{Different regulations and components of city infrastructure impact different types of AVs.~}
So far, we have treated AVs as one type of vehicle. Yet AVs are far from homogeneous. (Think autonomous long-haul trucks, autonomous commercial drivers' vehicles, autonomous scooters for last-mile transportation, and food delivery robots.) Therefore, they will likely achieve wide adoption at different times, use different parts of the city infrastructure, and operate under different traffic and transportation regulations (e.g., AV scooters will likely be subject to micro-mobility laws, while low-haul trucks will be to Hours of Service regulations in the U.S.)
In this sense, the wide variety of future AVs will add further complexities to the already complex AV-city-policy design landscape.
% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }
% AVs are like micromobility and trains simultaneously
% \subsubsection{What is novel about AVs in terms of planning complexity?}
% Autonomous vehicles represent a new frontier in urban and rural planning complexity.
% In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
% Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
% Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  
% In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% \section{Research Method}

% % This paragraph: Our goal is to investigate XXX. In order to do so, we did XXX (literature review....)
% % \placeholder{What methods can bridge AV, cities, and policy design? Specifically, what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?}

% Our goal is to investigate what methods can bridge AVs, urban and rural design, as well as policy making.
% In order to understand the potential design-related problems as well as opportunities that could emerge from the interactions across these, we conducted a comprehensive literature review.
% % Based on a comprehensive literature analysis on autonomous vehicles, transportation, city design, and policy, this paper explores 

% The initial research question guiding this review work was “How should we design autonomous vehicles and cities together at scale?”. Branching off from this, we ventured into diverse fields human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, artificial intelligence, operations research, economy, philosophy, and social sciences; and research areas city design, policymaking, safety research, AV interaction research, AV datasets, AV ethics, agent optimization, simulation, economics, AV ethics, and participatory design. \hauke{seperated fields and research areas}
% The analysis of the contributing literature revealed a strong grade of specialization into subfields with desire for interdisciplinary collaboration. 
% In the next section we synthesize the conclusions drawn from open problems mentioned in the literature, particularly related to those with relationship to AV Design, such as technology and infrastructure, the impact of AVs on transportation, as well as the role of policy in regulating the deployment of AVs.

% As no solutions and methods for the design of AV and city together at scale were identified, we conducted several thought experiments to explore potential scenarios that may arise from the deployment of AVs in urban environments. 

\section{Exploring Methods for Designing AVs, Cities, and Policies Simultaneously}\label{sec:proposition}
% This chapter is half Related Work (existing methods) and half our new ideas/contributions (iCAP-- “What do you argue and what’s the evidence?”)
% Length budget: 2 pages of texts + 1 figure.

\subsection{Common Methods Used In Current Practice}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}


% what methods can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across city infra, AVs, and policy?






% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 


%%%%% =====  stuff moved from chatper 2 to here START ====== %%%%
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }
% \qian{trade-offs across multiple goals}
% Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}
% \qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
% \placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
% most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
% Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
% Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

% \qian{This paragraph: As a result, people call for coordination among agencies.}
% While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  
%%%%% =====  Stuff moved from chatper 2 to here END ====== %%%%


% This paragraph: Current methods are isolated (AV design - 3D simulation on basic road conditions, road trials; city planning - low-detail maps and patterns, PD prototyping; urban infrastrcture - simulaion . Give examples.
Methods commonly used in designing AVs, cities, and policies rarely support the coordination among them~\cite{Rouse2021-ph,Yang2019-nr}.
% As \citet{Yang2019-nr} note, there is a lack of decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textit{Designing AV driving behavior algorithms:} Designers typically train algorithms using data that capture how human drivers drive on today's roads or test roads~\cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja,Dowling2022-wu, Suo2021-vm}. They then further evaluate and improve the algorithms using human feedback.  Virtual Reality (VR) and microscopic driving simulation, is used to gather insights to enable AVs better coordinate with other road users at crossroads~\cite{Dosovitskiy2017-jb, NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp}. These simulation environments typically are simple road situations rather than real-world driving conditions; Most have few if any pedestrians or other types of vehicles, and do not use AI models to simulate AV behavior.~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz, Pell2017-al};

% Most traffic road simulators do not even support autonomous vehicles \cite{Pell2013-vo}. 

% These research methods incorporate human considerations, but not policy or infrastructure. 
% Due to the limitationThese simulation environments typically only include simple road situations, such as prototypical crossroads and parking space, with few if any pedestrians or other types of vehicles.s of technical AV testing, researchers devised Wizard of Oz methods for human-AV experiments on real roads~\cite {Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}.  Many simulations focus on AV behavior only, with often basic road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}, due to limitations researchers devised VR simulators~\cite{Goedicke2022-ys}. 
% Testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}.  
    \item \textit{City planning:~} City planning heavily relies upon established design patterns~\cite{alexander1977pattern}. Planners then apply or update the design patterns using low-detail maps or street cross-profiles~\cite{Riggs2017-hm, Lee2022-vd, Remix_by_Via2021-vm}. Geographic information systems manage access to increasing layers of information \cite{Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}. In recent years, participatory design (PD) methods have gained popularity, helping incorporate citizen needs and preferences into the process of urban design and prototyping~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew};
% low-detail maps and patterns, PD prototyping
    \item \textit{Urban infrastructure design and policy~}also heavily relies on established design patterns and guidelines~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. Additionally, designers~\cite{Zhang2022-uh, Dembski2020-gk} and policy makers~\cite{White2021-vo, Charitonidou2022-zg} use infrastructure simulations to identify, for example, the city bus lane arrangement that causes the least traffic disruption; % they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
    \item \textit{Traffic, transportation, and civil rights policy:~}\qian{We should describe current methods for policy as well. Prev. draft only mentioned PD.} Transportation research for policymaking uses modeling approaches, to examine questions of how for example, toll and fines impact traffic. Some researchers critique that the study of transportation policy is focusing too strongly on quantitative methods and tools, has become distant from the acutal messy policymaking cycle in the field, and assumes top-down execution of proposed ideas~\cite{Marsden2017-lu}. 
    To overcome these  limitations, methods that enable policymakers themselves to make good decisions through data from the environment and citizens are proposed~\cite{White2021-vo, Marcucci2020-qg}. Participatory methods have been part of policymaking since the beginning, through officials, agencies, and organized interest groups. Progress on how to scale up these approaches, better recognize efforts, and align various interests is still ongoing~\cite{Blomkamp2018-yg, Blomkamp2022-be, Oostveen2004-lk}. 
     \placeholder{Pilots in isolated regions to test AV safety. \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}}
\end{itemize}
% This parargaph: Some methods have the potential of supporting multiple designs. But no one acted on it.
A few researchers have argued that some of these methods have the potential to support in multiple design tasks. For example, \citet{Haegler2021-xv} argued that VR microscopic driving simulations might also help prototype infrastructure and policy re-development. \hauke{VR microscopic driving simulation is not something I came across. The link is for a city simulation for architecture only. I don't know about a specifc research that argues this.}
\citet{Marcucci2020-qg} and \citet{White2021-vo} have called for simulation and design tools for designing urban infrastructure and policy simultaneously. \citet{Riggs2020-yc} even extended this idea to AV, outlining the interrelated road space allocation and policy design issues related to AV and livable streets.
Interestingly, no research that we are aware of further explored this possibility or created such tools. 
% This paragraph: People have started designing policy and cities together
% A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
% There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 
% If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

% hauke:
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …



\input{fig_rw_methods}

\subsection{Challenges in Bridging AV, City, Policy Design Methods}

A closer look into current AV-, city-, and policy-design methods, however, reveals a number of more significant challenges in combining them.


% This paragraph: (1) scale/scope of their studies setup
First, AV design and city- and policy-design operate at different scales, with varying levels of granularity.
Take simulation studies as an example. In AV driving behavior design, simulations help designers choreograph interactions among individual vehicles and pedestrians, typically within short periods of time (e.g., when merging on highway)~\cite{Saidallah2016-zx}. 
In city infrastructure and policy design, simulation methods such as digital twins focus on traffic flows, their longitudinal patterns, and potential macro impact on the city (e.g., would AV navigation patterns catalyze social inequalities across neighborhoods over time?~\cite{Gilbert-Sociotechnical}.) \qian{Isn't digital twins an exception to this (it does both individual vehicle level and traffic flow level simulations)?}
Combining methods of varying granularity levels means that designers must wrestle with all of the above human-AV-environment interactions at the same time. Such integrative methods are likely to be cognitively demanding for the designers and computationally demanding for their simulation systems. 
\qian{How is our method immune to this problem?}


% Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}. 
% Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
% As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.

% This paragraph is summarizing the proposed methods.
% Current scope-limited AV tests, complementary simulation studies, and analysis of natural human driving do not fully capture the effects that AVs will have at scale. They also do not consider the opportunities for re-designing urban and rural infrastructure or address nuanced human preferences.

% This paragraph: These methods can lead to results that are difficult to synthesize, because (2) they work under different assumptions and towards different goals
Even if their simulated road environment can be integrated, AV, city, and policy design methods often operate on different assumptions and pursue different goals.
In urban infrastructure design, AVs are often part of the public infrastructure, aiming to provide maximum public goods. In AV motion design, AVs are (often privately-owned) commercial products that provide passengers value. \qian{I know I wrote this, but I am not sure if these two sentences are true... They read like sweeping arguments. Will come back to this.}
These differences can be seen as the roots of many debates around how AVs should move, who has a say in how AVs should move, and how they fit into the public sphere~\cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.

% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 

% This paragraph: acknowledging the politics involved in designing the trio simutanously: 
\qian{Third challenge: Their Av, city, policy design apparently are jobs of different sectors of the society. Getting them to cooperate is never as easy as it should be.} 
\placeholder{
AV, city, and policy design involve complex political processes that are often not fully acknowledged. The design of infrastructure, in particular, is embedded with politics and can shape the power dynamics of a society. As Winner argues, "the design of technology is itself a profoundly political activity" \cite{Winner1985-hp}. Similarly, Marsden \cite{Marsden2017-lu} argues that policymaking studies often overlook the complexities of the policymaking cycle. Bringing together these different sectors to cooperate in designing AVs, cities, and policies requires recognizing and addressing these political complexities and is not an easy task.
}\qian{For example, we only see democratic/participatory approaches to AV design used in policy/city design contexts, but not in AV company design contexts.}
% \hauke{I have a bit of that in line 187  \cite{Marsden2017-lu} argues that the field of policymaking study do not acknowledge the comlexities in the policy making cycle. Other than that I do not have a direct source in mind I read. https://www.taylorfrancis.com/books/mono/10.4324/9780203857557/politics-mobility-geoff-vigar (not read). We could also reference Winners bridges to briefly acknowldge that infrastructure (datasets, algorithms and policy too)  has built politics in.}



% Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} 
% For infrastructure design, guidelines, and design patterns were established over time~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. These demand an update with specific AV patterns~\cite{Nacto2019-pe}.  
% Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
% Participatory design methods are used in multiple areas to understand people's needs, in urban planning, tactical urbanism, citizen-led prototyping is becoming popular and shows unsatisfied needs by conventional planning~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}. Tactical urbanism has informed policymaking, but not AV design.

% Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
% There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019-gn, Meeder2017AutonomousVP, Acheampong2021-ql}. 


\subsection{Our Proposal: Integrative City-AV-Policy Simulation (iCAPS)}
% \hauke{Complete, Citizen Centered City Simulation (4CS)}
% \hauke{Complete, Citizen Centered City AV Replicator (4CAR)} (or renderer)

We identify two promising approaches. \textit{Citizen led city-AV-policy design} can help to ease value tension through democratic (participatory) processes. \textit{Holistic simulations} can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

\subsubsection{Citizen Led City-AV-Policy Design}
We propose utilizing participatory design methods across all areas having impact on and being impacted by AVs. 
Besides a lack of methods that allow coordination, we identified a method blind spot. While participatory design is fairly common for infrastructure design and civil rights inquiries, it is rare for AV motion design/traffic regulations and AV service design/transportation regulations. It is crucial for AV motion design and AV service design to address citizens' needs and moral values. 

\begin{itemize}
\item \textit{AV Neighborhood Prototyping:~}
%Many citizen needs cannot be understood through quantitative simulation and optimization. We suggest adopting rising participatory design methods in urban planning for AV planning. 
%Testing urban prototypes with members of the public and guerilla style action of individuals have successfully reshaped urban room in many cities. These methods are grouped under the category of tactical urbanism. 
Urban prototyping, offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. 
We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. We see potential to create hybrid methods, using Wizard of Oz to design AV motion and traditional participatory design to design policy and AV Service, all simultaneously. % WoZ with simulated AVs is most useful to simulate individual interactions with vehicles in individual streets. %Just as with tactical urbanism, 
AV Neighborhood Prototyping will be most effective with people from their relevant neighborhoods and enable them to influence design choices such as where AV pick up spots and delivery stations shall be placed. 

\item \textit{Nuanced AV Motion Design:~}
%this paragraph describes one potential citizen led CAPS experiment
A change in traffic regulations just on AV provider's request without sufficient evidence is unlikely. To prove that, new av motion, which requires change in regulations, is satisfying user needs, a VR driving study could be conducted that asks people to fine-tune AV motion, traffic regulations, and urban infrastructure while assuming various perspectives such as a passenger, pedestrian encountering a vehicle, and resident in a neighborhood. The outcome of such a study will unravel different preferences for AV motion (e.g., AV acceleration values), urban infrastructure (e.g., width of AV lane) and traffic regulations (e.g., AV speed limit). With such a study, we can go beyond current AV motion design, which imitates human \textit{driver} behavior and takes regulations as well as infrastructure as fixed.
%this paragraph describes a second potential citizen led CAPS experiment
\item \textit{Moral Cities:~}:
% Another similar study, could probe for upcoming moral questions of AV traffic routing and zoning. In an online experiment, participants could contribute opinions on complicated AV transportation regulation questions with impact on infrastructure. Should AVs drive through the predominantly poor district, or through the sightseeing district;  assuming the same efficiency, who should bear the noise and emissions? Should AVs park outside the city in dedicated slots, providing space for other use, or inside the city at the curb, minimizing pick up waiting time? Experiments like this can gather information about socially acceptable norms for AV service, AV transport regulations, and AV infrastructure. 
A comparable study, targeting transportation regulation, could explore future ethical AV dilemmas, by conducting an online experiment; participants provide input on complex questions related to AV traffic routing and zoning that have implications for infrastructure. These questions might include determining whether AVs should travel through primarily low-income areas or sightseeing districts when efficiency is equal, who should bear the burden of noise and emissions. Additionally, the study could investigate whether AVs should park in designated slots outside the city to free up space for other uses or at curbside in the city to minimize wait times for pick-up.
\end{itemize}
The three examples presented above for citizen-led city AV-policy design can inform and assist policymakers and AV developers in coordinating actionable human preferences and resolving \textit{seemingly} trolley-problem-like conflicts.

\subsubsection{Holistic Simulation}
% Takeaway of this subsection: We can leverage holistic policy+urban infra+AV simulation to understand the interdependencies across each component and also help align how these ideals (livable, sustainable, etc.) should look in reality.

Simulators are necessary because only they allow for the evaluation and optimization of future transportation policies, city designs and AV behavior in a safe, controlled, and cost-effective environment. 
Holistic city simulators allow various stakeholders to engage across disciplines, but they allow policymakers to simulate how AV service and motion design might react to regulation and infrastructure changes. Do the implemented changes lead to the desired effects, will they cause unintended consequences, will the learning and automated AVs evade them?

% This paragraph: Make clear what we mean by holistic policy+urban infra+AV 
% This paragraph: Why can it reveal opportunities? 
% With holistic approaches to the simulation of AVs, urban infrastructure, and policies, we can better understand the interdependencies between these components and also help stakeholders align how these ideals (livable, sustainable, etc.) should look in reality. Shared mobility services allowed to collect some pre-AV-deployment insights to AV service design and policy. The interdependencies of AV motion design, and infrastructure design are of higher urgency as they are less researched. 



% This paragraph: Why can it identify challenges?

% Using holistic simulation, we can discuss tensions early on and better avoid Planning mistakes. Also, we can better anticipate if the public should intervene and influence AVs. 

% \hauke{Multi Goal optimation would not be an own method and so do the other not. All our envisioned/found methods fall under the category holistic simulation. Digital methods can be easily combined into \textit{holistic tools.} The promise of digital twins, and geospatial information systems, always was to bring diverse information as layers and help to compare and see it side by side. Requries that modeling and simulatio are done in compatible data formats/enviornments. Similar to work by taubman harvard analogue (participatory) methods can be called simulations too. }

\begin{itemize}
    \item \textit{Transgenic Twin:~}  To make Digital Twins, which are data-based replicas of cities components and processes, useful for prototyping AVs, city infrastructure, and policies simultaneously they need to be equipped with the appropriate design tools to manipulate AV behavior, regulations, and infrastructure. Nowadays, these tools are not found in digital twins but only in the specific tools such as city planners. Also, digital Twin assets are often static. We need to either include HD Maps, usually expensive proprietary assets, or develop tools which, for example, transfer point clouds of city scans into modifiable geometry of houses, streets, and traffic signs. Machine learning methods that can detect bounding boxes of houses, street and traffic signs, already used for AV motion design, can automate these processes. To simulate the complex processes of the city,  rather than hand modeling, we can learn behavior from the twins rich data~\cite{Suo2021-vm}. Once processes and components are turned flexible, react with each other in a complex model, we can start to play with the simulated DNA of the city,  engineering preferable twins.   % \hauke{For combining data that can be used for AV motion design as well as infrastrucute and policy desing, 3d spatial digital twins are the ideal tool. They are continuos updating data sources and therfore an ideal enviornment to train and finetune AVs in. With another layer of transportation, the AV service design can also be integrated. This can aid coordination. New infrastructure designs aan immediately tested with AV models. }
    \item \textit{Multi-Goal Optimization}:~   \hauke{I am tending to favour to leave multi goal simulation out. }
    % \hauke{Multi goal optimization is a method to optimize multiple goals. Even if not done in a lot of 'traditional; traffic modeling work it is becoming a default practice.} 
In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These address the problems of their specific subfields.  
    AV motion design predominately tries to solve the safety of AVs, achieving  better than human levels of safety. Traffic regulation research favors network efficiency, without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Transportation regulations nowadays turned to sustainability. AV service design prioritizes the optimization of the efficient use of all AVs.  Human needs are multi-goal, therefore urban rural infrastructure design addresses many goals. Livable cities, and transport, cannot be described in narrow single  goal terms. We propose the good practice to use (bayesian) multi goal optimzaton for simulations that acknowledge multiple goals. 
    % This paragraph: Multi-goal optimization can be one possible method that understands the trade-offs between these goals and move towards these goals through the combination of all three aspects
    % This paragraph: We offer an example to elaborate on the promises of such methods: the tensions between AVs as commercial products versus AVs as public infrastructure.
    % Because of the oftentimes conflicting goals, it can be hard to balance them, and understand how adapting them influences the cities at a fine-grained level. 
    % Some multi-goal-optimization limitations are resolved meanwhile, and therefore it can become a tool for policy optimization. A few examples of Bayesian multi goal traffic optimization, are promising direction \cite{Schultz2018-lo, Liu2020-et, Tay2022-zg, Dandl2021-dn}. 
 
\end{itemize}



% \subsubsection{An Example}



% \qian{This paragraph: There is a need to understand when and how AVs need special considerations during city planning.}
% \placeholder{AVs impact cities everywhere throughout the city all at once. e.g., it's both micro-mobility, public transportation hub, etc....}
% % The outspread, dominating impact of AVs in cities influences cities wholistically, unlike for example addition of public transport hubs. 
% Adding new train stations, and bus deposits is influencing transportation hot spots which are carefully planned. Only a few, often governmental transport agencies, have to coordinate. 
% Autonomous vehicles for transport of passengers and goods, on the other hand, will operate in most city streets. Presumably, dozens of competing providers, will occupy space. These providers build their AVs on different technology, with various business models, and visions for the future. 
% Therefore, these AVs will pose greater complexities in integrating across the whole street network and neighborhoods, where careful multi-stakeholder planning can hardly occur. 

The existing and proposed methods complement and complete each in a rich method space. Insights represented inside Transgenic Twins, combined with insights from Citizen Led City-AV-Policy Design can, with novel multi goal optimization techniques, help to find the Pareto optimal configuration of the city, and then policymakers can use subjective criteria and deliberation to decide for the best compromise. 





\section{Discussion: What is needed from government, industry, and academia?}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated and participatory city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. 
%, as it allows for the most flexibility and consolidation. 

%\subsection{Requirement: Open Data, Simulators and Standards}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. Data sharing platforms could also facilitate communication and collaboration between different stakeholders, making it easier to identify potential conflicts or issues. Finally, we suggest developing integrated design guidelines and standards that cover all aspects of AV design, city infrastructure, and policy can help ensure that all designs are compatible with each other and contribute to the goals of better cities. These guidelines and standards could be developed collaboratively by designers, policymakers, and other stakeholders and could be used to evaluate and approve new AV designs, infrastructure plans, and policy proposals.

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. HCI should step ahead with the development of such methods and tools.

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote citizen-led and integrated approaches, specialized field expertise is necessary, we do not see participatory methods and holistic simulators as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v8.tex <==
\section{Introduction}
% Title+  Introduction: 1 page


% This paragraph: The great promises of AVs = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Driverless vehicles (commonly referred to as Autonomous Vehicles, AVs) promise to improve cities in ways that would not have been possible otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
They can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighborhoods~\cite{Gilbert-Sociotechnical}. 
They can reduce congestion and cruising-for-parking, hence decreasing vehicle emissions~\cite{Rojas-Rueda2017-xl}. % by coordinating with each other and smart city infrastructure
AVs' promises of safer, more equal, more sustainable, or more livable cities have excited scholars and innovators for years.

% This paragraph: Realizing these promises requires considering AVs, cities, and policies simultaneously.
Yet driverless vehicles' societal benefits are far from guaranteed; Realizing them requires not just thoughtful AV driving behavior design, but urban design and policy innovations~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019-gn, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Making AVs available to the public alone involves complex policy questions (e.g., liability, privacy, insurance)~\cite{fagnant2015preparing} and potential city-scale infrastructural changes (e.g., should autonomous food-delivery robots use new dedicated lanes?~\cite{food-delivery-robot-bikelane-wired}), much more so in realizing AVs' ambitious promises of better cities. 
% \hauke{This example is somehow throwing me off. }
% Why? If you don't like it, feel free to change to a different one.
% much more so in making AVs catalysts of safer, more equal, more sustainable, or more livable cities.
Prior work, therefore, has argued for considering AV design, city planning, and policy making simultaneously~\cite{Matowicki2020-vy,Aoyama2021-jj,Duarte2018-wg,OToole2020-so,Freemark2020-ms,Staricco2019-gn}. 

% This paragraph: Considering AV/city/policy simultaneously is easy to say than done. They form a knot.
But how? 
AV, city, and policy designs are not just connected. They form a difficult ``\textit{knot}''~\cite{Gilbert-Sociotechnical,Wu2018-oy, Brozynski2022-yv}:
% It requires designers to confront the three-way ``\textit{chick-and-egg}'' relationships among them 
Changes to any one of the three---AVs' driving pattern, urban design, or traffic law---must be compatible with the other two to work; 
Meanwhile, changes to any of them also change the other two.
Taking a lesson from earlier HCI work~\cite{policy-knot}, we argue that the path towards better AV cities is \textit{not} as a linear process of matching city designs and policies with AVs' technological innovations, but an iterative prototyping process: Innovations happen step-wise as the ``\textit{knot}'' of AV, city, and policy design unwinds and reties, loosens and tightens.

% This paragraph: This paper takes this knot relationship as a starting point, and helps better address this knot and promote innovation by 1) tracing the policy knot, 2) understanding need for new method
\textbf{This paper takes the knot-like entanglement among AV, city, and policy design as a starting point and asks: How can innovators innovate AVs, urban design, and policies simultaneously and productively?}
This paper has two parts.
First, we trace how the AV-city-policy ``\textit{knot}'' is tied. We map out the interconnections among the many AV, city, and policy design decisions based on a literature review across human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, operations research, economy, and philosophy.
Through this map, we hope to help innovators identify potential AV design constraints and opportunities across the traditional bounds of AV design, urban planning, and law/policy.
% By tracing how the AV-city-policy design ``\textit{knot}'' is tied, this map helps designers identify relevant design issues across traditional disciplinary boundaries across AV design, urban planning, and legal and policy design. % 

Next, we explore how innovators might simultaneously prototype AV, city, and policy innovations. 
Synthesizing existing prototyping methods for each, we identify key barriers in combining these methods for simultaneous AV-city-policy prototyping: (1) Organizational barriers to collaborative AV-city-policy design, (2) computational barriers to multi-granularity AV-city-policy simulation, and (3) different assumptions and goals in AV-city-policy optimization.
We discuss two broad approaches that can potentially address these challenges, namely ``\textit{ML-enabled low-fidelity AV-city-policy simulation} and ``\textit{participatory optimization design}''.
Taken together, this work aspires to catalyze a more principled discussion around \textit{how} AV designers, urban planners, and policymakers can work together to shape future cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Mapping AV, City, and Policy Design Issues}\label{sec:rw}
% This chapter is entirely Related Work (“What do other people think so far”?).
% Our contribution is merely organizing related work.
% Length budget: 2 pages of texts + 1 figure.


% This paragraph: AV, city, policy designs needs coordination, because any driving behavior, city, and policy designs need coordination. The components are the same.
 \input{fig_rw_interactions}
% \vspace{3pt}\noindent
% \textbf{The design choices around AV movement, AV services, city infrastructure, and policies are inherently interrelated.~}

In this chapter, we trace how the AV-city-policy ``\textit{knot}'' is tied~(Figure~\ref{fig:interactions}.) The connections among the three echo the inherent connections among any vehicle's driving behavior design, city planning and infrastructure, and policies. 
From top to bottom: \textit{Civil rights laws and policies}\footnote{This paper focuses mainly on US law and policies. This is a limitation of this work.} set rules that apply to all players in transportation. For example, they require car companies and their designs to allow free sharing of car-repair-related data~\cite{Robertson2020-uq}; they mandate that cities have certain amount of accessible parking and ride-sharing services have certain amount of accessible vehicles~\cite{Reck2018-sq, ADA_National_Network2018-bq}. 
\textit{Traffic regulations} instruct how vehicles and people should move (e.g., that all vehicles should yield to blind pedestrians and stop for school buses), % e.g., pedestrians law, school bus stopping law, clean ice and snow, yield to blind pedestrians, etc.
while \textit{transportation regulations} set rules and incentives related to road use and vehicle use (e.g., authorizing protected planes for bikes and scooters~\cite{Pierce2022-vq}.) % e.g., safety and accidents, auto insurance law, highway law, accessible parking mandates, electric vehicle subsidies, micromobility vehicle laws (e.g., protected lanes for scooters and bikers).
Within these legal and regulatory bounds (red arrows in Fig~\ref{fig:interactions}), AV designers design algorithms to instruct how their AVs move in relation to city infrastructure and other actor on the road (\textit{AV motion design}); AV service designers create additional rules and incentives related to such movements (e.g., via dynamic pricing~\cite{Kaddoura2020-vw}).
Good designs and services, after proven effective, could change transport infrastructure and even become policy mandates (green arrows in Fig~\ref{fig:interactions}, e.g., the wide adoption of ride-hailing services led to dedicated guest boarding zones at airports).
% With urban infrastructure, we refer to transport infrastructure such as roadway features and traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. 

This map reaffirms that realizing AVs' societal benefits \textit{requires} the coordinated innovations of AVs, cities, and policies. 
Empirical evidence from small-scale AV trials and large-scale traffic simulations agree~\cite{Soteropoulos2019-tw,Sperling2018-vk, Freemark2020-ms, Nacto2019-pe,Riggs2019-lx, Niroumand2023-an,Staricco2019-gn,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
For example, reducing congestion requires not only efficient AV navigation algorithms, but AV services, policies, and city infrastructure that incentivize shared rather than personally-owned AVs~\cite{Campbell2018-rr, Sanguinetti2019-de, Kaddoura2020-vw}.
Making future cities more accessible to people with mobility disabilities needs more than accessible AVs.
Incorporating accessible AVs into public transport services can radically scale up AV's accessibility benefits, while corresponding laws and policies could help minimize risks (e.g., by mandating blind driver boarding zones, or standardized way finding beacons)~\cite{Reck2018-sq, ADA_National_Network2018-bq,Ustwo2015-ck}.
% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
% According to a review study on AV modelling work, in the absence of policy intervention, the use of autonomous vehicles is likely to increase overall as they offer greater convenience over mass transportation~\cite{Soteropoulos2019-tw}.
% To fully realize the promised benefits of AVs, it is, therefore, crucial to implement AV-specific policies. Literature has suggested policies to mitigate the potential negative impacts of AVs, that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}, and promoting benefits such as ensuring a minimum number of accessible AVs. 


 % (e.g., when AVs stop or accelerate)
  % (e.g., AV ride-sharing)
   % (e.g., road signs, public cameras and sensors)
   % s (e.g., how pedestrians are supposed to move) 
    % (e.g., when drivers stop or accelerate)
    % (ride-sharing)



\section{Exploring How to Design AVs, Cities, and Policies Simultaneously}\label{sec:proposition}
% This chapter is half Related Work (existing methods) and half our new ideas/contributions (iCAP-- “What do you argue and what’s the evidence?”)
% Length budget: 2 pages of texts + 1 figure.

So far, we have argued that AV, city, and policy design issues are inherently entangled and should be considered simultaneously. But how? This chapter explores the methods and tools that allow innovators to prototype AV, city, and policy innovations simultaneously. 
% By tracing how the AV-city-policy design ``\textit{knot}'' is tied, this map helps designers identify relevant design issues across traditional disciplinary boundaries across AV design, urban planning, and legal and policy design. % 

\subsection{Existing Methods for AV, City, and Policy Design}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}

% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 

%%%%% =====  stuff moved from chatper 2 to here START ====== %%%%
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }
% \qian{trade-offs across multiple goals}
% Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}
% \qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
% \placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
% most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
% Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
% Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

% \qian{This paragraph: As a result, people call for coordination among agencies.}
% While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  
%%%%% =====  Stuff moved from chatper 2 to here END ====== %%%%


% This paragraph: Current methods are isolated (AV design - 3D simulation on basic road conditions, road trials; city planning - low-detail maps and patterns, PD prototyping; urban infrastrcture - simulaion . Give examples.
AV, city, and policy design today shares few common design methods~\cite{Rouse2021-ph,Yang2019-nr}.~For example:
% As \citet{Yang2019-nr} note, there is a lack of decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textit{AV driving behavior design uses road trials and microscopic VR driving simulations.~} Designers train AV driving behavior machine learning models using datasets that capture how people drive on today's roads or test roads~\cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja,Dowling2022-wu,Suo2021-vm}. Noteably, AV designers and researchers have also become interested in Virtual Reality (VR) driving simulation studies~\cite{Dosovitskiy2017-jb,NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp,driving-like-you}. Rather than messy real-world driving conditions and interactions, these studies capture in rich detail drivers' naturalistic behaviors in controlled, simple road situations (e.g., merging on highways). However, these simulated road situations typically only involve 1-2 drivers, with few, if any, other road users (e.g., other vehicles, pedestrians)~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe,Yang2021-oz, Pell2017-al}. It is also unclear whether and how AV designers actually incorporate these insights into AVs' driving behavior models.
% In these studies, designers observe how people ``\textit{drive}'' alongside an AV in prototypical road situations (e.g., merging on highways), and revise AVs' driving behavior models according to the observed interactions. Noteworthingly, these models are trained on data that reflect today's roads and cities, and the VR simulations are typically % -----  in VR environments where  are also present. By investigating 
    % \item These simulation environments typically are simple road situations rather than real-world driving conditions; Most have few if any pedestrians or other types of vehicles, and do not use AI models to simulate AV behavior.~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz, Pell2017-al};
    % \item .   and microscopic driving simulation, is used to gather insights to enable AVs better coordinate with other road users at crossroads


% These research methods incorporate human considerations, but not policy or infrastructure. 
% Due to the limitationThese simulation environments typically only include simple road situations, such as prototypical crossroads and parking space, with few if any pedestrians or other types of vehicles.s of technical AV testing, researchers devised Wizard of Oz methods for human-AV experiments on real roads~\cite {Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}.  Many simulations focus on AV behavior only, with often basic road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}, due to limitations researchers devised VR simulators~\cite{Goedicke2022-ys}. 
% Testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}.  
    \item \textit{Urban planning uses design patterns and participatory design.~} Urban planners heavily rely upon established design patterns~\cite{alexander1977pattern}. They then apply or update the patterns using maps, geographic information systems, or street cross-profiles~\cite{Riggs2017-hm,Lee2022-vd, Remix_by_Via2021-vm,Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}.
% Geographic information systems manage access to increasing layers of information \cite{Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}.
In recent years, participatory design (PD) has gained popularity, incorporating citizen needs and preferences into the process of urban design and prototyping~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}.

% low-detail maps and patterns, PD prototyping
    \item \textit{Urban infrastructure design and policy-making uses design patterns and macroscopic traffic simulation.~}Urban infrastructure design also relies on established design patterns and guidelines~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. Additionally, designers~\cite{Zhang2022-uh, Dembski2020-gk} and policy makers~\cite{White2021-vo, Charitonidou2022-zg} use computational simulations to identify optimal infrastructure designs, for example, identifying the bus lane arrangement that causes minimal traffic disruption. % they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
    \item \textit{Traffic law design inherits prevailing law-making processes and uses quantitative modeling, regulatory sandboxes, and more.~}AV regulation is an active research topic in legal fields. Its approaches so far are largely reminiscent of traditional traffic law-making approaches. For example, conventional transportation research uses mathematical modeling to address policy questions (e.g., how tolls and fines impact traffic flows). Yet, some criticized that this approach assumes a top-down execution of proposed policies and is too detached from the messy policy-making cycles in practice.~\cite{Marsden2017-lu}. In response, lawmakers have adopted participatory approaches in making AV policies~\cite{van2022politics,lyons2022driverless}. They have created ``\textit{regulatory sandbox}'' for AV safety regulations as a means of providing a flexible regulatory environment for companies to iteratively test emerging technologies and business models~\cite{oecd2020-regulatory-sandbox,burd2021regulatory, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}. 
   % To overcome these  limitations, methods that enable policymakers themselves to make good decisions through data from the environment and citizens are proposed~\cite{White2021-vo, Marcucci2020-qg}. 
% Participatory methods have been part of policy-making since the beginning, through officials, agencies, and organized interest groups. Progress on how to scale up these approaches, better recognize efforts, and align various interests is still ongoing~\cite{Blomkamp2018-yg, Blomkamp2022-be, Oostveen2004-lk}.  % <- These are not AV-related policy work, right
     % \placeholder{Pilots in isolated regions to test AV safety. \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}}
\end{itemize}


% This parargaph: Some methods have the potential of supporting multiple designs. But no one acted on it.
Notably, researchers have argued that city-level simulation tools have the potential to support simultaneous urban infrastructure and policy design~\cite{Marcucci2020-qg,White2021-vo,Riggs2020-yc}. 
Interestingly, no research that we are aware of further explored this possibility or created such tools. 
%For example, %\citet{Haegler2021-xv} argued that VR microscopic driving simulations might also help prototype infrastructure and policy re-development. \hauke{VR microscopic driving simulation is not something I came across. The link is for a city simulation for architecture only. I don't know about a specifc research that argues this.}
% \citet{Marcucci2020-qg} and \citet{White2021-vo} argued that simulation tools have the potential to support simultaneous urban infrastructure and policy design.
% \citet{Riggs2020-yc} explored this idea in designing livable AV-infused cities, outlining how simulation tools can support both road space allocation and policy design.
Beyond traditional traffic simulations, ``\textit{digital twins}'' can appear a particular promising, albeit emerging, tool~\cite{shahat2021city}. Digital twin refers to a dynamic 3D model that mirrors a city's physical form and contains a city's information (e.g., street network space syntax, commuting patterns, the socioeconomic data of a neighborhood) throughout its lifecycle.
Digital twin's rich data allows for machine learning models that can answer ``\textit{what if}'' policy questions~\cite{nochta2021socio}.
Its comprehensive data offers a rare platform to support collaboration across city and policy design spheres and among the various stakeholders of the city~\cite{hamalainen2020smart}. 
% Dembski, F.; Wössner, U.; Letzgus, M.; Ruddat, M.; Yamu, C. Urban digital twins for smart cities and citizens: The case study of Herrenberg, Germany. Sustainability 2020, 12, 2307. 


% This paragraph: People have started designing policy and cities together
% A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
% There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 


% hauke:
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …


% \input{fig_rw_methods}

\subsection{Challenges in Designing AV, City, Policy Simultaneously}

Our analysis of existing methods also reveals a number of more significant barriers in prototyping AV, city, and policy design simultaneously.


\vspace{3pt}\noindent
\textbf{Different organizations own the design decisions of AVs, different components of city infrastructure, and different regulations.~}
Let us start with the biggest elephant in the room: that different private corporations and government agencies own the various AV, city, and policy design decisions. 
While multiple AV design researchers argued that small tweaks to traffic lights and road signs could significantly improve AV's computer vision model performance and driving safety~\cite{Niroumand2023-an,Gilbert-Sociotechnical,Riggs2019-lx, Nacto2019-pe}, they simply do not have the decision-making power in adopting these design proposals.
Designing AV, city, and policy simultaneously requires innovators to navigate the related political and organizational complexities, and it is not an easy task. 

% Further, in order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}
% If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

% This paragraph: acknowledging the politics involved in designing the trio simutanously: 
% AV, city, and policy design involve complex political processes that are often not fully acknowledged. The design of infrastructure, in particular, is embedded with politics and can shape the power dynamics of a society. As Winner argues, "the design of technology is itself a profoundly political activity" \cite{Winner1985-hp}. Similarly, Marsden \cite{Marsden2017-lu} argues that policymaking studies often overlook the complexities of the policymaking cycle. 
% Bringing together these different sectors to cooperate in designing AVs, cities, and policies requires recognizing and addressing these political complexities and is not an easy task.
% }\qian{For example, we only see democratic/participatory approaches to AV design used in policy/city design contexts, but not in AV company design contexts.}
% \hauke{I have a bit of that in line 187  \cite{Marsden2017-lu} argues that the field of policymaking study do not acknowledge the comlexities in the policy making cycle. Other than that I do not have a direct source in mind I read. https://www.taylorfrancis.com/books/mono/10.4324/9780203857557/politics-mobility-geoff-vigar (not read). We could also reference Winners bridges to briefly acknowldge that infrastructure (datasets, algorithms and policy too)  has built politics in.}

Moreover, driverless vehicles are far from homogeneous. (Think autonomous long-haul trucks, autonomous commercial drivers' vehicles, autonomous scooters for last-mile transportation, and food delivery robots.) Therefore, AVs will likely achieve wide adoption at different times, use different parts of the city infrastructure, and operate under different traffic and transportation regulations (e.g., AV scooters will likely be subject to micro-mobility laws, while low-haul trucks will be to Hours of Service regulations in the U.S.)
The wide variety of future AVs will add further complexities to the already complex AV-city-policy design landscape.


\vspace{3pt}\noindent
\textbf{Prototyping AV-human-city interactions both at individual and societal levels is computationally (too) demanding.~}
AV, city, and policy design operate at different scales, using varying levels of abstraction.
Take simulation as an example. 
Designing AV driving behavior models needs microscopic simulations. These simulations depict interactions among individual vehicles and pedestrians, typically in isolated encounters within short periods of time (e.g., when merging on highway)~\cite{Saidallah2016-zx}. 
City infrastructure and policy design need macroscopic simulations. They focus on traffic flows, their longitudinal patterns, and potential holistic impact on the city (e.g., would AV navigation patterns catalyze social inequalities across neighborhoods over time?~\cite{Gilbert-Sociotechnical}.) %\qian{Isn't digital twins an exception to this (it does both individual vehicle level and traffic flow level simulations)?}
Combining these simulations appears a promising approach to prototyping AV, city, and policy design simultaneously. However, this approach is computationally highly demanding.
Recent research has applied this integrative simulation approach to compare the impact of two scenarios of electric vehicles’ charging locations on charging demand~\cite{nochta2021socio}. It is unclear whether it is computationally feasible to simultaneously simulate multiple more complex AV, city, and policy design changes. 
% of varying granularity levels means that designers must wrestle with all of the above human-AV-environment interactions at the same time. Such integrative methods are likely to be cognitively demanding for the designers and computationally demanding for their simulation systems. 
% \qian{How is our method immune to this problem?}
% Nochta et al. illustrated the evaluation of different scenarios of electric vehicles’ charging locations and the cross-sectoral impacts through the city digital twin

% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }
% AVs are like micromobility and trains simultaneously
% \subsubsection{What is novel about AVs in terms of planning complexity?}
% Autonomous vehicles represent a new frontier in urban and rural planning complexity.
% In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
% Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
% Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  
% In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}. 
% Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
% As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.

% This paragraph is summarizing the proposed methods.
% Current scope-limited AV tests, complementary simulation studies, and analysis of natural human driving do not fully capture the effects that AVs will have at scale. They also do not consider the opportunities for re-designing urban and rural infrastructure or address nuanced human preferences.

% This paragraph: These methods can lead to results that are difficult to synthesize, because (2) they work under different assumptions and towards different goals
\vspace{3pt}\noindent
\textbf{Different assumptions and design goals underlie different AV, city, policy design efforts.~}
Even if one can simulate AV, city, and policy design changes in a shared simulation system, it can be difficult to align their design goals.
AV, city, and policy design methods often operate on different assumptions and pursue different goals.
In urban infrastructure design, driverless vehicles are often part of the public infrastructure. Innovators optimize AV, policy, and city design towards maximum public good, for example, less congestion~\cite{Metz2018-jn}, easier road maintenance~\cite{Gilbert-Sociotechnical}, and less environmental impact~\cite{Felipe-Falgas2022-dz}.
In AV motion design, AVs are privately-owned or company-owned commercial products that provide customers value. 
These varying assumptions led to insistent debates around, for example, how AVs should move, who has a say in how AVs should move, and how AVs fit into the public sphere~\cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
% \qian{I know I wrote this, but I am not sure if these two sentences are true... They read like sweeping arguments. Will come back to this.} \hauke{I can see why you do not buy this. This unsureness about how it actually will unfold is discussed in the Ju Nissenbaum Paper. \url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3875889}
% They identigy three archetypes of AVS: autonomous vehicles—advanced driver-assist systems (private), fully driverless cars (AV service), and connected cars. I am not certain about the connected cars though. cars of the other two categories can be conneted to?}
% \placeholder{Competing ownership visions (individually owned, service owners, governmental ownership) , different technology (connected via radio waves, high resolution sensor \&ml based)}





% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 




% Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} 
% For infrastructure design, guidelines, and design patterns were established over time~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. These demand an update with specific AV patterns~\cite{Nacto2019-pe}.  
% Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
% Participatory design methods are used in multiple areas to understand people's needs, in urban planning, tactical urbanism, citizen-led prototyping is becoming popular and shows unsatisfied needs by conventional planning~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}. Tactical urbanism has informed policymaking, but not AV design.

% Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
% There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019-gn, Meeder2017AutonomousVP, Acheampong2021-ql}. 


%\subsection{Our Proposal: Integrative City-AV-Policy Simulation (iCAPS)}
% \hauke{Complete, Citizen Centered City Simulation (4CS)}
% \hauke{Complete, Citizen Centered City AV Replicator (4CAR)} (or renderer)
\subsection{Proposing methods to untangle City, AV and Policy Design}

% We identify two promising approaches. \textit{Citizen led city-AV-policy design} can help to ease value tension through democratic (participatory) processes. \textit{Holistic simulations} can help anticipate the opportunities and breakdowns/tensions that might emerge from the interactions across urban/rural infrastructure, AVs, and regulation.

To address design problems related to cities, AVs, and policy, it's important to acknowledge that different stakeholders own the decision-making process in each of these fields. It's unrealistic to expect designers to acquire the necessary expertise and authority in all three areas. Therefore, continuous collaboration among stakeholders is a necessity.
Given political, business and organizational difficulties, we stress here that this type of collaboration is not unheard of. Mobility service startups and vehicle companies are already testing novel concepts with a few cities. 
We identify two methods below that can be used by cities, AV designers and policymakers to work together on these issues and catalyze these collaborations.


\begin{itemize}
\item \textit{AV Neighborhood Prototyping:~}

Urban prototyping, offers a wealth of possible methods for planning AV by doing prototyping in the real physical space. 
We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for AV prototyping. We see potential to create hybrid methods, using Wizard of Oz to design AV motion and traditional participatory design to design policy and AV Service, all simultaneously. % WoZ with simulated AVs is most useful to simulate individual interactions with vehicles in individual streets. %Just as with tactical urbanism, 
AV Neighborhood Prototyping will be most effective with people from their relevant neighborhoods and enable them to influence design choices such as where AV pick up spots and delivery stations shall be placed. 

\item \textit{Nuanced AV Motion Design:~}
%this paragraph describes one potential citizen led CAPS experiment
A change in traffic regulations just on AV provider's request without sufficient evidence is unlikely. To prove that, new av motion, which requires change in regulations, is satisfying user needs, a VR driving study could be conducted that asks people to fine-tune AV motion, traffic regulations, and urban infrastructure while assuming various perspectives such as a passenger, pedestrian encountering a vehicle, and resident in a neighborhood. The outcome of such a study will unravel different preferences for AV motion (e.g., AV acceleration values), urban infrastructure (e.g., width of AV lane) and traffic regulations (e.g., AV speed limit). With such a study, we can go beyond current AV motion design, which imitates human \textit{driver} behavior and takes regulations as well as infrastructure as fixed.
%this paragraph describes a second potential citizen led CAPS experiment
\item \textit{Moral Cities:~}:

A comparable study, targeting transportation regulation, could explore future ethical AV dilemmas, by conducting an online experiment; participants provide input on complex questions related to AV traffic routing and zoning that have implications for infrastructure. These questions might include determining whether AVs should travel through primarily low-income areas or sightseeing districts when efficiency is equal, who should bear the burden of noise and emissions. Additionally, the study could investigate whether AVs should park in designated slots outside the city to free up space for other uses or at curbside in the city to minimize wait times for pick-up.
\end{itemize}
The three examples presented above for citizen-led city AV-policy design can inform and assist policymakers and AV developers in coordinating actionable human preferences and resolving \textit{seemingly} trolley-problem-like conflicts.

\subsubsection{Holistic Simulation}


Simulators are necessary because only they allow for the evaluation and optimization of future transportation policies, city designs and AV behavior in a safe, controlled, and cost-effective environment. 
Holistic city simulators allow various stakeholders to engage across disciplines, but they allow policymakers to simulate how AV service and motion design might react to regulation and infrastructure changes. Do the implemented changes lead to the desired effects, will they cause unintended consequences, will the learning and automated AVs evade them?



\begin{itemize}
    \item \textit{Transgenic Twin:~}  To make Digital Twins, which are data-based replicas of cities components and processes, useful for prototyping AVs, city infrastructure, and policies simultaneously they need to be equipped with the appropriate design tools to manipulate AV behavior, regulations, and infrastructure. Nowadays, these tools are not found in digital twins but only in the specific tools such as city planners. 
    
    
    Also, digital Twin assets are often static. We need to either include HD Maps, usually expensive proprietary assets, or develop tools which, for example, transfer point clouds of city scans into modifiable geometry of houses, streets, and traffic signs. Machine learning methods that can detect bounding boxes of houses, street and traffic signs, already used for AV motion design, can automate these processes. 
    
    To simulate the complex processes of the city,  rather than hand modeling, we can learn behavior from the twins rich data~\cite{Suo2021-vm}. Once processes and components are turned flexible, react with each other in a complex model, we can start to play with the simulated DNA of the city,  engineering preferable twins.   
    \item \textit{Multi-Goal Optimization}:~   \hauke{I am tending to favour to leave multi goal simulation out. }

In practice, many simulations exist for sub-problems in their fields. In  these problem areas, different goals are prioritized. These address the problems of their specific subfields.  
    AV motion design predominately tries to solve the safety of AVs, achieving  better than human levels of safety. Traffic regulation research favors network efficiency, without negatively impacting safety. In civil rights laws, equity with questions of accessibility is prioritized. Transportation regulations nowadays turned to sustainability. AV service design prioritizes the optimization of the efficient use of all AVs.  Human needs are multi-goal, therefore urban rural infrastructure design addresses many goals. Livable cities, and transport, cannot be described in narrow single  goal terms. We propose the good practice to use (bayesian) multi goal optimzaton for simulations that acknowledge multiple goals. 

 
\end{itemize}


The existing and proposed methods complement and complete each in a rich method space. Insights represented inside Transgenic Twins, combined with insights from Citizen Led City-AV-Policy Design can, with novel multi goal optimization techniques, help to find the Pareto optimal configuration of the city, and then policymakers can use subjective criteria and deliberation to decide for the best compromise. 





\section{Discussion: What is needed from government, industry, and academia?}
% Discussion (“so what?”)
% Discussion: ⅓ page
With the conclusions drawn in this short paper, we hope to induce the development of more integrated and participatory city design and AV policy prototyping tools. We proposed simulation as the most promising ground for such tools. 
%, as it allows for the most flexibility and consolidation. 

%\subsection{Requirement: Open Data, Simulators and Standards}
We find that holistic simulators cannot be built without open sharing of data, models, as well as standardizing interfaces. While open-source efforts of research data have improved, few simulators are open sourced and many urban design tools are proprietary technology. Further, most datasets collected by shared mobility services and AV developers are not accessible openly. These data sources would be extremely valuable for policy making and building policy simulations. We recommend policymakers to enact policy to allow them to access data from AV motion design. Data sharing platforms could also facilitate communication and collaboration between different stakeholders, making it easier to identify potential conflicts or issues. Finally, we suggest developing integrated design guidelines and standards that cover all aspects of AV design, city infrastructure, and policy can help ensure that all designs are compatible with each other and contribute to the goals of better cities. These guidelines and standards could be developed collaboratively by designers, policymakers, and other stakeholders and could be used to evaluate and approve new AV designs, infrastructure plans, and policy proposals.

% Call for collaboration
We direct our call for development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human centered design methods and success developing novel software based prototyping tools. HCI should step ahead with the development of such methods and tools.

% Limitations
Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. Even though we promote citizen-led and integrated approaches, specialized field expertise is necessary, we do not see participatory methods and holistic simulators as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page



%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}


==> archive/v9.tex <==
\section{Introduction}
% Title+  Introduction: 1 page


% This paragraph: The great promises of AVs = more livable/efficient, sustainable, and equitable cities. 
% Subtext: despite the many problems/challenges in connecting policy/AV/city design (as we will describe in the next paragraph), it's still worth pursuing.
Driverless vehicles (commonly referred to as Autonomous Vehicles, AVs) promise to improve cities in ways that would not have been possible otherwise~\cite{World_Economic_Forum2020-ox,Appleyard2014-ph, The_Intelligent_Transportation_Society_of_America2021-ew}. 
AVs can reduce crashes, deaths, and injuries~\cite{Golbabaei2020TheRO,PETTIGREW201964,fagnant2015preparing}. 
They can allow easier travel for the elderly, the handicapped, and those living in poorly-connected neighborhoods~\cite{Gilbert-Sociotechnical}. 
They can reduce congestion and cruising-for-parking, hence decreasing vehicle emissions~\cite{Rojas-Rueda2017-xl}. % by coordinating with each other and smart city infrastructure
AVs' promises of safer, more equal, more sustainable, or more livable cities have excited scholars and innovators for years.

% This paragraph: Realizing these promises requires considering AVs, cities, and policies simultaneously.
Yet driverless vehicles' societal benefits are far from guaranteed; Realizing them requires not just thoughtful AV driving behavior design, but urban design and policy innovations~\cite{Faisal2019UnderstandingAV, Acheampong2021-ql, Metz2018-jn,Yigitcanlar2019DisruptiveIO, Golbabaei2020TheRO, Meeder2017AutonomousVP, Staricco2019-gn, PETTIGREW201964, Bobisse2019-wj, Gonzalez-Gonzalez2019-cn, Rouse2021-ph, Legacy2019-me,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
Making AVs available to the public alone involves complex policy questions (e.g., liability, privacy, insurance)~\cite{fagnant2015preparing} and potential city-scale infrastructural changes (e.g., should autonomous food-delivery robots use new dedicated lanes?~\cite{food-delivery-robot-bikelane-wired}), much more so in realizing AVs' ambitious promises of better cities. 
% \hauke{This example is somehow throwing me off. }
% Why? If you don't like it, feel free to change to a different one.
% much more so in making AVs catalysts of safer, more equal, more sustainable, or more livable cities.
Prior work, therefore, has argued for considering AV design, city planning, and policymaking simultaneously~\cite{Matowicki2020-vy,Aoyama2021-jj,Duarte2018-wg,OToole2020-so,Freemark2020-ms,Staricco2019-gn}. 

% This paragraph: Considering AV/city/policy simultaneously is easy to say than done. They form a knot.
But how? 
AV, city, and policy designs are not just connected. They form a difficult ``\textit{knot}''~\cite{Gilbert-Sociotechnical,Wu2018-oy, Brozynski2022-yv}:
% It requires designers to confront the three-way ``\textit{chick-and-egg}'' relationships among them 
Changes to any one of the three---AVs' driving pattern, urban design, or traffic law---must be compatible with the other two to work; 
Meanwhile, changes to any of them also change the other two.
Taking a lesson from earlier HCI work~\cite{policy-knot}, we argue that the path towards better AV cities is \textit{not} as a linear process of matching city designs and policies with AVs' technological innovations, but an iterative prototyping process: Innovations happen step-wise as the ``\textit{knot}'' of AV, city, and policy design unwinds and reties, loosens and tightens.

% This paragraph: This paper takes this knot relationship as a starting point, and helps better address this knot and promote innovation by 1) tracing the policy knot, 2) understanding need for new method
\textbf{This paper takes the knot-like entanglement among AV, city, and policy design as a starting point and asks: How can innovators innovate AVs, urban design, and policies simultaneously and productively?}
This paper has two parts.
First, we trace how the AV-city-policy ``\textit{knot}'' is tied. We map out the interconnections among the many AV, city, and policy design decisions based on a literature review across human-computer/robot interaction (HCI/HRI), transportation science, urban studies, law and policy, operations research, economy, and philosophy.
Through this map, we hope to help innovators identify potential AV design constraints and opportunities across the traditional bounds of AV design, urban planning, and law/policy.
% By tracing how the AV-city-policy design ``\textit{knot}'' is tied, this map helps designers identify relevant design issues across traditional disciplinary boundaries across AV design, urban planning, and legal and policy design. % 

Next, we explore how innovators might simultaneously prototype AV, city, and policy innovations. 
Synthesizing existing prototyping methods for each, we identify key barriers in combining these methods for simultaneous AV-city-policy prototyping: (1) Organizational barriers to collaborative AV-city-policy design, (2) computational barriers to multi-granularity AV-city-policy simulation, and (3) different assumptions and goals in AV-city-policy optimization.
We discuss two broad approaches that can potentially address these challenges, namely ``\textit{ML-enabled low-fidelity AV-city-policy simulation} and ``\textit{participatory design optimization}''.
Taken together, this work aspires to catalyze a more principled discussion around \textit{how} AV designers, urban planners, and policymakers can work together to shape future cities.
% \qian{we should add a note the laws and policies here have a strong US bias.}
% \hauke{And europe -> western}  % Did we mention any european laws and policies? I was looking throught the list. Not sure. Design and simulation studies were using european context for sure.  % That's method, not law and policy right? I can see GDPR certainly being relevant here. but I don't think we talked about it much.

%Shall we keep the name iCAPS?
% In a comprehensive analysis of related work, we point out that trade-offs and tensions exist in designing and implementing AVs, policies, and urban infrastructure, and these need to be addressed through more holistic approaches. 
% The paper suggests that current methods for AV design and urban infrastructure simulations do not adequately consider the complexity of these issues.
% We conclude that designing policies, road infrastructure, and AVs together can lead to entirely new concepts and solutions for improving cities, and envision a new approach, \newmethodlong (\newmethod) to prototype AV, driving policy, and the necessary urban infrastructure together. 

% While prior work acknowledged the interdependence between AVs, policies, and urban infrastructure, it did not develop anticipatory prototyping methods. As a result, city planners and policymakers can not optimally prepare urban infrastructure and policies for the arrival of AVs. 

\section{Mapping AV, City, and Policy Design Issues}\label{sec:rw}
% This chapter is entirely Related Work (“What do other people think so far”?).
% Our contribution is merely organizing related work.
% Length budget: 2 pages of texts + 1 figure.


% This paragraph: AV, city, policy designs needs coordination, because any driving behavior, city, and policy designs need coordination. The components are the same.
 \input{fig_rw_interactions}
% \vspace{3pt}\noindent
% \textbf{The design choices around AV movement, AV services, city infrastructure, and policies are inherently interrelated.~}

In this chapter, we trace how the AV-city-policy ``\textit{knot}'' is tied~(Figure~\ref{fig:interactions}.) The connections among the three echo the inherent connections among any vehicle's driving behavior design, city planning and infrastructure, and policies. 
From top to bottom: \textit{Civil rights laws and policies}\footnote{This paper focuses mainly on US law and policies. This is a limitation of this work.} set rules that apply to all players in transportation. For example, they require car companies and their designs to allow free sharing of car-repair-related data~\cite{Robertson2020-uq}; they mandate that cities have certain amount of accessible parking and ride-sharing services have certain amount of accessible vehicles~\cite{Reck2018-sq, ADA_National_Network2018-bq}. 
\textit{Traffic regulations} instruct how vehicles and people should move (e.g., that all vehicles should yield to blind pedestrians and stop for school buses), % e.g., pedestrians law, school bus stopping law, clean ice and snow, yield to blind pedestrians, etc.
while \textit{transportation regulations} set rules and incentives related to road use and vehicle use (e.g., authorizing protected planes for bikes and scooters~\cite{Pierce2022-vq}.) % e.g., safety and accidents, auto insurance law, highway law, accessible parking mandates, electric vehicle subsidies, micromobility vehicle laws (e.g., protected lanes for scooters and bikers).
Within these legal and regulatory bounds (red arrows in Fig~\ref{fig:interactions}), AV designers design algorithms to instruct how their AVs move in relation to city infrastructure and other actor on the road (\textit{AV motion design}); AV service designers create additional rules and incentives related to such movements (e.g., via dynamic pricing~\cite{Kaddoura2020-vw}).
Good designs and services, after proven effective, could change transport infrastructure and even become policy mandates (green arrows in Fig~\ref{fig:interactions}, e.g., the wide adoption of ride-hailing services led to dedicated guest boarding zones at airports).
% With urban infrastructure, we refer to transport infrastructure such as roadway features and traffic control devices as well as public transport infrastructure such as transit stops, subways, and other city infrastructure such as public parks or schools. 

This map reaffirms that realizing AVs' societal benefits \textit{requires} the coordinated innovations of AVs, cities, and policies. 
Empirical evidence from small-scale AV trials and large-scale traffic simulations agree~\cite{Soteropoulos2019-tw,Sperling2018-vk, Freemark2020-ms, Nacto2019-pe,Riggs2019-lx, Niroumand2023-an,Staricco2019-gn,Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
For example, reducing congestion requires not only efficient AV navigation algorithms, but AV services, policies, and city infrastructure that incentivize shared rather than personally-owned AVs~\cite{Campbell2018-rr, Sanguinetti2019-de, Kaddoura2020-vw}.
Making future cities more accessible to people with mobility disabilities needs more than accessible AVs.
Incorporating accessible AVs into public transport services can radically scale up AV's accessibility benefits, while corresponding laws and policies could help minimize risks (e.g., by mandating blind driver boarding zones, or standardized way finding beacons)~\cite{Reck2018-sq, ADA_National_Network2018-bq,Ustwo2015-ck}.
% Unfortunately, case studies, simulations and real-world examples of new mobility concepts, e.g., the introduction of on-demand taxis and micromobility services, suggest that these benefits will not unfold without intervention~\cite{Bosch2018-pl, Merlin2019-fb, Marx2022-rm}.
% According to a review study on AV modelling work, in the absence of policy intervention, the use of autonomous vehicles is likely to increase overall as they offer greater convenience over mass transportation~\cite{Soteropoulos2019-tw}.
% To fully realize the promised benefits of AVs, it is, therefore, crucial to implement AV-specific policies. Literature has suggested policies to mitigate the potential negative impacts of AVs, that incentivize AV-sharing and dynamic pricing of curbside parking as well as empty trips~\cite{Sperling2018-vk, Freemark2020-ms, Nacto2019-pe}, and promoting benefits such as ensuring a minimum number of accessible AVs. 


 % (e.g., when AVs stop or accelerate)
  % (e.g., AV ride-sharing)
   % (e.g., road signs, public cameras and sensors)
   % s (e.g., how pedestrians are supposed to move) 
    % (e.g., when drivers stop or accelerate)
    % (ride-sharing)



\section{Exploring How to Design AVs, Cities, and Policies Simultaneously}\label{sec:proposition}
% This chapter is half Related Work (existing methods) and half our new ideas/contributions (iCAP-- “What do you argue and what’s the evidence?”)
% Length budget: 2 pages of texts + 1 figure.

So far, we have argued that AV, city, and policy design issues are inherently entangled and should be considered simultaneously. But how? This chapter explores the methods and tools that allow innovators to prototype AV, city, and policy innovations simultaneously. 
% By tracing how the AV-city-policy design ``\textit{knot}'' is tied, this map helps designers identify relevant design issues across traditional disciplinary boundaries across AV design, urban planning, and legal and policy design. % 

\subsection{Existing Methods for AV, City, and Policy Design}
% \hauke{Feed the examples one by one (rather than copmplexity all at once)
% Write the example you want to communicate and rework back}

% This versatility presents unique challenges that need to be managed across entire cities and regions. 
% The rollout of AVs can happen gradually over time or quickly and spontaneously all at once. Furthermore, AV deployment can occur in individual locations or everywhere simultaneously. Competitors might aggressively compete to segment the market.
% This poses policy challenges that require careful management across a broad range of local complexities. 

%%%%% =====  stuff moved from chatper 2 to here START ====== %%%%
% People know policies, urban infra, AVs are interrelated/mutually influential, they \textbf{should} be considered together. There are the \textbf{trade-offs between these goals} (more livable, sustainable, efficient, and equitable cities)
% e.g., planned vs. self-organized
% Evidence: simulations focus on one goal only
% }
% \qian{trade-offs across multiple goals}
% Realizing AV-infused better cities also requires \textit{trade-offs} between the designs of AV behaviors, policies, and urban infrastructure.
% \qian{Let's unpack each of these questions. It's not intuitive what they mean. Plus, it's not self-evident why "should autonomous vehicles be owned or shared" is an either-or problem; the last paragraph just said that cities have required minimum shared AVs.}
% \qian{This paragraph: Further complicating things is not only the amount of different design choices involved, but that these design choices belong to different agencies.}
% \placeholder{the [4] makes a good argument how optimizing these tradeoffs is conflicting:
% most people prefer utilitarian vehicles in their society that would prioritize the collective good. However most people would only use vehicles that prioritze their own good.
% Thus even for collective good individualism enhancing AVs might be preferrable as only they encourage use.
% Making these choices is up to policy makers, AV companies are anticipated to optimize everything that drives adoption.}

% \qian{This paragraph: As a result, people call for coordination among agencies.}
% While we do not know the reasons for more holistic design and development of AVs, urban infrastructure and policy, in individual workshops, some cross field collaboration happens in workshops that call for cities' AV 'readiness' \cite{Rupprecht2018-qf}. Cities are encouraged to have a seat on AV policy \cite{Nacto2019-pe}, and local policymakers show support for individual AV policies with infrastructure impact \cite{Freemark2020-ms}.  
%%%%% =====  Stuff moved from chatper 2 to here END ====== %%%%


% This paragraph: Current methods are isolated (AV design - 3D simulation on basic road conditions, road trials; city planning - low-detail maps and patterns, PD prototyping; urban infrastrcture - simulaion . Give examples.
AV, city, and policy design today share few common design methods~\cite{Rouse2021-ph,Yang2019-nr}.~For example:
% As \citet{Yang2019-nr} note, there is a lack of decision-making toolkits for integrated design of transport infrastructure and public spaces with consideration of human behavior.

\begin{itemize}[leftmargin=*, itemsep=2pt]
    \item \textit{AV driving behavior design uses road trials and microscopic driving simulations.~} Designers train AV driving behavior machine learning models using datasets that capture how people drive on today's roads or test roads~\cite{Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja,Dowling2022-wu,Suo2021-vm}. Noteably, AV designers and researchers have also become interested in immersive driving simulation studies~\cite{Dosovitskiy2017-jb,NVIDIA_Corporation2023-tn, Amini2021-qu, Jin2018-sw, Craighead2007-vp,driving-like-you}. Rather than messy real-world driving conditions and interactions, these studies capture in rich detail drivers' naturalistic behaviors in controlled, simple road situations (e.g., merging on highways). However, these simulated road situations typically only involve 1-2 drivers, with few, if any, other road users (e.g., other vehicles, pedestrians)~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe,Yang2021-oz, Pell2017-al}. It is also unclear whether and how AV designers actually incorporate these insights into AVs' driving behavior models.
% In these studies, designers observe how people ``\textit{drive}'' alongside an AV in prototypical road situations (e.g., merging on highways), and revise AVs' driving behavior models according to the observed interactions. Noteworthingly, these models are trained on data that reflect today's roads and cities, and the VR simulations are typically % -----  in VR environments where  are also present. By investigating 
    % \item These simulation environments typically are simple road situations rather than real-world driving conditions; Most have few if any pedestrians or other types of vehicles, and do not use AI models to simulate AV behavior.~\cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz, Pell2017-al};
    % \item .   and microscopic driving simulation, is used to gather insights to enable AVs better coordinate with other road users at crossroads


% These research methods incorporate human considerations, but not policy or infrastructure. 
% Due to the limitationThese simulation environments typically only include simple road situations, such as prototypical crossroads and parking space, with few if any pedestrians or other types of vehicles.s of technical AV testing, researchers devised Wizard of Oz methods for human-AV experiments on real roads~\cite {Pettersson2017-wi,Baltodano2015-yf,Rothenbucher2016-ja}.  Many simulations focus on AV behavior only, with often basic road situations \cite{Osorio2011-kj, Kavas-Torris2021-xm, Wang2017-qe, Yang2021-oz}, due to limitations researchers devised VR simulators~\cite{Goedicke2022-ys}. 
% Testing in the physical world, i.e., on real-roads and test beds, takes the urban infrastructure as determinate \cite{Dowling2022-wu}.  
    \item 
    \textit{Urban planning uses design patterns and participatory design.~} Urban planners heavily rely upon established design patterns~\cite{alexander1977pattern}. They then apply or update the patterns using maps, geographic information systems, or street cross-profiles~\cite{Riggs2017-hm,Lee2022-vd, Remix_by_Via2021-vm,Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}.
% Geographic information systems manage access to increasing layers of information \cite{Ziliaskopoulos2000-az, Rasheed2020-op,Charitonidou2022-zg}.
In recent years, participatory design (PD) has gained popularity, incorporating citizen needs and preferences into the process of urban design and prototyping~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}.

% low-detail maps and patterns, PD prototyping
    \item \textit{Urban infrastructure design and policy-making uses design patterns and macroscopic traffic simulation.~}Urban infrastructure design also relies on established design patterns and guidelines~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. Additionally, designers~\cite{Zhang2022-uh, Dembski2020-gk} and policy makers~\cite{White2021-vo, Charitonidou2022-zg} use computational simulations to identify optimal infrastructure designs, for example, identifying the bus lane arrangement that causes minimal traffic disruption. % they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
    \item \textit{Traffic law design inherits prevailing law-making processes and uses quantitative modeling, regulatory sandboxes, and more.~}AV regulation is an active research topic in legal fields. Its approaches so far are largely reminiscent of traditional traffic law-making approaches. For example, conventional transportation research uses mathematical modeling to address policy questions (e.g., how tolls and fines impact traffic flows). Yet, some criticized that this approach assumes a top-down execution of proposed policies and is too detached from the messy policy-making cycles in practice.~\cite{Marsden2017-lu}. In response, lawmakers have adopted participatory approaches in making AV policies~\cite{van2022politics,lyons2022driverless}. They have created ``\textit{regulatory sandbox}'' for AV safety regulations as a means of providing a flexible regulatory environment for companies to iteratively test emerging technologies and business models~\cite{oecd2020-regulatory-sandbox,burd2021regulatory, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}. 
   % To overcome these  limitations, methods that enable policymakers themselves to make good decisions through data from the environment and citizens are proposed~\cite{White2021-vo, Marcucci2020-qg}. 
% Participatory methods have been part of policy-making since the beginning, through officials, agencies, and organized interest groups. Progress on how to scale up these approaches, better recognize efforts, and align various interests is still ongoing~\cite{Blomkamp2018-yg, Blomkamp2022-be, Oostveen2004-lk}.  % <- These are not AV-related policy work, right
     % \placeholder{Pilots in isolated regions to test AV safety. \cite{BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2019-wd, BMWK-Federal_Ministry_for_Economics_Affairs_and_Climate_Action2022-ck}}
\end{itemize}


% This parargaph: Some methods have the potential of supporting multiple designs. But no one acted on it.
Notably, researchers have argued that city-level simulation tools have the potential to support simultaneous urban infrastructure and policy design~\cite{Marcucci2020-qg,White2021-vo,Riggs2020-yc}. 
Interestingly, no research that we are aware of further explored this possibility or created such tools. 
%For example, %\citet{Haegler2021-xv} argued that VR microscopic driving simulations might also help prototype infrastructure and policy re-development. \hauke{VR microscopic driving simulation is not something I came across. The link is for a city simulation for architecture only. I don't know about a specifc research that argues this.}
% \citet{Marcucci2020-qg} and \citet{White2021-vo} argued that simulation tools have the potential to support simultaneous urban infrastructure and policy design.
% \citet{Riggs2020-yc} explored this idea in designing livable AV-infused cities, outlining how simulation tools can support both road space allocation and policy design.
Beyond traditional traffic simulations, ``\textit{digital twins}'' can appear a particular promising, albeit emerging, tool~\cite{shahat2021city}. Digital twin refers to a dynamic 3D model that mirrors a city's physical form and contains a city's information (e.g., street network space syntax, commuting patterns, the socioeconomic data of a neighborhood) throughout its lifecycle.
Digital twin's rich data allows for machine learning models that can answer ``\textit{what if}'' policy questions~\cite{nochta2021socio}.
Its comprehensive data offers a rare platform to support collaboration across city and policy design spheres and among the various stakeholders of the city~\cite{hamalainen2020smart}. 
% Dembski, F.; Wössner, U.; Letzgus, M.; Ruddat, M.; Yamu, C. Urban digital twins for smart cities and citizens: The case study of Herrenberg, Germany. Sustainability 2020, 12, 2307. 


% This paragraph: People have started designing policy and cities together
% A few notable exceptions exist: There are calls and early in development tools for designing urban infrastructure and policy (still excluding AVs) together using simulations \cite{Marcucci2020-qg, White2021-vo}.
% There is a framework to think about road space allocation and policies with AV growth \cite{Riggs2020-yc}. 


% hauke:
% People who try to design policies, AVs, and urban infrastructure lack methods to work together; therefore they mostly work separately; Their methods exclude other moving parts’ complexity.
% Evidence 1: AV design methods do not consider policies \&  infrastructure
% simulations focus on AV only (and simple road situations, etc.) + real world testing
% Cities are governed by complex rules that were established over long periods of time; current AV design, through real-world trials, takes urban infrastructure, and AV policy as determinate.
% Evidence 2: Urban infrastructure design \& policies don’t consider AV behavior design
% simulations focus on policy (only in online spaces) or city infra only
% Autonomous Vehicles (AV) are anticipated to radically change how we travel in the near future, with impact on how cities will be designed ultimately. Because of that wide acknowledged impact, local and federal governments want to regulate AV early on. 
% There are exceptions: In subfields…
% …


% \input{fig_rw_methods}

\subsection{Challenges in Designing AV, City, Policy Simultaneously}

Our analysis of existing methods also reveals a number of more significant barriers in prototyping AV, city, and policy design simultaneously.


\vspace{3pt}\noindent
\textbf{Different organizations own the design decisions of AVs, different components of city infrastructure, and different regulations.~}
Let us start with the biggest elephant in the room: that different private corporations and government agencies own the various AV, city, and policy design decisions. 
While multiple AV design researchers argued that small tweaks to traffic lights and road signs could significantly improve AV's computer vision model performance and driving safety~\cite{Niroumand2023-an,Gilbert-Sociotechnical,Riggs2019-lx, Nacto2019-pe}, they simply do not have the decision-making power in adopting these design proposals.
Designing AV, city, and policy simultaneously requires innovators to navigate the related political and organizational complexities, and it is not an easy task. 

% Further, in order for AVs and cities to form symbiotic relationships, research suggests tailoring for AV new types of roads, lanes, crossings~\cite{Riggs2019-lx, Nacto2019-pe}, traffic lights \cite{Niroumand2023-an}, reducing or displacing parking space \cite{Staricco2019-gn}, and designating alternative use of street space \cite{Freemark2020-ms}.  %\hauke{Changed to present tense as this has not happened yet.}
% If policies, road infrastructure and AVs \textit{are} designed together, entirely new concepts will become possible, \citet{Niroumand2023-an} propose a white traffic light phase at intersections, where AVs take over complete control of the right of way coordination. 

% This paragraph: acknowledging the politics involved in designing the trio simutanously: 
% AV, city, and policy design involve complex political processes that are often not fully acknowledged. The design of infrastructure, in particular, is embedded with politics and can shape the power dynamics of a society. As Winner argues, "the design of technology is itself a profoundly political activity" \cite{Winner1985-hp}. Similarly, Marsden \cite{Marsden2017-lu} argues that policymaking studies often overlook the complexities of the policymaking cycle. 
% Bringing together these different sectors to cooperate in designing AVs, cities, and policies requires recognizing and addressing these political complexities and is not an easy task.
% }\qian{For example, we only see democratic/participatory approaches to AV design used in policy/city design contexts, but not in AV company design contexts.}
% \hauke{I have a bit of that in line 187  \cite{Marsden2017-lu} argues that the field of policymaking study do not acknowledge the comlexities in the policy making cycle. Other than that I do not have a direct source in mind I read. https://www.taylorfrancis.com/books/mono/10.4324/9780203857557/politics-mobility-geoff-vigar (not read). We could also reference Winners bridges to briefly acknowldge that infrastructure (datasets, algorithms and policy too)  has built politics in.}

Moreover, driverless vehicles are far from homogeneous. (Think autonomous long-haul trucks, autonomous commercial drivers' vehicles, autonomous scooters for last-mile transportation, and food delivery robots.) Therefore, AVs will likely achieve wide adoption at different times, use different parts of the city infrastructure, and operate under different traffic and transportation regulations (e.g., AV scooters will likely be subject to micro-mobility laws, while low-haul trucks will be to Hours of Service regulations in the U.S.)
The wide variety of future AVs will add further complexities to the already complex AV-city-policy design landscape.


\vspace{3pt}\noindent
\textbf{Prototyping AV-human-city interactions both at individual and societal levels is computationally (too) demanding.~}
AV, city, and policy design operate at different scales, using varying levels of abstraction.
Take simulation as an example. 
Designing AV driving behavior models needs microscopic simulations. These simulations depict interactions among individual vehicles and pedestrians, typically in isolated encounters within short periods of time (e.g., when merging on highway)~\cite{Saidallah2016-zx}. 
City infrastructure and policy design need macroscopic simulations. They focus on traffic flows, their longitudinal patterns, and potential holistic impact on the city (e.g., would AV navigation patterns catalyze social inequalities across neighborhoods over time?~\cite{Gilbert-Sociotechnical}.) %\qian{Isn't digital twins an exception to this (it does both individual vehicle level and traffic flow level simulations)?}
Combining these simulations appears a promising approach to prototyping AV, city, and policy design simultaneously. However, this approach is computationally highly demanding.
Recent research has applied this integrative simulation approach to compare the impact of two scenarios of electric vehicles’ charging locations on charging demand~\cite{nochta2021socio}. It is unclear whether it is computationally feasible to simultaneously simulate multiple more complex AV, city, and policy design changes. 
% of varying granularity levels means that designers must wrestle with all of the above human-AV-environment interactions at the same time. Such integrative methods are likely to be cognitively demanding for the designers and computationally demanding for their simulation systems. 
% \qian{How is our method immune to this problem?}
% Nochta et al. illustrated the evaluation of different scenarios of electric vehicles’ charging locations and the cross-sectoral impacts through the city digital twin

% \hauke{
% - AVs can act as last mile transportation, intermediate distance transport networks, and even long-distance transport. 
% - AVs rollout can act slowly over time, or spontaneously all at once. 
% - AV rollout can occur in individual locations, or everywhere all at once. 
% - AV deployment thus poses policy challenges that need to be managed across whole cities, with many difficult local complexities. Once the tech is ready multiple competitors will try to enter the market all at once.  
% }
% AVs are like micromobility and trains simultaneously
% \subsubsection{What is novel about AVs in terms of planning complexity?}
% Autonomous vehicles represent a new frontier in urban and rural planning complexity.
% In the related work, we distinguished between transportation regulations and their relationship to AV service design, from traffic regulations and their relationship to AV motion design. 
% Unlike other transportation options, AVs can serve as last-mile transportation, intermediate distance networks, and long-distance transport. 
% Policy making for AVs requires regulating the local vehicle behavior—the AI driver, as well as its impact on the whole transportation—the AI taxi/bus service.  
% In this sense, AV service deployment for policymakers can be like deploying micromobility, coordination of shared mobility, and designing public transport systems all at once, adding layers of complexity to transportation planning that will require innovative solutions and careful consideration. 

% Some of these tensions can be attributed to an inherent conflict between AVs as commercial products versus AVs as public infrastructure \cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}. 
% Such trade-offs often occur in \placeholder{either-or social dilemmas}, for example, “\textit{should interest of passengers or the public good predominate}”~\cite{Bonnefon2015TheSD}, “\textit{should autonomous vehicles be owned or shared}”~\cite{Lee2019AutonomousVC, Campbell2018-rr}, and “\textit{should AVs be planned or self-organize}” \cite{Bosch2017-sv}? 
% As a result, tensions between different goals fields, and sectors, including the tensions between governmental and private entities, such as the tensions between AVs as commercial products versus AVs as public infrastructure, are discussed but never resolved.

% This paragraph is summarizing the proposed methods.
% Current scope-limited AV tests, complementary simulation studies, and analysis of natural human driving do not fully capture the effects that AVs will have at scale. They also do not consider the opportunities for re-designing urban and rural infrastructure or address nuanced human preferences.

% This paragraph: These methods can lead to results that are difficult to synthesize, because (2) they work under different assumptions and towards different goals
\vspace{3pt}\noindent
\textbf{Different assumptions and design goals underlie different AV, city, policy design efforts.~}
Even if one can simulate AV, city, and policy design changes in a shared simulation system, it can be difficult to align their design goals.
AV, city, and policy design methods often operate on different assumptions and pursue different goals.
In urban infrastructure design visions, driverless vehicles are often part of the public infrastructure. Innovators optimize AV, policy, and city design towards maximum public good, for example, less congestion~\cite{Metz2018-jn}, easier road maintenance~\cite{Gilbert-Sociotechnical}, and less environmental impact~\cite{Felipe-Falgas2022-dz}.
In AV motion design, AVs are privately-owned or company-owned commercial products that provide customers value. 
These varying assumptions led to insistent debates around, for example, how AVs should move, who has a say in how AVs should move, and how AVs fit into the public sphere~\cite{Wadud2021-zs, Rojas-Rueda2017-xl, Campbell2018-rr}.
% \qian{I know I wrote this, but I am not sure if these two sentences are true... They read like sweeping arguments. Will come back to this.} \hauke{I can see why you do not buy this. This unsureness about how it actually will unfold is discussed in the Ju Nissenbaum Paper. \url{https://papers.ssrn.com/sol3/papers.cfm?abstract_id=3875889}
% They identigy three archetypes of AVS: autonomous vehicles—advanced driver-assist systems (private), fully driverless cars (AV service), and connected cars. I am not certain about the connected cars though. cars of the other two categories can be conneted to?}
% \placeholder{Competing ownership visions (individually owned, service owners, governmental ownership) , different technology (connected via radio waves, high resolution sensor \&ml based)}





% Simulations are often better than modeling or optimization when dealing with complex systems, uncertainty, real-world scenarios, or exploratory analysis. Simulation, though, can run into computational limitations. Here, recent work pushed simulators to run at large scale~\cite{Chan2018-km}. 




% Common are microscopic simulation models, which model individual entities, and their interactions between traffic members, but they are limited in the scope they can model \cite{Saidallah2016-zx} 
% For infrastructure design, guidelines, and design patterns were established over time~\cite{Nacto2013-zd,Federal_Highway_Administration2023-wu}. These demand an update with specific AV patterns~\cite{Nacto2019-pe}.  
% Urban infrastructure simulations focus on improving urban infrastructure \cite{Zhang2022-uh, Dembski2020-gk}, or urban infrastructure policies only \cite{White2021-vo, Charitonidou2022-zg}; they do not consider AV behavior design or their implications \cite{Rouse2021-ph}.
% Participatory design methods are used in multiple areas to understand people's needs, in urban planning, tactical urbanism, citizen-led prototyping is becoming popular and shows unsatisfied needs by conventional planning~\cite{Streetplans_Collaborative2016-xt, Lydon2015-nn, Pfeifer2013-ew}. Tactical urbanism has informed policymaking, but not AV design.

% Policymakers, City, and AV designers need to make hard choices in the design process. This nuanced consideration of trade-offs is usually not considered in simulations and optimization, where only individual goals are measured or optimized \cite{Sharath2021-os, Rilett2020-fb}. Evaluation frameworks are multi-metric, with metrics like traffic flow, energy efficiency, vehicle routing/allocation, revenue, public health, and safety \cite{Yang2019-nr}. 
% There is disagreement, often unknowingly to stakeholders, how these ideals of livable, sustainable, equitable cities should look like in reality \cite{Staricco2019-gn, Meeder2017AutonomousVP, Acheampong2021-ql}. 


%\subsection{Our Proposal: Integrative City-AV-Policy Simulation (iCAPS)}
% \hauke{Complete, Citizen Centered City Simulation (4CS)}
% \hauke{Complete, Citizen Centered City AV Replicator (4CAR)} (or renderer)
\subsection{Potential Methods for Simultaneously Prototyping AV, City, and Policy Designs}
How to address these methodological and tooling challenges is worthwhile for future research to discuss.  To jump-start this discussion, we discuss three directions worthy of further exploration.
We direct our call for the development of such tools to the Human-Computer Interaction (HCI) community, due to their historic strong interdisciplinary work, human-centered design methods, and success in developing novel software-based prototyping tools. HCI should step ahead with the development of such methods and tools to address these methodological and tooling challenges, which are worthwhile for future research to discuss.


\vspace{3pt}\noindent
\textbf{Establish collaboration platforms and communities for AV designers, city planners, and policymakers.~}
% This paragraph: Recap -- These 3 groups of people have to work together, otherwise it’s just possible to anticipate cities or policies. Currently org barriers are high. How to make that happen is unclear.
To address design problems related to cities, AVs, and policy, it's important to acknowledge that different stakeholders own the decision-making process in each of these fields. It's unrealistic to expect designers to acquire the necessary expertise and authority in all three areas. Therefore, continuous collaboration among stakeholders is a necessity.

% This paragraph: It’s not impossible, things are happening.... Give examples of those signs.
Given political, business and organizational difficulties, we stress here that this type of collaboration is not unheard of. Mobility service startups and vehicle companies are already testing novel concepts with a few cities, states started requiring minimal AV data reports, and some local governments established collaborative policy design labs. 

% This paragraph: connect to the next two methods.
Below we describe two approaches that can support the collaborations among AV, city, and policy innovators. We hope that the emergence of such approaches can help catalyze such cross-sectional collaborations.


\vspace{3pt}\noindent
\textbf{Low-fidelity, integrative AV-city-policy prototyping by combining digital twins, machine learning behavioral modeling, and data visualization.~}
% This paragraph: Explain what we mean by this approach.
We recognize a parallel trend of increasing data collection and increased modeling detail for simulations in urban planning, service design, and AV motion design. Cross field data sharing can bring these high-fidelity data sources together in digital twins, specifically intended for untangling the AV, city policy design complexity. %  to design AV motion and traditional participatory design to design policy and AV Service, all simultaneously.  % WoZ with simulated AVs is most useful to simulate individual interactions with vehicles in individual streets. %Just as with tactical urbanism, 
% A change in traffic regulations just on AV provider's request without sufficient evidence is unlikely. To prove that, new av motion, which requires change in regulations, is satisfying user needs, a VR driving study could be conducted that asks people to fine-tune AV motion, traffic regulations, and urban infrastructure while assuming various perspectives such as a passenger, pedestrian encountering a vehicle, and resident in a neighborhood. The outcome of such a study will unravel different preferences for AV motion (e.g., AV acceleration values), urban infrastructure (e.g., width of AV lane) and traffic regulations (e.g., AV speed limit). With such a study, we can go beyond current AV motion design, which imitates human \textit{driver} behavior and takes regulations as well as infrastructure as fixed.
Integrative simulation environments, are necessary because only they allow for the evaluation and optimization of future transportation policies, city designs and AV behavior in a safe, controlled, and cost-effective environment; thereby also allowing to forecast opportunities and breakdowns/tensions that might emerge from the interactions between.

% Simulators are necessary because only they allow for the evaluation and optimization of future transportation policies, city designs and AV behavior in a safe, controlled, and cost-effective environment. 


% This paragraph: Previously people have solved the low-resolution design problems, but cannot “fine-tune” the models for different cities/local policies.
Previous simulation work allows for solving low-resolution network optimization: which districts should a bus line connect, how does an AV behave when a child walks in front of it. Increased level or resolution is desirable for AVs to fine-tune to different cities with local policies: How shall the new AV service connect these new communities exactly. 
Once processes and components are turned flexible, react with each other in a complex model, we can start to play with the simulated DNA of the city,  engineering preferable twins.   

% This paragraph: Previous barrier is computational intensity: ML can solve that by offering approximation. Evidence it would work: computer graphics.
As data storage and computation limit the integration fidelity, these digital twins have to use abstractions of representations. 
Transportation research faces the issue of computational barriers in modeling networks. Here, progress in ML algorithm optimization can help to simulate networks of increasing detail. For example, similar, in computer graphics, the rendering equation, long known, describes how to render scenes in a physically realistic way; optimizing this equation is still an ongoing challenge. Integrating the many simulations describing the interactions in the city requires directed effort in improving the simulation efficiency without impacting the simulation realism. 

% This paragraph: But ML also creates two new problems (1) this is a data-hungry solution. Describe why it’s important. Describe the progress made so far in data sharing. Future work should...
%\subsection{Requirement: Open Data, Simulators and Standards}
ML based digital twin simulations are data hungry. Many urban design tools, AV technology and traffic simulators are proprietary technology. Though progress is being made with open sharing of data, models, standardizing interfaces and open sourcing AV simulators. These tools and data sources are extremely valuable starting points for building a holistic simulator. 
Future policy work needs to address how the community can obtain access to the necessary data and models
%. Data sharing platforms could also facilitate communication and collaboration between different stakeholders, making it easier to identify potential conflicts or issues. 
% Finally, we suggest developing integrated design guidelines and standards that cover all aspects of AV design, city infrastructure, and policy can help ensure that all designs are compatible with each other and contribute to the goals of better cities. These guidelines and standards could be developed collaboratively by designers, policymakers, and other stakeholders and could be used to evaluate and approve new AV designs, infrastructure plans, and policy proposals.

% This paragraph: (2) needs visualization tools and ML approximation methods that can help people moving up and down levels of granularity
To make Digital Twins useful for prototyping AVs, city infrastructure, and policies simultaneously, they need to be equipped with the appropriate design tools to manipulate AV behavior, regulations, and infrastructure. Nowadays, these tools are not found in digital twins but only in the specific tools such as city planners.  Instead of using expensive handcrafting, Machine learning (ML) can aid by transferring point clouds of city scans into modifiable geometry of houses, streets, and traffic signs. 
%Machine learning methods that can detect bounding boxes of houses, street and traffic signs, already used for AV motion design, can automate these processes.
Complex processes of the city, and agent behaviors within, can be learned from the twin's rich data~\cite{Suo2021-vm}. These new data insights demand approximation methods that can help people move up and down levels of granularity.

% This paragraph: These two problems are interrelated -- cuz better way of visualizing/summarizing the trend  -> better sharing.
Creating better tools for sharing cities processes and behaviors and better tools for visualizing them synergetically benefit each other. 

% Holistic city simulators allow various stakeholders to engage across disciplines, but they allow policymakers to simulate how AV service and motion design might react to regulation and infrastructure changes. Do the implemented changes lead to the desired effects, will they cause unintended consequences, will the learning and automated AVs evade them?



\vspace{3pt}\noindent
\textbf{Participatory design optimization.~}
Participatory design (PD) methods, provide input by setting initial assumptions for further design steps, such as desired mix of privately owned and shared vehicles. Based on these assumptions, system designers can then, through multi-goal optimization, construct city, av, policy designs with optimal relationships between. If these  modeled designs, then reach the optimal configuration of trade-offs (also called Pareto boundary), again, PD can resolve conflicts by contributing additional subjective decision criteria, such as aesthetics. 
% \placeholder{Describe our solution: PD sets priorities, setting assumptions/setups (e.g., what mix of privately-owned vs. shared) + multi-goal optimization with AV/policy/city designers + PD resolving conflicts/trade-offs}
The two examples below can inform and assist policymakers and AV developers in coordinating actionable human preferences and resolving \textit{seemingly} trolley-problem-like conflicts.

% This paragraph: Why PD
\textit{Iterative Participatory Prototyping }can ease value tension through democratic decision-making. Participatory methods (PD) are preferred when tradeoffs between different goals lead to situations where improving one outcome will necessarily deteriorate another goal. Participatory design grounds these design decisions in the actual needs of the people affecting them, thereby effectively untangling goals and assumptions on the local (i.e., neighborhood), city spanning, and governmental level. 

% This paragraph: How might we do PD (for av policy city on local, city-spanning and governmental level)
People from their relevant neighborhood contribute local design knowledge such as where AV pick up spots and delivery stations shall be placed. Urban prototyping, offers engaging design methods to do so, by doing prototyping in the real physical space. %We suggest that policymakers and AV producers familiarize themselves with these rapid guerilla design methods and adopt them for participatory AV, policy, city prototyping. 

Apparent ethical AV dilemmas, can be resolved by conducting \textit{Participatory Ethics Experiments}. For example, in an online experiment; participants could provide input on complex questions related to AV traffic routing and zoning that have implications for infrastructure. These questions might include determining whether AVs should travel through primarily low-income areas or sightseeing districts,
%when efficiency is equal, who should bear the burden of noise and emissions. 
or whether AVs should park in designated slots outside the city to free up space or at curbside in the city. For later design stages, VR studies can be run in great detail and deliver nuanced human preferences: Currently, AV motion design is done with data obtained from driver perspectives (real world-data) VR diving studies can help to collect nuanced human preferences from AVs imagined being commanded as passengers, pedestrians, and people of local communities. This data could be used in the fine-tuning stage of AV models. 

% This paragraph: Why multi-goal simulation
In practice, many simulations exist for sub-problems in their fields. In these problem areas, different goals are prioritized. These address the problems of their specific subfields.  AV motion design predominately tries to solve the safety of AVs. Traffic regulation research favors network efficiency. In civil rights laws, equity with questions of accessibility is prioritized. Transportation regulations nowadays turned to sustainability. AV service design prioritizes the efficient use of all AVs. Urban rural infrastructure design addresses multiple goals that result in livable cities. We propose the good practice to use (Bayesian) multi goal optimization for simulations that acknowledge multiple goals to arrive at potentially equilibrated network designs. 

% The existing and proposed methods complement and complete each in a rich method space. Insights represented inside Transgenic Twins, combined with insights from Citizen Led City-AV-Policy Design can, with novel multi goal optimization techniques, help to find the Pareto optimal configuration of the city, and then policymakers can use subjective criteria and deliberation to decide for the best compromise. 


% \section{Discussion: What is needed from government, industry, and academia?}
% Discussion (“so what?”)
% Discussion: ⅓ page
% With the conclusions drawn in this short paper, we hope to induce the development of more integrated and participatory city design and AV policy prototyping tools. 
%, as it allows for the most flexibility and consolidation. 


% Limitations
% Ultimately, even the HCI community cannot devise these tools on their own, cross field and cross sector collaboration is necessary to achieve safe, livable, sustainable, efficient, and equitable cities with well-integrated AVs. 
\vspace{3pt}\noindent
\textbf{Limitations.~}Even though we promote citizen-led and integrated prototyping approaches, specialized field expertise is necessary. We do not see participatory methods and holistic simulators as the holy grail for all planning. While integrated tools can model and simulate many problems, they may not provide the necessary level of resolution for certain issues. As such, we encourage researchers in their respective subfields to continue their work, while advocating for standardization of software interfaces and open sharing of models.


%\section{Conclusion}
% Conclusion: 0 page

\section{Acknowledgement}
The authors are supported by the U.S. National Science Foundation under grants IIS-2107111 and IIS-2212431.
The second author is also partially supported by Schmidt Futures' AI2050 Early Career Fellowship.

%%
%% The next two lines define the bibliography style to be used, and
%% the bibliography file.
\bibliographystyle{ACM-Reference-Format}
\bibliography{paperpile,Sandhaus_manual}

% \appendix
%     \newpage
%     \section{Appendix}

